$S$-wave contribution to rare $D^0 \to \pi^+ \pi^- \ell^+ \ell^-$ decays in the Standard Model and sensitivity to New Physics

Physics of the up-type flavour offers unique possibilities of testing the Standard Model (SM) compared to the down-type flavour sector. Here, we discuss SM and New Physics (NP) contributions to the rare charm-meson decay $ D^0 \to \pi^+ \pi^- \ell^+ \ell^- $. In particular, we discuss the effect of including the lightest scalar isoscalar resonance in the SM picture, namely, the $f_0 (500)$, which manifests in a big portion of the allowed phase space. Other than showing in the total branching ratio at an observable level of about $ 20\% $, the $f_0 (500)$ resonance manifests as interference terms with the vector resonances, such as at high invariant mass of the leptonic pair in distinct angular observables. Recent data from LHCb optimize the sensitivity to $P$-wave contributions, that we analyse in view of the inclusion of vector resonances. We propose the measurement of alternative observables which are sensitive to the $S$-wave and are straightforward to implement experimentally. This leads to a new set of null observables, that vanish in the SM due to its gauge and flavour structures. Finally, we study observables that depend on the SM interference with generic NP contributions from semi-leptonic four-fermion operators in the presence of the $S$-wave.

==> Amplitude_analyses.tex <==





\section{Amplitude analyses based on the isobar model [for future work]}

One of the most important theoretical uncertainty components seems to be the unknown relative strong phases (i.e., beyond the strong phases encoded in Breit-Wigner functions, or another kind of line shape). We will attempt to have a better description of such aspect of the strong dynamics.

%NOTE: extract relevant information about normalisations and the strong phases [this last part is the ideal, but not necessarily well justified, i.e., not ``rocket-science''; one will have to argue that it is a step forward, calling for further dedicated work and better experimental and theoretical methods]

%NOTE: I am not convinced such analyses are ``universal'', i.e., information extracted from one decay mode can be employed in another (in other words yet, I am worried the analyses are reaction-dependent); hence, I don't know if the strong phases extracted via this approach can be used meaningfully elsewhere. One will have to argue that this is a step forward for a very challenging problem. [it should be OK as a starting point/first approximation; clearly, this is not ``rocket-science'']

%[note that one does not include $ 1 \to 1 $ in the analysis, possibly among other mechanism; this can be absorbed as a total $1 \to 2$]

Although an amplitude analysis based on the (non-dispersive) isobar model is not a model-independent technique,
we will exploit it to identify salient channels, and extract relevant information about normalisations and the strong phases.
We will assume the universality of the parameters extracted.
This is a working assumption for a very challenging problem, calling for further dedicated work and better experimental and theoretical methods.
In the future, we plan on improving on that based on dispersive methods, see e.g. \cite{Daub:2015xja}.
%step forward/starting point/first approximation

Experimentally, it is assumed that the relative strong phases aforementioned vary slowly (the faster variations being expected for the line shapes), so one takes them as constants in a first approximation if the main resonances are included in the analysis [the underlying mechanism for such strong phases should be rescattering effects].

Among the most relevant intermediate resonances, \cite{dArgent:2017gzv} identifies: $ a_1 (1260)^\pm $, $ \rho (770)^0 $, $ \sigma, f_0 (1370) $, $ \pi (1300)^\pm $ in $ D^0 \to \pi^+ \pi^- \pi^+ \pi^- $; while \cite{LHCb:2018mzv} identifies: $ \phi (1020) $, $ \rho (770)^0 $, $ K_1 (1270)^\pm $, $ K_1 (1400)^\pm $, $ K^\ast (892)^0 $, $ K^\ast (1680)^0 $ in $ D^0 \to K^+ K^- \pi^+ \pi^- $ [briefly summarize these papers; mention the quality of their fits; note that they include non-resonant contributions in their fits].
The relevant intermediate channels for rare decays are displayed in Tabs.~\ref{tab:amplitude_analysis_4pi} and \ref{tab:amplitude_analysis_2pi2K}, together with the relative complex/strong phases.

Note that Breit-Wigner is precarious for the $f_0 (500)$; \cite{dArgent:2017gzv} employs the model of Bugg [for consistency anyways one has to use the same model of \cite{dArgent:2017gzv}; for the background however they use a different lineshape for the $\sigma$].
The Gounaris-Sakurai parameterization of $ \rho (770)^0 \to \pi \pi $ is used in \cite{dArgent:2017gzv} [need to xcheck].

$ D^0 \to \pi^+ \pi^- \ell^+ \ell^- $ may require saying something about $\rho (770)^0 \to \pi^+ \pi^-$ ($I=1, J=1$) and $\phi (1020) \to K^+ K^-$ ($I=0, J=1$) to make amplitude analyses less reaction-dependent: it should be encoded in the Breit-Wigner line shapes, and the coupling $g_{\rho \pi \pi}$ -- $\rho (770)^0$ is isolated from $\rho (1450)^0$, and $\omega (782)$ and $\omega (1420)$ do not decay to $K^+ K^-$.

[comment about two-photon couplings]

It should be easier starting by looking at $ D^0 \to K^+ K^- \ell^+ \ell^- $. ($D^0 \to \phi (1020) \phi (1020) $ is not possible.)

%We could alternatively employ scalar isoscalar form factors, see Sec.~\ref{sec:FFs_DRs}.

\begin{figure}
    \centering
    \includegraphics[scale=0.25]{Q2B.png}
    \caption{Quasi two-body topologies.}
    \label{fig:Q2B_AAs}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.25]{cascade.png}
    \caption{Cascade topologies.}
    \label{fig:cascade_AAs}
\end{figure}

\input{tables.tex}

==> BABAR_extracts.tex <==
\section{BABAR analysis \cite{BaBar:2010vmf} [section not to be included in the final version]}

\begin{figure}
    \centering
    \hspace{-4mm}
    \includegraphics[scale=0.4,trim={0 13cm 0 0},clip]{Kpi_BABAR_threshold_800MeV.png} \\
    \includegraphics[scale=0.4,trim={0 13cm 0 0},clip]{Kpi_BABAR_800MeV_900MeV.png} \\
    \includegraphics[scale=0.4,trim={0 13cm 0 0},clip]{Kpi_BABAR_900MeV_1000MeV.png} \\
    \includegraphics[scale=0.4,trim={0 13cm 0 0},clip]{Kpi_BABAR_1000MeV_1600MeV.png} \\
    \caption{Extracts from BABAR \cite{BaBar:2010vmf}, from top to bottom: $ m_{K \pi} $ from threshold to 800~MeV, from 800~MeV to 900~MeV, from 900~MeV to 1000~MeV, and from 1000~MeV to 1600~MeV. When plotting the differential branching ratio as a function of $\cos \theta_{P_1}$: only $ I_{1,2} $ contribute, the $S-P$ interference is responsible for a term proportional to $\cos \theta_{P_1}$, $P$-only contributions to terms $\cos^2 \theta_{P_1}$ and $\sin^2 \theta_{P_1}$, while $S$-only is responsible for an offset. As a function of $\chi$: only $ I_{3,5,7} $ contribute non trivially ($ I_{1,2} $ give an offset), the $S$-wave gives dependences in $\sin \chi$ and $\cos \chi$, so an asymmetry in the former case, and the $P$-only gives $\cos 2 \chi$. As a function of $\cos \theta_e$: only $ I_{1,2,6} $ contribute, with no distinct contribution from the $S$-only.}
    %Picture of J-, W-type contributions: I am discussing only angular dependences, so this won't change the comments made above
    \label{fig:Kpi_BABAR}
\end{figure}

==> BESIII_extracts.tex <==
\section{BESIII analysis \cite{BESIII:2018qmf} [section not to be included in the final version]}

\begin{figure}
    \centering
    \includegraphics[scale=0.29]{BESIII_Dtopipienue_v2.png}
    \caption{Figure 2 from \cite{BESIII:2018qmf}. The $\sigma$ contribution is shown in red. ``To suppress the background to the $D^+$ signal from the decay of $D^+ \to K_S^0 e^+ \nu_e$, $K_S^0 \to \pi^+ \pi^-$, we veto events with a $\pi^+ \pi^-$ invariant mass within $\pm 70$ MeV/$c^2$ of the nominal $K_S^0$ mass, which eliminates about 98.3\% of such background.'' Note that the contribution from the scalar wave is large in the $q^2$ distribution, for which there is no interference with the $P$-wave! Its effect is visible in the angular distributions, producing asymmetries and differences compared to the channel $D^0 \to \pi^- \pi^0 e^+ \nu_e$, for which there is no $f_0 (500)$ contribution; more pronounced effects are expected when considering slices of $m_{\pi^+ \pi^-}$ instead of integration over all its allowed values (such is seen in the case of $D^+ \to K^- \pi^+ e^+ \nu_e$ \cite{BaBar:2010vmf}).}
    \label{fig:BESIII_Dtopipienue}
\end{figure}

==> CMD2_extracts.tex <==
\section{CMD-2 analysis \cite{CMD-2:2001ski} [section not to be included in the final version]}

\begin{figure}
    \centering
    %\includegraphics[scale=0.4]{lhcbComparisonWdatapoints.png}
    \includegraphics[scale=0.2]{CMDII_rho_omega.png}
     \caption{Figure~4 from CMD-2 \cite{CMD-2:2001ski}, which extracts $ \mathcal{B} (\omega \to \pi^+ \pi^-) = (1.33 \pm 0.24 \pm 0.05) \% $; we also employ information from \cite{BESIII:2018qmf,Shulei}}
\end{figure}

==> Estimating_the_phases_from_the_angular_observables.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Estimating the phases from the angular observables?}
[appendix for temporary use]
For the only-W/$C_9^{eff}$ case, $I_4$(of P-wave) always comes out positive by construction, because of the values that the form factors take. For the same reason $I_3$ would also come out always negative. In the presence of $J$, there is a possibility to have a contribution, to the angular observable expression, of the opposite sign around bins 5 and 6, because of a factor $\cos(\arg J-\arg W)$. However this contribution doesn't achieve flipping the sign altogether (but we're still looking into possibilities of different phases).
[\rd{we later identified a problem comparison with LHCb because angles are seemingly defined differently}]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{tabular}{|c|c|c|}
    \hline 
    $\sqrt{q^2}$  region & $<I_2>, \phi_\rho=\phi_\phi=0$(\%) & $<I_2>, \phi_\rho=\pi, \phi_\phi=0$ (\%) \\
    \hline 
   %%$ r^{({\rm low})} $ & -15 &\\ 
   %%$ r^{(\eta)} $ & -15 &\\ 
   %%$ r^{(\rho: {\rm inf})} $  & -11 &\\
   $ r^{(\rho: {\rm sup})} $  & -10 &\\ 
   $ r^{(\phi: {\rm inf})} $   & -9  &\\
   $ r^{(\phi: {\rm sup})} $    & -9  &\\
   %%$ r^{({\rm high})} $    & -12 & \\
       \hline
    \end{tabular}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{tabular}{|c|c|c|c|}
    \hline 
    $\sqrt{q^2}$  region & $<I_3>, \phi_\rho=\phi_\phi=0$(\%) & $<I_3>, \phi_\rho=\pi, \phi_\phi=0$ (\%) & $<I_3>, \phi_\rho=4.5, \phi_\phi=0$ (\%)\\
    \hline 
   %%$ r^{({\rm low})} $ & -2.5 & -2.3 & -2.3\\ 
   %%$ r^{(\eta)} $ & -4.3 & -4.1 & -4.2\\ 
   %%$ r^{(\rho: {\rm inf})} $  & -8.4 & -8.3 & -8.4\\
   $ r^{(\rho: {\rm sup})} $  & -10  & -9.8 & -9.8\\ 
   $ r^{(\phi: {\rm inf})} $   & -14  & -13.8& -13.7\\
   $ r^{(\phi: {\rm sup})} $    & -14  & -14.2& -14.1\\
   %%$ r^{({\rm high})} $    & -13  &  -15 & -15.1\\
       \hline
    \end{tabular}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{tabular}{|c|c|c|c|}
    \hline 
    $\sqrt{q^2}$  region & $<I_4>, \phi_\rho=\phi_\phi=0$(\%) & $<I_4>, \phi_\rho=\pi, \phi_\phi=0$ (\%) & $<I_4>, \phi_\rho=4, \phi_\phi=0$ (\%)\\
    \hline 
   %%$ r^{({\rm low})} $ & 11 & 10 & 16\\ 
   %%$ r^{(\eta)} $ & 15 & 15 & 22\\ 
   %%$ r^{(\rho: {\rm inf})} $  & 19 & 19 & 28\\
   $ r^{(\rho: {\rm sup})} $  & 19 & 20 & 30\\ 
   $ r^{(\phi: {\rm inf})} $   & 19 & 19 & 28\\
   $ r^{(\phi: {\rm sup})} $    & 18 & 19 & 29\\
   %%$ r^{({\rm high})} $    & 17  & 19 & 29\\
       \hline
    \end{tabular}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Form_factors.tex <==
\subsection{Expressions for form factors}

Paper by Bajc et al. \cite{Bajc:1997nx}.
For a more recent reference see Ivanov et al. \cite{Ivanov:2019nqd}.

[Hai-Yang Cheng et al. (hep-ph/2201.00460) discusses the $f_0 (500)$ in hadronic charm meson decays]

%[for $a_1, K_1$, see Hai-Yang Cheng et al. (hep-ph/0301198, hep-ph/1002.2466, etc.)]

==> Form_factors_in_hadronic_weak_decays.tex <==
\textbf{Form factors in hadronic weak decays}

Discussion of Daub et al. \cite{Daub:2015xja} of $\overline{B}^0_{d/s} \to J / \psi \pi \pi$. The assumption being made therein is that the $J/\psi$ and the $\pi^+ \pi^-$ factorize, as no particular structure is seen for the invariant mass of $ J/\psi \pi^+ $ (i.e., a simpler analytic structure holds)\footnote{The qualitative idea is that the most relevant effect is the exchange of resonances in the $s$-channel, which is taken into account dispersively.}, [this being the only argument provided to support their analysis that I have identified so far]; there is also a discussion about intermediate contributions from $ \psi (2 S) $ and $ B^\ast $. Ref.~\cite{Ropertz:2018stk} includes an effective $4 \pi$ channel for the sake of going beyond $\sqrt{s} = 1.05$~GeV for the invariant mass of the pion pair. See also \cite{Albaladejo:2016mad}, and \cite{Gardner:2001gc} in the context of $ B^0 (\overline{B}^0) \to f_0 (500) \pi^0 $. For Cabibbo-favored $ D^+ \to K \pi \pi^+ $ decays, see e.g. \cite{Oller:2004xm,Boito:2009qd,Nakamura:2015qga,Niecknig:2015ija,Niecknig:2017ylb}.
Note also \cite{JPAC:2017vtd}.

We could make an analogous assumption in the case of rare charm meson decays $ D^0 \to [\rho (770)^0 \to \ell^+ \ell^-] \, \pi^+ \, \pi^- $ and $ D^0 \to [\rho (770)^0 \to \ell^+ \ell^-] \, K^+ \, K^- $. However, note e.g. the presence of the resonances $ a_1 (1260)^\pm [\to \pi^\pm \, \rho (770)^0] $ (of total width $ 250 - 600 $~MeV, according to PDG) and $ K_1 (1270)^\pm [\to [K^\pm \, \rho (770)^0]_{L=0}] $ (of total width $ 90 \pm 20 $~MeV, according to PDG): it may be possible to perform a similar analysis as in the cases $\overline{B}^0_{d/s} \to J / \psi \pi \pi$ staying sufficiently below $ \sim 1 $~GeV, i.e., for large enough invariant mass of the leptonic pair, which may be the case for the full extent of the high window in charm meson decays.

There is also the possibility of an (elastic?) analysis of $ D^0 \to [\phi (1020)^0 \to \ell^+ \ell^-] \, \pi^+ \, \pi^- $. As before, note e.g. the presence of the resonance $ a_1 (1260)^\pm [\to [\pi^\pm \, \phi (1020)^0]_{L=0}] $.

%(Neglecting penguin operators, it seems that there is no CPV in $ D^0 \to \phi (1020) \pi \pi $, since there is a single weak phase available, the one from $ c \to s \bar{s} u $; $ \phi (1020) $ is essentially a strange-quark pair.)
%If a similar comment applies to $ D^0 \to \rho (770)^0 \pi \pi $ (namely, $ \rho (770)^{\pm, 0} $ is essentially a light-quark pair.), then there is no CPV in this system as well, since there would be a single weak phase. [rescattering should invalidate this reasoning, but it should not change Okubo's rule; not sure the reasoning is meaningful]

[\textit{this dispersive discussion could provide a better understanding of QCD, and of interference terms: $I_{4,5,7,8}$ are sensitive to the interference of $\rho \to \pi \pi$ and $\sigma \to \pi \pi$}]
%but this direction won't be useful for NP, since after factorization of the vector resonance both SM and NP would share the same strong phases, and dispersive modulation (aka Omn\`{e}s factor): we have the vector, and also the scalar contributions
%even if the former is J=1 (I=1), and the latter J=0 (I=0)?
%the rho is massive; the rho couples to the photon to produce a lepton pair

(Spectator-quark annihilation topologies may be relevant in the context of charm physics compared to bottom physics; it may complicate the analysis of charm decays even more; cf. Feldmann et al.)

==> LHCb_extracts.tex <==
\section{LHCb analysis \cite{LHCb:2021yxk} [section not to be included in the final version]}

\begin{figure}
    \centering
    \includegraphics[scale=0.15]{hidef_fig6a.png} \hspace{5mm} \includegraphics[scale=0.15]{hidef_fig6b.png} \\
    \includegraphics[scale=0.15]{hidef_fig6c.png} \hspace{5mm} \includegraphics[scale=0.15]{hidef_fig6d.png}
    \caption{Background subtracted mass spectra of the two-body combinations. Dominik Mitzel: ``You can clearly see the dominance of the P-wave in $m(hh)$, but also other possible contributions.'' Note, \cite{LHCb:2021yxk}: ``The piece-wise integration in $\cos \theta_h$ is defined to optimise the sensitivity given that the dihadron system is dominated by intermediate $P$-wave resonances, which further decay into $h^+ h^-$ ($\rho \to \pi^+ \pi^-$ and $\phi \to K^+ K^-$ for $D^0 \to \pi^+ \pi^- \mu^+ \mu^-$ and $D^0 \to K^+ K^- \mu^+ \mu^-$ decays, respectively). No further attempt to separate partial waves contributing to the coefficients $\langle I_i \rangle$ is made.'' [is the pic at around $0.5$~GeV due to a $K_S^0$ (diagram with a $W$ exchanged with the spectator quark; Cabibbo allowed, lepton pair emitted via bremsstrahlung)?, see case $D^+ \to \pi^+ \pi^- e^+ \nu_e$] Dominik Mitzel: ``$K_S^0$ contributions are not explicitly vetoed. However, from an experimental point of view, we require all four final state tracks to originate from a common decay vertex, so $K_S^0$ should be suppressed to a certain amount, but unfortunately I cannot give a more quantitative reply.''}
    \label{fig:LHCb_supplementary_material}%https://lhcbproject.web.cern.ch/Publications/LHCbProjectPublic/LHCb-PAPER-2021-035.html
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.32]{symmetric_combinations.png}
    \includegraphics[scale=0.32]{asymmetric_combinations.png}
    \caption{Extracts of \cite{LHCb:2021yxk}. Large values for some bins of $\langle S_{4, 5, 8} \rangle$ ($\langle S_7 \rangle$ completes the list) DO NOT indicate the presence of the $S$-wave: by definition, the integration $ \langle \cdot \rangle $ eliminates the $S$-wave contribution.
    %However, the statistical significance as of now is limited.
    No large correlations (larger than $23\%$ in modulus) for the bins $ 565 - 780 $~MeV, $ 780 - 950 $~MeV, $ 950 - 1020 $~MeV, $ 1020 - 1100 $~MeV across different observables is present. The $\eta$ region and the high-mass window have poor significance of events \cite{LHCb:2017uns} and the angular observables are not measured therein. [a statistical comparison is possible, however w/o cascade decays I don't know if that would be fully meaningful][Why $\langle S_1 \rangle, \langle A_1 \rangle$ are not being shown?, they are basically $\langle S_2 \rangle, \langle A_2 \rangle$][ANGLES ARE DIFFERENT???]}
    %\label{fig:my_label}
\end{figure}

==> Lattice_QCD.tex <==
\subsection{Lattice results}

Luka mentioned a decay mode: ``A lattice QCD study of $B \to \rho \ell \nu$''; ``A lattice QCD study of the $B \to \pi\pi \ell \nu$ transition''; will $D \to \rho$ also be available?

==> OLDobservablesvalues.tex <==
\begin{table}
\hskip-3.3cm
    \begin{tabular}{|c|c|c|c|c||c|c|}
    \hline 
   $\sqrt{q^2}$  region & $\Gamma[10^{-5}]$ & $ \frac{\Gamma_\sigma}{\Gamma}(\%) $ & $(\int   dp^2 I_2)_{\text{total}}[10^{-5}]$ & $(\int   dp^2 I_2)_\sigma /(\int   dp^2 I_2)_{\text{total}}(\%)$ & $(\int   dp^2 I_3)_+[10^{-6}]$ & $(\int   dp^2 I_4)_-[10^{-5}]$ \\
    \hline 
   $ r^{({\rm low})} $ & 0.09 &   9.1  & -0.014  &14 & -0.024 & 0.016\\ 
   $ r^{(\eta)} $ & 0.04 &   8.3  & -0.007   &16& -0.019 & 0.010\\ 
   $ r^{(\rho: {\rm inf})} $  & 3.71 &    7.2  & -0.41   &21& -3.15 & 1.06\\
   $ r^{(\rho: {\rm sup})} $  & 3.68 &  6.4   &  -0.35   &22 & -3.67& 1.09\\ 
   $ r^{(\phi: {\rm inf})} $   & 3.94 &  16.6  &   -0.35    &65& -5.46& 1.13\\
   $ r^{(\phi: {\rm sup})} $    & 3.14 &  18.0    &  -0.29     & 69& -4.35& 0.88\\
   $ r^{({\rm high})} $  & 0.004 & 27.7 & -0.00056  & 81  & -0.006& 0.012\\
       \hline 
    \end{tabular}
    \caption{In $q$-bins, observables in the SM where the effect of the $\sigma$ is additive ($\Gamma, I_2$) and observables which only receive P-wave contributions ($I_3, I_4$). For an estimate of the angular observables comparable to the bins provided by LHCb, divide the respective column with the first. The decay rates and the $I_i$'s both need to be multiplied by a common constant factor, $|C_2\lambda_d e G_F/\sqrt{2}|^2\frac{e^2}{m_D}$ }
    \label{gammas,i2}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\begin{tabular}{|c|c|c|c|}
        \hline
  $\sqrt{q^2}$  region & $\frac{2}{\pi}(\int   dp^2 I_2)_{(+,S)}[10^{-5}]$ & $\frac{2}{\pi}(\int   dp^2 I_4)_{(+,S)}[10^{-5}]$ & $\frac{2}{\pi}(\int   dp^2 I_8)_{(+,S)}[10^{-7}]$  \\
\hline 
   $ r^{({\rm low})} $ &  & -0.0019 &  -0.026 \\ 
   $ r^{(\eta)} $ & &  -0.0012&  -0.020 \\ 
   $ r^{(\rho: {\rm inf})} $  & & -0.124&    -2.41  \\
   $ r^{(\rho: {\rm sup})} $ &  &  -0.119&   -2.88 \\ 
   $ r^{(\phi: {\rm inf})} $  &  & -0.198& -6.55   \\
   $ r^{(\phi: {\rm sup})} $  &  &  -0.166& -5.25 \\
   $ r^{({\rm high})} $  &  & -0.0004& -0.0004\\
       \hline
    \end{tabular}
    \caption{In $q$-bins, angular observables in the SM which isolate the effect of $\sigma$ in its interference with the P-wave, when integrated in our suggested way.For an estimate of the observables comparable to the bins provided by LHCb, divide the corresponding columns with the binned decay rates of the first column of \ref{gammas,i2}.}
\label{i2i4i8}
 \end{table}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   \begin{tabular}{|c|c|c|c|c|}
%    \hline 
%    $\sqrt{q^2}$  region (GeV) & $\Gamma[10^{-5}]$ & $ \frac{\Gamma_\sigma}{\Gamma}(\%) $ & $(\int   dp^2 I_2)_{\text{total}}[10^{-5}]$ & $(\int   dp^2 I_2)_\sigma /(\int   dp^2 I_2)_{\text{total}}(\%)$ \\
%    \hline 
%   0.212-0.525 &  28.1 & 3.8 & -0.014  &14\\ 
%   0.525-0.565 &   4.70& 4.7 & -0.007   &16\\ 
%   0.565-0.78  &  58.5 & 6.5 & -0.41   &21\\
%   0.78- 0.95 &  28.5 & 6.6  &  -0.35   &22\\ 
%   0.95-1.02  & 6.04 & 21 &   -0.35    &65\\
%1.02-1.1  &  4.63 &  23   &  -0.29     & 69\\
%       1.1-1.59  & 0.0054 & 30 & -0.00056  & 81\\
%       \hline
%    \end{tabular}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{table}[]
%    \centering
%   \begin{tabular}{|c|c|c|}
%    \hline
%    $\sqrt{q^2}$ region (GeV) & $(\int   dp^2 I_3)_+[10^{-6}]$ & $(\int   dp^2 I_4)_-[10^{-5}]$\\
%    \hline
% 0.212-0.525 & -0.024 & 0.016\\ 
%   0.525-0.565 & -0.019 & 0.010\\ 
%   0.565-0.78  & -3.15 & 1.06\\
%   0.78- 0.95 & -3.67& 1.09\\ 
%   0.95-1.02  & -5.46& 1.13\\
%    1.02-1.1   & -4.35& 0.88\\
%    1.1-1.59   & -0.006& 0.012\\
%    \hline
%    \end{tabular}
%    \caption{In $q^2$-bins, observables, in the SM, which are only sensitive to the P-wave. For a comparison to the LHCb values, divide by the decay rates provided in \ref{gammas,i2}.
%    For the absolute values of the presented observables they need to be multiplied by a common constant factor, $|C_2\lambda_d e G_F/\sqrt{2}|^2\frac{e^2}{m_D}$}
%    \label{i3}
%\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    $\sqrt{q^2}$  region & $\frac{2}{\pi}(\int   dp^2 I_5)_{(+,S)}[10^{-7}]$ & $\frac{3}{2}(\int   dp^2 I_5)_{(-,P)}[10^{-7}]$ &$\frac{2}{\pi}(\int   dp^2 I_7)_{(+,S)}[10^{-7}]$ & $(\int   dp^2 I_6)_{(+,P)}$ \\
      \hline 
   $ r^{({\rm low})} $ &-3.5 & 16.2 & -0.42 & \\ 
   $ r^{(\eta)} $ &-1.4&  6.6 & -0.14&  \\ 
   $ r^{(\rho: {\rm inf})} $  &-2.4&  2.9& 9.7&  \\
   $ r^{(\rho: {\rm sup})} $ & 0.53& -3.1& 7.0 &  \\ 
   $ r^{(\phi: {\rm inf})} $  & 8.8& -43 & 14.3& \\
   $ r^{(\phi: {\rm sup})} $   &-5.6 & 23 & -9.4&  \\
   $ r^{({\rm high})} $   & -0.32& 0.2& -0.2 & \\
       \hline
    \end{tabular}
    \caption{In $q^2$-bins, observables that vanish in the SM, here calculated for $C_9'=C_{10}'=0$ and non-zero $C_{10}$. $\braket{I_5}_+$ and $\braket{I_7}_+$ are sensitive to NP in the presence of the $\sigma$. $\braket{I_5}_-$ and $\braket{I_6}_+$ (integrated as per LHCb) are sensitive to NP through the P-wave and unaffected by the S-wave. The rest of the null-test observables 5-7 vanish or are below detectable levels; the same is true for $\braket{I_8}_-, \braket{I_9}_+$ in this particular configuration of NP Wilson coefficients. The observables have to be multiplied by $C_{10} C_2\lambda_d e^2 G_F/\sqrt{2}\frac{1}{m_D}$ \rd{[corrected]; here it is assuming there's no prefactor in C10]}.[probably $C_{10}^*$ but I set the phase to zero, check] [\LVS{also include branching ratios}]}
    \label{NPobsevables}
\end{table}

==> Some_estimates.tex <==
\paragraph{Some estimates [OBSOLETE]}
With the above implementation we check what the effect is on the differential branching ratio plotted over $q^2$. The results can be seen in fig.\ref{d5Gammas}. It seems 
\begin{figure}
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=0.5\linewidth]{d5Gamma.jpeg}
  \caption{Differential branching ratio for the full range of $q^2$, with or without $\sigma$ with $a_s=2$}
  \label{fig:sfig1}
\end{subfigure}%
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=.5\linewidth]{d5Gammacomparison.jpeg}
  \caption{The same but for higher $q^2$}
  \label{fig:sfig2}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.2\linewidth]{d5Gammaonlysigma.jpeg}
  \caption{The effect of $\sigma$ alone parameterised as in BES with $a_s=2$, ignoring all other contributions.}
  \label{fig:sfig3}
\end{subfigure}
%\caption{plots of....}
\label{d5Gammas}
\end{figure}


We try with different "relative magnitudes" but the result does not change. We try to see where the difference between the effect of $\rho$ and that of $\sigma$ comes from. 

Let us rewrite the expressions for the dihadron part of the amplitude: 
\begin{equation}
    <\pi\pi|j^\mu|D^0>_\sigma=2\frac{h(p^2)}{1-\frac{q^2}{m_A^2}}\frac{1}{P_\sigma(p^2)}b_\sigma p^\mu
\end{equation}
\begin{equation}
    <\pi\pi|j^\mu|D^0>_\rho=-\frac{i}{m_D+m_\rho}\frac{h_{A2}}{1-\frac{q^2}{m_{A2}^2}}q\cdot\epsilon_{(\rho)}^* \Bigl(p_D+p-\frac{m_D^2-m_\rho^2}{q^2}q\Bigl)^\mu+...
\end{equation}

\begin{enumerate}
    \item Propagators: plotted over $p^2$ the propagator of $\sigma$ is at least 2 times larger than the one of $\rho$%, see fig. \ref{propagatorsfig}.
    \item Form factors, numerator: We identify $a_s M\Gamma_1(p^2)$ with $2h(p^2)b_\sigma$, and can take that at high $p^2$: $h(p^2)\approx h_pi=ff(D\rightarrow\pi,q^2=0)$. $h_pi$ is similar to the $h$'s that appear in $D\rightarrow\rho$, but we have the extra factor of 2 in front. For small $p^2$ the "modified form factor" is significantly smaller.
     \item Form factors, denominator: All $m_A$, $m_V$ are of similar order.
    \item $b$ constants: $b_\rho\approx (2-3)b_\sigma$
\end{enumerate}

%\begin{figure}
%    \centering
 %   \includegraphics{propagators.jpeg}
%    \caption[scale=0.3]{The propagators of the scalar and $\rho$}
%    \label{propagatorsfig}
%\end{figure}

==> Vgamma-DecayConstants.tex <==
Eq. \eqref{HVgamma} comes directly from the resonance chiral theory framework (with individual decay constants for the different resonances). However, if this Lagrangian is implemented then the decay constants have to be consistent: instead of the ones of the appendix, we would need to have 
\begin{align}
    \langle \rho^0 | \overline{d}\gamma^\mu d  | 0 \rangle = - f_\rho m_\rho \epsilon^{*\mu} \\
    \langle \omega | \overline{u}\gamma^\mu u  | 0 \rangle  = f_\omega m_\omega \epsilon^{*\mu} \\
    \langle \phi | \overline{s}\gamma^\mu s     | 0   \rangle = \sqrt{2} f_\phi m_\phi \epsilon^{*\mu}
\end{align}

In that case the values of the decay constants are of course not the ones around 200 MeV quoted in the appendix.  Instead, if we have the decay constants of the appendix, then \textbf{the Hamiltonian should be rewritten as}

\begin{equation}
    \mathcal{H}_{\mathcal{V}\gamma} = -e \, \left(\frac{f_{\rho^0}}{\sqrt{2}m_{\rho^0}}\left(\rho^0\right)^\mu \,+\frac{1}{3}  \frac{f_{\mathcal{\omega}}}{\sqrt{2}m_{\mathcal{\omega}}} \, \mathcal{\omega}^\mu -\frac{\sqrt{2}}{3}\frac{f_{\mathcal{\phi}}}{\sqrt{2}m_{\mathcal{\phi}}} \, \mathcal{\phi}^\mu \right) \, \square A_\mu 
\end{equation}
and consequently for the W-type we have $ c^W_{\rho^0} = 1/2$, $ c^W_\omega = -1/6 $ and $ c^W_\phi = -1/3 $ whereas for the J-type we just have $ c^J_{\rho^0} = 1/\sqrt{2} $, $ c^J_\omega = +1/(3\sqrt{2}) $ and $ c^J_\phi = 0 $. We also have an extra $1/sqrt{2}$ from the $0\to\rho(\to \pi\pi)$, as before.

Regarding what I have written in the code, it seems that $B_{\rho,code}=B_\rho$, $B_{\omega,code}=B_{\omega}$, $B_{\phi,code}=1/\sqrt{2}B_\phi$. The relative phases between the $\rho,\omega,\phi$ should be as extracted from the fit, with no modification.

==> angobservablesHilleretc.tex <==
\begin{eqnarray}

    && I_1 = \frac{1}{8} \left[ | \mathcal{F}_0 |^2 \, \rho^-_1 + \frac{3}{2} \sin^2 \theta_{P_1} \left\{ | \mathcal{F}_\Vert |^2 \, \rho^-_1 + | \mathcal{F}_\perp |^2 \, \rho^+_1 \right\} \right] \\
    && \qquad\qquad\qquad \stackrel[]{SM}{\to} \frac{1}{8} \left[ | \mathcal{F}_0 |^2 + \frac{3}{2} \sin^2 \theta_{P_1} \left\{ | \mathcal{F}_\Vert |^2 + | \mathcal{F}_\perp |^2 \right\} \right] \, | C_9^{\rm eff} |^2 \,, \nonumber\\
    && I_2 = -\frac{1}{8} \left[ | \mathcal{F}_0 |^2 \, \rho^-_1 - \frac{1}{2} \sin^2 \theta_{P_1} \left\{ | \mathcal{F}_\Vert |^2 \, \rho^-_1 + | \mathcal{F}_\perp |^2 \, \rho^+_1 \right\} \right] \\
    && \qquad\qquad\qquad \stackrel[]{SM}{\to} -\frac{1}{8} \left[ | \mathcal{F}_0 |^2 - \frac{1}{2} \sin^2 \theta_{P_1} \left\{ | \mathcal{F}_\Vert |^2 + | \mathcal{F}_\perp |^2 \right\} \right] \, | C_9^{\rm eff} |^2 \,, \nonumber\\
    && I_3 = \frac{1}{8} \left[ | \mathcal{F}_\perp |^2 \, \rho^+_1 - | \mathcal{F}_\Vert |^2 \, \rho^-_1 \right] \, \sin^2 \theta_{P_1} \stackrel[]{SM}{\to} \frac{1}{8} \left[ | \mathcal{F}_\perp |^2 - | \mathcal{F}_\Vert |^2 \right] \, \sin^2 \theta_{P_1} \, | C_9^{\rm eff} |^2 \,, \\
    && I_4 = -\frac{1}{4} \text{Re} ( \mathcal{F}_0 \mathcal{F}^\ast_\Vert ) \, \rho^-_1 \, \sin \theta_{P_1} \stackrel[]{SM}{\to} -\frac{1}{4} \text{Re} ( \mathcal{F}_0 \mathcal{F}^\ast_\Vert ) \, \sin \theta_{P_1} \, | C_9^{\rm eff} |^2 \,, \\
    && I_5 = \left[ \text{Re} \left( \mathcal{F}_0 \mathcal{F}^\ast_\perp \right) \, \text{Re} \rho^+_2 + \text{Im} \left( \mathcal{F}_0 \mathcal{F}^\ast_\perp \right) \, \text{Im} \rho^-_2 \right] \, \sin \theta_{P_1} \stackrel[]{SM}{\to} 0 \,, \\
    && I_6 = - \left[ \text{Re} \left( \mathcal{F}_\Vert \mathcal{F}^\ast_\perp \right) \, \text{Re} \rho^+_2 + \text{Im} \left( \mathcal{F}_\Vert \mathcal{F}^\ast_\perp \right) \, \text{Im} \rho^-_2 \right] \, \sin^2 \theta_{P_1} \stackrel[]{SM}{\to} 0 \,, \\
    && I_7 = \text{Im} ( \mathcal{F}_0 \mathcal{F}^\ast_\Vert ) \, \delta \rho \, \sin \theta_{P_1} \stackrel[]{SM}{\to} 0  \,, \\
    && I_8 = \frac{1}{2} \left[ \text{Re} \left( \mathcal{F}_0 \mathcal{F}^\ast_\perp \right) \, \text{Im} \rho^+_2 - \text{Im} \left( \mathcal{F}_0 \mathcal{F}^\ast_\perp \right) \, \text{Re} \rho^-_2 \right] \, \sin \theta_{P_1} \stackrel[]{SM}{\to} - \frac{\text{Im} \left( \mathcal{F}_0 \mathcal{F}^\ast_\perp \right)}{2} \sin \theta_{P_1} \, | C_9^{\rm eff} |^2 \,, \label{I8fact} \\
    && I_9 = \frac{1}{2} \left[ \text{Re} ( \mathcal{F}_\perp \mathcal{F}^\ast_\Vert ) \, \text{Im} \rho^+_2 + \text{Im} ( \mathcal{F}_\perp \mathcal{F}^\ast_\Vert ) \, \text{Re} \rho^-_2 \right] \, \sin^2 \theta_{P_1} \stackrel[]{SM}{\to} \frac{\text{Im} ( \mathcal{F}_\perp \mathcal{F}^\ast_\Vert )}{2} \sin^2 \theta_{P_1} \, | C_9^{\rm eff} |^2 \,,
    \label{Isfact}
\end{eqnarray}



\begin{eqnarray}
    && \langle I_1 \rangle_{-} = \frac{1}{4} \text{Re} \left( \mathcal{F}_S \mathcal{F}^\ast_P \right) \, \rho^-_1 \,, \\
    && \langle I_2 \rangle_{-} = -\frac{1}{4} \text{Re} \left( \mathcal{F}_S \mathcal{F}^\ast_P \right) \, \rho^-_1 = -\langle I_1 \rangle_{-} \,, \\
    && \langle I_3 \rangle_{-} = 0 \,, \\
    && \frac{3}{2} \langle I_4 \rangle_{-} = -\frac{1}{4} \text{Re} \left( \mathcal{F}_P \mathcal{F}^\ast_\Vert \right) \, \rho^-_1 \,, \label{I4vector} \\
    && \frac{3}{2} \langle I_5 \rangle_{-} = \left[ \text{Re} \left( \mathcal{F}_P \mathcal{F}^\ast_\perp \right) \, \text{Re} \rho^+_2 + \text{Im} \left( \mathcal{F}_P \mathcal{F}^\ast_\perp \right) \, \text{Im} \rho^-_2 \right] \,, \\
    && \langle I_6 \rangle_{-} = 0 \,, \\
    && \frac{3}{2} \langle I_7 \rangle_{-} = \text{Im} \left( \mathcal{F}_P \mathcal{F}^\ast_\Vert \right) \, \delta \rho \,, \\
    && \frac{3}{2} \langle I_8 \rangle_{-} = \frac{1}{2} \left[ \text{Re} \left( \mathcal{F}_P \mathcal{F}^\ast_\perp \right) \, \text{Im} \rho^+_2 - \text{Im} \left( \mathcal{F}_P \mathcal{F}^\ast_\perp \right) \, \text{Re} \rho^-_2 \right] \,, \label{I8vector} \\
    && \langle I_9 \rangle_{-} = 0 \,,
\end{eqnarray}

\begin{eqnarray}
    && \langle I_1 \rangle_{+} = \frac{1}{8} \left[ | \mathcal{F}_S |^2 \, \rho^-_{1,S} + \frac{2}{3} | \mathcal{F}_P |^2 \, \rho^-_1 + 2 | \mathcal{F}_\Vert |^2 \, \rho^-_1 + 2 | \mathcal{F}_\perp |^2 \, \rho^+_1 \right] \,, \\
    && \langle I_2 \rangle_{+} = -\frac{1}{8} \left[ | \mathcal{F}_S |^2 \, \rho^-_{1,S} + \frac{2}{3} \left\{ | \mathcal{F}_P |^2 \, \rho^-_1 - | \mathcal{F}_\Vert |^2 \, \rho^-_1 - | \mathcal{F}_\perp |^2 \, \rho^+_1 \right\} \right] \,, \\
    && \langle I_3 \rangle_{+} = \frac{1}{6} \left[ | \mathcal{F}_\perp |^2 \, \rho^+_1 - | \mathcal{F}_\Vert |^2 \, \rho^-_1 \right] \,, \\
    && \frac{2}{\pi} \langle I_4 \rangle_{+} = -\frac{1}{4} \text{Re} \left[ \mathcal{F}_S \mathcal{F}^\ast_\Vert  \left( (C_{9,S}-C_9')(C_9-C_9')^\ast+|C_{10}-C_{10}'|^2   \right) \right]  \,, \label{I4scalar} \\
     && \frac{2}{\pi} \langle I_5 \rangle_{+} = \frac{1}{2} \text{Re} \left[  \mathcal{F}_S \mathcal{F}^\ast_\perp \left( (C_{9,S}-C_9')(C_{10}+C_{10}')^\ast+(C_9+C_9')^\ast (C_{10}-C_{10}')  \right) \right]\, \\
    && \langle I_6 \rangle_{+} = - \frac{4}{3} \left[ \text{Re} \left( \mathcal{F}_\Vert \mathcal{F}^\ast_\perp \right) \, \text{Re} \rho^+_2 + \text{Im} \left( \mathcal{F}_\Vert \mathcal{F}^\ast_\perp \right) \, \text{Im} \rho^-_2 \right] \,, \\
    && \frac{2}{\pi} \langle I_7 \rangle_{+} = \text{Im} \left( \mathcal{F}_S \mathcal{F}^\ast_\Vert \right) \, \delta \rho \,, \\
    && \frac{2}{\pi} \langle I_7 \rangle_{+} = \frac{1}{2}\text{Im} \left[ \mathcal{F}_S \mathcal{F}^\ast_\Vert \left( (C_{9,S}-C_9')(C_{10}-C_{10}')^\ast+(C_9+C_9')^\ast (C_{10}-C_{10}')  \right) \right]  \,, \\
    && \frac{2}{\pi} \langle I_8 \rangle_{+} = \frac{1}{2} \left[ \text{Re} \left( \mathcal{F}_S \mathcal{F}^\ast_\perp \right) \, \text{Im} \rho^+_2 - \text{Im} \left( \mathcal{F}_S \mathcal{F}^\ast_\perp \right) \, \text{Re} \rho^-_2 \right] \,, \\
    && \langle I_9 \rangle_{+} = \frac{2}{3} \left[ \text{Re} ( \mathcal{F}_\perp \mathcal{F}^\ast_\Vert ) \, \text{Im} \rho^+_2 + \text{Im} ( \mathcal{F}_\perp \mathcal{F}^\ast_\Vert ) \, \text{Re} \rho^-_2 \right] \,.
\end{eqnarray}


With some expressions corrected: 

\begin{eqnarray}
    && I_1 = \frac{1}{8} \left[ | \mathcal{F}_S|^2 \rho^-_{1,S}+2\text{Re}(\mathcal{F}_S\mathcal{F}_{P}^\ast ((C_{9,S}-C_9')(C_9-C_9')^\ast+|C_{10}-C_{10}'|^2)) \cos\theta_{P_1} + \cos^2\theta_{P_1} |\mathcal{F}_{P} |^2 \, \rho^-_1 + \frac{3}{2} \sin^2 \theta_{P_1} \left\{ | \mathcal{F}_\Vert |^2 \, \rho^-_1 + | \mathcal{F}_\perp |^2 \, \rho^+_1 \right\} \right] \\
    && \qquad\qquad\qquad \stackrel[]{SM}{\to} \frac{1}{8} \biggl\{ \left[ \cos^2 \theta_{P_1}| \mathcal{F}_{P} |^2 + \frac{3}{2} \sin^2 \theta_{P_1} \left\{ | \mathcal{F}_\Vert |^2 + | \mathcal{F}_\perp |^2 \right\} \right] \, | C_9^{\rm eff} |^2 \\
    &&+|\mathcal{F}_S|^2 | C_{9,S} |^2+2\text{Re}\{\mathcal{F}_S \mathcal{F}_{0,P}^\ast C_{9,S}C_9^{\rm eff \ast}  \}\biggr\}\,, \nonumber\\
    && I_2 = -\frac{1}{8} \left[ | \mathcal{F}_S|^2 \rho^-_{1,S}+2\text{Re}(\mathcal{F}_S\mathcal{F}_{P}^\ast ((C_{9,S}-C_9')(C_9-C_9')^\ast+|C_{10}-C_{10}'|^2)) \cos\theta_{P_1} + \cos^2\theta_{P_1} |\mathcal{F}_{P} |^2 \, \rho^-_1 - \frac{1}{2} \sin^2 \theta_{P_1} \left\{ | \mathcal{F}_\Vert |^2 \, \rho^-_1 + | \mathcal{F}_\perp |^2 \, \rho^+_1 \right\} \right] \\
    && \qquad\qquad\qquad \stackrel[]{SM}{\to} -\frac{1}{8}\biggl\{ \left[ \cos^2 \theta_{P_1}| \mathcal{F}_{P} |^2 - \frac{1}{2} \sin^2 \theta_{P_1} \left\{ | \mathcal{F}_\Vert |^2 + | \mathcal{F}_\perp |^2 \right\} \right] \, | C_9^{\rm eff} |^2 \\
     &&+|\mathcal{F}_S|^2 | C_{9,S} |^2+2\text{Re}\{\mathcal{F}_S \mathcal{F}_{0,P}^\ast C_{9,S}C_9^{\rm eff \ast}  \}\biggr\}\,, \nonumber\\ 
    && I_3 = \frac{1}{8} \left[ | \mathcal{F}_\perp |^2 \, \rho^+_1 - | \mathcal{F}_\Vert |^2 \, \rho^-_1 \right] \, \sin^2 \theta_{P_1} \stackrel[]{SM}{\to} \frac{1}{8} \left[ | \mathcal{F}_\perp |^2 - | \mathcal{F}_\Vert |^2 \right] \, \sin^2 \theta_{P_1} \, | C_9^{\rm eff} |^2 \,, \\
    && I_4 = -\frac{1}{4} \cos\theta_{P_1} \text{Re} ( \mathcal{F}_P \mathcal{F}^\ast_\Vert ) \, \rho^-_1 \, \sin \theta_{P_1} \\
    && -\frac{1}{4}\text{Re}\bigl[\mathcal{F}_S \mathcal{F}^\ast_\Vert \bigl( (C_{9,S}-C_9')(C_9-C_9')^\ast+|C_{10}-C_{10}'|^2 \bigr) \bigr]\, \sin \theta_{P_1}\\
   && \stackrel[]{SM}{\to} -\frac{1}{4} \text{Re} ( \mathcal{F}_P \mathcal{F}^\ast_\Vert ) \, \cos\theta_{P_1}\sin \theta_{P_1} \, | C_9^{\rm eff} |^2 -\frac{1}{4} \text{Re}(\mathcal{F}_S \mathcal{F}^\ast_\Vert C_{9,S}C_9^\ast)\sin \theta_{P_1} \,, \\
    && I_5 = \cos\theta_{P_1} \sin\theta_{P_1} \frac{3}{2}\langle I_5 \rangle_{-}+\sin\theta_{P_1}\frac{2}{\pi}\langle I_5 \rangle_{+} \stackrel[]{SM}{\to} 0 \,, \\
    && I_6 = - \left[ \text{Re} \left( \mathcal{F}_\Vert \mathcal{F}^\ast_\perp \right) \, \text{Re} \rho^+_2 + \text{Im} \left( \mathcal{F}_\Vert \mathcal{F}^\ast_\perp \right) \, \text{Im} \rho^-_2 \right] \, \sin^2 \theta_{P_1} \stackrel[]{SM}{\to} 0 \,, \\
    && I_7 = \cos\theta_{P_1} \sin\theta_{P_1} \frac{3}{2}\langle I_7 \rangle_{-}+\sin\theta_{P_1}\frac{2}{\pi}\langle I_7 \rangle_{+} \stackrel[]{SM}{\to} 0  \,, \\
    && I_8 = \frac{1}{2} \left[ \text{Re} \left( \mathcal{F}_0 \mathcal{F}^\ast_\perp \right) \, \text{Im} \rho^+_2 - \text{Im} \left( \mathcal{F}_0 \mathcal{F}^\ast_\perp \right) \, \text{Re} \rho^-_2 \right] \, \sin \theta_{P_1} \stackrel[]{SM}{\to} - \frac{\text{Im} \left( \mathcal{F}_0 \mathcal{F}^\ast_\perp \right)}{2} \sin \theta_{P_1} \, | C_9^{\rm eff} |^2 \,, \label{I8fact} \\
    && I_9 = \frac{1}{2} \left[ \text{Re} ( \mathcal{F}_\perp \mathcal{F}^\ast_\Vert ) \, \text{Im} \rho^+_2 + \text{Im} ( \mathcal{F}_\perp \mathcal{F}^\ast_\Vert ) \, \text{Re} \rho^-_2 \right] \, \sin^2 \theta_{P_1} \stackrel[]{SM}{\to} \frac{\text{Im} ( \mathcal{F}_\perp \mathcal{F}^\ast_\Vert )}{2} \sin^2 \theta_{P_1} \, | C_9^{\rm eff} |^2 \,,
    \label{Isfact}
\end{eqnarray}



\begin{table}[]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline 
    $\sqrt{q^2}$-bin $r$ & $\Gamma^r$ (SM+NP) & $\int \langle I_5 \rangle_{+}^r$ (\%) & $\int \langle I_5 \rangle_{-}^r$ (\%) & $\int \langle I_7 \rangle_{+}^r$ (\%) & $\int \langle I_6 \rangle_{+}^r$ (\%) \\
    %\cline{3-6}
    %& & \multicolumn{4}{c|}{$ [10^{-2}] $} \\
    \hline 
   %%$ r^{({\rm low})} $ & $0.08 + 0.09|\tilde{C}_{10}|^2$       & $0.5$ & $-0.5$  &$-0.5$ &$-0.4$\\ 
   %%$ r^{(\eta)} $ &     $ 0.03+  0.02|\tilde{C}_{10}|^2  $     & $0.2$ &  $-0.2$   &$-0.2$&$-0.2$\\ 
   %%$ r^{(\rho: {\rm inf})} $ & $1.09+  0.11|\tilde{C}_{10}|^2$ & $1.8$ &  $0.7$ &    $-2.4$&$1.0$\\
   $ r^{(\rho: {\rm sup})} $ & $0.59+ 0.10 \, |\tilde{C}_{10}|^2$  & $-0.2$&  $2.8$ &$ -0.003$&$3.8$ \\ 
   $ r^{(\phi: {\rm inf})} $ & $1.00+ 0.04 \, |\tilde{C}_{10}|^2 $ & $0.8$&  $-0.7$&$  0.9$&$-1.1$\\
   $ r^{(\phi: {\rm sup})} $ & $0.85+ 0.03 \, |\tilde{C}_{10}|^2$  & $0.04$& $1.1$ &$  -0.2$&$1.7$\\
   %%$ r^{({\rm high})} $  &     $0.01+ 0.03|\tilde{C}_{10}|^2$  & $-0.07$& $0.17$ &  $-0.008$&$ 0.3$\\
       \hline
    \end{tabular}
    \caption{\rd{To be removed}The decay rate in the presence of NP and observables that vanish in the SM, here calculated for $C_9'=C_{10}'=C_9^{\rm NP}=0$ and non-zero $C_{10}$. The cases $\braket{I_5}_+$ and $\braket{I_7}_+$ are sensitive to the SM-NP interference in the presence of the $S$-wave. Instead, $\braket{I_5}_-$ and $\braket{I_6}_+$ are sensitive to the SM-NP interference through the $P$-wave, while $\braket{I_7}_-$ approximately vanishes. The same overall multiplicative factor shown in the caption of Tab.~\ref{gammas,i2} applies; additionally, the four last columns are multiplied by $ \tilde{C}_{10} $. [\rd{give at most two digits; can you provide for inner use unbinned plots of the angular observables as a function of $q^2$?}]}
    \label{NPobsevablesold}
\end{table}

==> angularObservablesModified.tex <==
\section{Modification of angular observables in the absence of $C_9$ in the SM in presence of S-wave}

We are interested in how the angular observables change in the presence of the S-wave resonance. As discussed, when only one factorisable contribution, namely through vector resonances (what we called W-type), is sizeable then we can identify an effective $C_9$ operator. When a second contribution is significant (J-type), as is the case in D decays, then under some assumptions we can replace the W- and J- type with an approximate modified W $W_{mod}$, for which the branching ratios deviate from the full expression by no more than 40\% in the high-$q^2$ region. Once we introduce the scalar resonance, we see that this proceeds only through the W-type factorisation. Hence it can either be grouped with the $W$ from the vector part, and then the $J$ is left out, or we remain with a $W$ from the scalar contribution and a $W_mod$ from the vector contributions. In any case we cannot write a single effective $C_9$.

To examine the forms of the angular observables, we resort to their original definitions as quantities from the integration of the $d^5\Gamma$ over different kinematical variables. For example,

$$\frac{d^3\Gamma}{dq^2 dp^2 d\cos\theta_P}=2I_1-\frac{2}{3}I_2$$
We ignore NP contributions and focus on the long-distance ones. With a $C_9$ the above quantity would be, according to the equations before \ref{Isfact},
$$ \frac{d^3\Gamma}{dq^2 dp^2 d\cos\theta_P} =\frac{1}{3}\left[ | \mathcal{F}_0 |^2 \,  + \sin^2 \theta_{P} \left\{ | \mathcal{F}_\Vert |^2 \, + | \mathcal{F}_\perp |^2 \,  \right\} \right]\rho_1=\frac{1}{3}\left[ | \mathcal{F}_0 |^2 \,  + \sin^2 \theta_{P} \left\{ | \mathcal{F}_\Vert |^2 \, + | \mathcal{F}_\perp |^2 \,  \right\} \right]|C_9^{eff}|^2 $$

Now modifying accordingly Babar's notation we get the correct expression 

$$ \frac{d^3\Gamma}{dq^2 dp^2 d\cos\theta_P} =\frac{1}{3}\left[ | \mathcal{F}_{0,W} W(q^2) +\mathcal{F}_{0,J}J(q^2) |^2 + \sin^2 \theta_{P} \left\{ | \mathcal{F}_{\Vert,W} W(q^2) +\mathcal{F}_{\Vert,J}J(q^2) |^2 + | \mathcal{F}_{\perp,W} W(q^2) +\mathcal{F}_{\perp,J}J(q^2) |^2 \right\} \right] $$
If instead we choose to use a modified $W$ for the P-wave, despite this introducing a small deviation at some regions, then separating the S- and P- wave the above expression becomes  
$$ \frac{d^3\Gamma}{dq^2 dp^2 d\cos\theta_P} =\frac{1}{3}\left[ | \mathcal{F}_S W(q^2) +\mathcal{F}_{0,P}\cos\theta_{P}W_{mod}^2(q^2) |^2 \,  + \sin^2 \theta_{P} \left\{ | \mathcal{F}_\Vert |^2 W_{mod}^2(q^2) \, + | \mathcal{F}_\perp |^2 W_{mod}^2(q^2) \right\} \right] $$

The above modifications also apply individually to the observables $I_1, I_2, I_3$, for which the $\rho_1^+$ and $\rho_1^-$ are replaced by the $W$ and $J$'s inside the $\mathcal{F}$'s. 

\begin{equation}
    \begin{aligned}
      I_3 = \frac{1}{8} \biggl\{\left[ | \mathcal{F}_\perp |^2 \, \rho^+_1 - | \mathcal{F}_\Vert |^2 \, \rho^-_1 \right]  
      + \left[ (| \mathcal{F}_{\perp,J} |^2 - | \mathcal{F}_{\Vert,J} |^2) \, |C_J|^2 \right] \\
      +2\left[ \text{Re}((C_9+C_9')C_J^*\mathcal{F}_\perp\mathcal{F}_{\perp,J})-\text{Re}((C_9-C_9')C_J^*\mathcal{F}_\Vert \mathcal{F}_{\Vert,J}) \right]\,\biggr\} \sin^2 \theta_{P_1}
    \end{aligned}
\end{equation}

\paragraph{Example: $I_4$}
\begin{equation}
    (I_4 = -\frac{1}{4} \text{Re} \left( (\mathcal{F}_{0,W}W(q^2)+\mathcal{F}_{0,J}J(q^2)) (\mathcal{F}_{\Vert,W} W(q^2)+\mathcal{F}_{\Vert,J} J(q^2 ))^\ast \right) \,\sin \theta_{P_1})
\end{equation}

\begin{equation}
    \begin{aligned}
        I_4 = -\frac{1}{4} \text{Re} ( \mathcal{F}_0 \mathcal{F}^\ast_\Vert ) \, \rho^-_1 \, \sin \theta_{P_1} 
        -\frac{1}{4} \text{Re} ( \mathcal{F}_{0,J} \mathcal{F}^\ast_{\Vert,J} )|C_J|^2 \sin \theta_{P_1} \\
        -\frac{1}{4} \bigl [\text{Re}(\mathcal{F}_{0} \mathcal{F}^\ast_{\Vert,J}+\mathcal{F}_{0,J} \mathcal{F}^\ast_{\Vert} )\text{Re}\bigl( (C_9-C_9')C_J^\ast  \bigr) 
        -\text{Im}(\mathcal{F}_{0} \mathcal{F}^\ast_{\Vert,J}-\mathcal{F}_{0,J} \mathcal{F}^\ast_{\Vert})\text{Im}\bigl( (C_9-C_9')C_J^\ast  \bigr) \bigr] \sin \theta_{P_1} 
    \end{aligned}
\end{equation}

The expression for the separable scalar-vector interference effect is 
\begin{equation}
\frac{2}{\pi} \int^{+1}_{-1} d \cos \theta_{P_1} I_4 = -\frac{1}{4} \text{Re} \left\{ \mathcal{F}_S W(q^2) (\mathcal{F}_{\Vert,W} W(q^2)+\mathcal{F}_{\Vert,J} J(q^2 ))^\ast \right\}
\end{equation}
or
\begin{equation}
\frac{2}{\pi} \int^{+1}_{-1} d \cos \theta_{P_1} I_4 = -\frac{1}{4} \text{Re} \left\{ \mathcal{F}_S W(q^2) (\mathcal{F}_{\Vert} W_{mod}(q^2))^\ast \right\}
\end{equation}
$\mathcal{F}_{\Vert}=\mathcal{F}_{\Vert,W}\sim A_1(q^2),\,  \mathcal{F}_{\Vert,J}\sim A_1(p^2)$



\paragraph{Null-test observables $I_{5,6,7}$}

The observables $I_5, I_6, I_7$ are zero for zero $C_{10}, C_9',C_{10}'$.These observables all come from interference terms such as
$$ Re(\mathcal{M}_{LD}(\mathcal{M}_{SD}^{10})^*) $$
(see Cappiello et al.) The $Q_{10}$ matrix element has the long-distance structure of the W-type contribution. According to the single-factorisation scheme, it would be 
$$ I_5, I_6, I_7 \sim Re(C_9^{eff}C_{10}^*)$$

In the presence of $\sigma$ and the second factorisation option these observables become
%\begin{align}
%    I_5 =  \text{Re} \left[ (\mathcal{F}_{0,W}W+\mathcal{F}_{0,J}J) (\mathcal{F}_{\perp,W}C_{10}) ^\ast + \mathcal{F}_{0,W} C_{10} (\mathcal{F}_{\perp,W}W+\mathcal{F}_{\perp,J} J)^\ast  \right] %\sin \theta_{P_1}  
   % + \text{Im} \left( \mathcal{F}_0 \mathcal{F}^\ast_\perp \right) \, \text{Im} \rho^-_2 \right] \, \sin \theta_{P_1}
%   \\
%   I_6 =  -\text{Re} \left[ (\mathcal{F}_{\Vert ,W}W+\mathcal{F}_{\Vert,J}J) (\mathcal{F}_{\perp,W}C_{10}) ^\ast + \mathcal{F}_{\Vert ,W} C_{10} (\mathcal{F}_{\perp,W}W+\mathcal{F}_{\perp,J} J)^\ast  \right] \sin^2 \theta_{P_1} \\
%   I_7 =  \text{Im} \left[ (\mathcal{F}_{0,W}W+\mathcal{F}_{0,J}J) (\mathcal{F}_{\Vert,W}C_{10}) ^\ast + \mathcal{F}_{0,W} C_{10} (\mathcal{F}_{\Vert,W}W+\mathcal{F}_{\Vert,J} J)^\ast  \right] \sin \theta_{P_1} 
%\end{align}

\begin{eqnarray*}
    && I_5 = \left[ \text{Re} \left( \mathcal{F}_0 \mathcal{F}^\ast_\perp \right) \, \text{Re} \rho^+_2 + \text{Im} \left( \mathcal{F}_0 \mathcal{F}^\ast_\perp \right) \, \text{Im} \rho^-_2 \right] \, \sin \theta_{P_1} \,\\
    &&+\frac{1}{2}\bigl[ \text{Re} \left( \mathcal{F}_{0,W} \mathcal{F}^\ast_{\perp,J} \right)   \text{Re} \left((C_{10}-C_{10}') C_J^*) \right)+ \text{Re} \left( \mathcal{F}_{0,J} \mathcal{F}^\ast_{\perp,W} \right)   \text{Re} \left((C_{10}+C_{10}') C_J^*)   \right)    \, \\
    &&+ \text{Im} \left( \mathcal{F}_{0,W} \mathcal{F}^\ast_{\perp,J} \right)   \text{Im} \left((C_{10}'-C_{10}) C_J^*) \right)+ \text{Im} \left( \mathcal{F}_{0,J} \mathcal{F}^\ast_{\perp,W} \right)   \text{Im} \left((C_{10}+C_{10}') C_J^*)   \right) \bigr] \, \sin \theta_{P_1}    \,, \\
    && I_6 = - \left[ \text{Re} \left( \mathcal{F}_\Vert \mathcal{F}^\ast_\perp \right) \, \text{Re} \rho^+_2 + \text{Im} \left( \mathcal{F}_\Vert \mathcal{F}^\ast_\perp \right) \, \text{Im} \rho^-_2 \right] \, \sin^2 \theta_{P_1}  \, \\
    &&-\frac{1}{2} \bigl[  \text{Re} \left( \mathcal{F}_{\Vert,W} \mathcal{F}^\ast_{\perp,J} \right)   \text{Re} \left((C_{10}-C_{10}') C_J^*) \right)+ \text{Re} \left( \mathcal{F}_{\Vert,J} \mathcal{F}^\ast_{\perp,W} \right)   \text{Re} \left((C_{10}+C_{10}') C_J^*)   \right)   \, \\
    &&+  \text{Im} \left( \mathcal{F}_{\Vert,W} \mathcal{F}^\ast_{\perp,J} \right)   \text{Im} \left((C_{10}'-C_{10}) C_J^*) \right)+ \text{Im} \left( \mathcal{F}_{\Vert,J} \mathcal{F}^\ast_{\perp,W} \right)   \text{Im} \left((C_{10}+C_{10}') C_J^*)   \right) \bigr]  \, \sin^2 \theta_{P_1}     \,, \\
    && I_7 = \text{Im} ( \mathcal{F}_0 \mathcal{F}^\ast_\Vert ) \, \delta \rho \, \sin \theta_{P_1}   \, \\
    &&+\frac{1}{2}\bigl[ \text{Im} \left( \mathcal{F}_{0,J} \mathcal{F}^\ast_{\Vert,W} \right) \text{Re} \left(C_J (C_{10}-C_{10}')^*\right)+\text{Im} \left( \mathcal{F}_{0,W} \mathcal{F}^\ast_{\Vert,J} \right) \text{Re} \left(C_J (C_{10}-C_{10}')^*\right) \\
    &&  +   \text{Re} \left( \mathcal{F}_{0,J} \mathcal{F}^\ast_{\Vert,W} \right) \text{Im} \left(C_J (C_{10}-C_{10}')^*\right)-\text{Re} \left( \mathcal{F}_{0,W} \mathcal{F}^\ast_{\Vert,J} \right) \text{Im} \left(C_J (C_{10}-C_{10}')^*\right)\bigr]\sin \theta_{P_1}
\end{eqnarray*}


\paragraph{Example: $I_8$}
Under the presence of the J-type contribution, the relation \ref{I8fact} is modified to 
\begin{equation*}
I_8 = \frac{1}{2} \left[ \text{Re} \left( (\mathcal{F}_{0,W}W+\mathcal{F}_{0,J}J) (\mathcal{F}_{\perp,W} W +\mathcal{F}_{\perp,J} J) ^\ast \right) \, \text{Im} \rho^+_2 \\
- \text{Im} \left( (\mathcal{F}_{0,W}W+\mathcal{F}_{0,J}J) (\mathcal{F}_{\perp,W} W +\mathcal{F}_{\perp,J} J)^\ast \right) \, \text{Re} \rho^-_2 \right] \, \sin \theta_{P_1} 
\end{equation*}

Assuming there are no NP terms, we are left with 
\begin{equation}
    I_8 =- \frac{1}{2} \left[ \text{Im} \left( (\mathcal{F}_{0,W}W+\mathcal{F}_{0,J}J) (\mathcal{F}_{\perp,W} W +\mathcal{F}_{\perp,J} J)^\ast \right) \, \text{Re} \rho^-_2 \right] \, \sin \theta_{P_1} 
\end{equation}

Note that if there was only a W-type contribution, as implicitly assumed in the factorisation expressions usually given, then the $I_8$ would be zero without the S-wave transversity form factor. In other words, the SM value for $I_8$ in the absence of the $\sigma$ resonance would be zero. However, when the J contribution is present, there is a non-vanishing $I_8$ distribution that comes from the interference of $J(q^2)$ and $W(q^2)$, which do have different phases; this is also lost when approximating the $W$ and $J$ with a modified $W$. Moreover, after the integration over the dihadron angle as defined in eq. \ref{I8vector}, which gets rid of the S-wave dependence and only includes the P-wave interference with itself, this $I_8$ would be zero in the absence of a $J$ carrying phases. This means that even if a non-zero $<I_8>$ is found experimentally, this is not necessarily a sign of NP. As we will see in the numerical results section, the contribution to the $<I_8>$ from the $J-W$ interference is much smaller than the scales typically appearing in the other angular observables; however, this could change if we include a better estimation of the hadronic phases [namely, we need to check what if J carries a $\rho$ phase different from the one in W. But also the main suppression comes from the fact that the form factors have very similar constants. Would a better estimation of the poles change things?? ]

This angular observable is the only one for which a non-vanishing value within the SM [in some bin of $p^2,q^2,\theta_h$] urges us to include the $\sigma$ contribution or the $J-$type one (see numerical results furher below).
However, because the $A_1, A_2, V$ form factors of $D\rightarrow\rho$ have numerically very similar parameters (poles and values at $k^2=0$), it turns out that the $I_8$ from vector-vector interference is very close to zero (see appendix for details).
\\
(what I want to say is: \\W and sigma : non-vanishing  \\
W and J, no sigma : non-vanishing \\
W and J become Wmod, no sigma : 0 \\
W and J become Wmod and sigma : non-vanishing but we are missing the J-W interference, although I should check better if that is compensated for)


\section{$I_8$}
\begin{equation}
    I_8(\text{vector-vector})=|W||J|\sin{(\delta_W-\delta_J)}\bigl[a_1 (A_1(q^2)V(p^2)- A_1(p^2)V(q^2))+a_2 (A_2(q^2)V(p^2)- A_2(p^2)V(q^2))  \bigr]
\end{equation}
 where 
 \begin{align*}
     a_1\sim (m_D^2-p^2-q^2)(m_D+m_\rho) \\
     a_2\sim \frac{-4m_D^2 p_{\pi\pi}^2}{m_D+m_\rho}
 \end{align*}
 $$ A_i(k^2)=\frac{h_{Ai}}{1-\frac{k^2}{m_{Ai}^2}} $$
 and $m_{A1}=m_{A2}\approx m_{V}\approx 2.5 GeV$ which is very close to the maximal values allowed for $p^2$ and $q^2$.

\section{Issue with too many phases in S-wave null tests}

\begin{eqnarray}
     && \frac{2}{\pi} \langle I_5 \rangle_{+} = \frac{1}{2} \text{Re} \left[  \mathcal{F}_S \mathcal{F}^\ast_\perp \left( (C_{9}^{{\rm eff}: S}+C_9^{\rm NP}-C_9')(C_{10}+C_{10}')^\ast \right. \right. \\
     && \quad \left. \left. +(C_{9}^{{\rm eff}: P}+C_9^{\rm NP}+C_9')^\ast (C_{10}-C_{10}')  \right) \right] \stackrel[]{SM}{\to} 0\, \\
     \sim \text{Re} \left[  \mathcal{F}_S \mathcal{F}^\ast_\perp \left( C_{9}^{{\rm eff}: S}C_{10}^\ast +C_{9}^{{\rm eff}: P}^\ast C_{10}'  \right) \right] \\
     \sim \text{Re} \left[  \mathcal{F}_S \mathcal{F}^\ast_\perp e^{i(\delta_{\sigma \rho}-\delta_{10})} (c_\rho^S ... + c_\omega^S e^{-i\Delta_3}+...e^{-i\Delta_4} )|C_{10}|\right] +\\
          \text{Re} \left[  \mathcal{F}_S \mathcal{F}^\ast_\perp e^{i(-\delta_{\rho \rho}+\delta_{10})}  (c_\rho^P* ... + c_\omega^P* e^{i\Delta_2}+...e^{i\Delta_2} )|C_{10}|\right] \\
    \sim \cos(\delta_{\sigma \rho}-\delta_{10})Re[...]-sin... Re[...]+\cos(-\delta_{\rho \rho}+\delta_{10})Re[...]...-sin(-\delta_{\rho \rho}+\delta_{10})Im[...]
\end{eqnarray}
so they can be calculated in principle, it's just that I haven't. But also they can't be calculated by setting the phases to specific numbers such as in the cases of the other observables. We also have to set modW=0 or modWsigma=0 one at a time. 


\section{Expressions for $<S>$}
 \begin{eqnarray}
    %&& \langle S_1 \rangle \equiv \frac{1}{2} \left( \langle I_1 \rangle +/- \langle \overline{I}_1 \rangle \right) = \,, \\
    && \langle S_2 \rangle_{(p^2, q^2)} \equiv \frac{1}{2} \left( \langle I_2 \rangle_{+} + \langle \overline{I}_2 \rangle_{+} \right) \stackrel[]{SM}{\to} -\frac{1}{8} \left[ | \mathcal{F}_S |^2 + \frac{2}{3} \left\{ | \mathcal{F}_P |^2 - | \mathcal{F}_\Vert |^2 - | \mathcal{F}_\perp |^2 \right\} \right] \times | C_{9,P}^{\rm eff}|^2_{\rm CP-even} \,, \\
    && \langle S_3 \rangle_{(p^2, q^2)} \equiv \frac{1}{2} \left( \langle I_3 \rangle_{+} + \langle \overline{I}_3 \rangle_{+} \right) \stackrel[]{SM}{\to} \frac{1}{6} \left[ | \mathcal{F}_\perp |^2 - | \mathcal{F}_\Vert |^2 \right] \times | C_{9,P}^{\rm eff}|^2_{\rm CP-even} \,, \\
    && \langle S_4 \rangle_{(p^2, q^2)} \equiv \frac{1}{2} \left( \langle I_4 \rangle_{-} + \langle \overline{I}_4 \rangle_{-} \right) \stackrel[]{SM}{\to} -\frac{1}{6} \text{Re} \left( \mathcal{F}_P \mathcal{F}^\ast_\Vert \right) \times | C_{9,P}^{\rm eff}|^2_{\rm CP-even} \,, \\
    && \langle S_5 \rangle_{(p^2, q^2)} \equiv \frac{1}{2} \left( \langle I_5 \rangle_{-} - \langle \overline{I}_5 \rangle_{-} \right) \stackrel[]{SM}{\to} 0 \,, \\
    && \langle S_6 \rangle_{(p^2, q^2)} \equiv \frac{1}{2} \left( \langle I_6 \rangle_{+} - \langle \overline{I}_6 \rangle_{+} \right) \stackrel[]{SM}{\to} 0 \,, \\
    && \langle S_7 \rangle_{(p^2, q^2)} \equiv \frac{1}{2} \left( \langle I_7 \rangle_{-} + \langle \overline{I}_7 \rangle_{-} \right) \stackrel[]{SM}{\to} 0 \,, \\
    && \langle S_8 \rangle_{(p^2, q^2)} \equiv \frac{1}{2} \left( \langle I_8 \rangle_{-} - \langle \overline{I}_8 \rangle_{-} \right) \stackrel[]{SM}{\to} -\frac{1}{6} \text{Im} \left( \mathcal{F}_P \mathcal{F}^\ast_\perp \right) \times | C_{9,P}^{\rm eff}|^2_{\rm CP-even} \stackrel[]{SM}{\to} 0\,, \\
    && \langle S_9 \rangle_{(p^2, q^2)} \equiv \frac{1}{2} \left( \langle I_9 \rangle_{+} - \langle \overline{I}_9 \rangle_{+} \right) \stackrel[]{SM}{\to} \frac{1}{3} \text{Im} ( \mathcal{F}_\perp \mathcal{F}^\ast_\Vert ) \times | C_{9,P}^{\rm eff}|^2_{\rm CP-even}\stackrel[]{SM}{\to} 0 \,,
\end{eqnarray}
For $A$, just replace $ | C_{9,P}^{\rm eff}|^2_{\rm CP-even} \to | C_{9,P}^{\rm eff}|^2_{\rm CP-odd} $. In the current work we neglect CP-odd contributions from the SM, hence all the $A$ observables vanish and all our $\braket{I}$ observables coincide with their respective $\braket{S}$ counterparts.

==> comparison_with_DeBoer_Hiller_Cappiello_CPV.tex <==
\subsection{Summary $ D^0 \to P^+ P^- \ell^+ \ell^- $, Cappiello et al.}

[comment on bremsstrahlung][note that CP asymmetry in $ K_L \to \pi^+ \pi^- e^+ e^- $ of $ 14\% $ ``is so large because the CP violating amplitude is enhanced by kinematic bremsstrahlung factors'', Bigi and Sanda textbook]

[Zweig violation is discussed for instance in \cite{Donoghue:1990xh}; it should be good enough for low invariant masses of the pion pair]





\subsection{Summary $ D^0 \to P^+ P^- \ell^+ \ell^- $, De Boer and Hiller}

They follow factorization as Cappiello et al. do, but with some differences. For the decays $D\rightarrow\pi\pi ll$ they use just $<\pi\pi|(\overline{u}c)_{V-A}|D^0><ll|a(\overline{l}l)_V|0>$, i.e. assume that the lepton pair comes from the vacuum. Cappiello et al. also include the contribution of  $<\pi\pi|(\overline{d}d)_{V-A}|0><ll|(\overline{u}c)_{V-A}|D^0>$ (later Hiller et al. comment that this effect is small and that they include some part of this contribution in the parameters that are fitted phenomenologically). For the decays $D\rightarrow KK ll$ they only consider $<KK|(\overline{s}s)_{V-A}|0><ll|(\overline{u}c)_{V-A}|D^0>$, which is the only option due to the suppression of rescattering (equivalent to the Zweig rule in this context), as stated also in Cappiello. 
\begin{itemize}
    \item For the hadronic part $<\pi\pi |(\overline{u}c)_{V-A}|D^0>$, they consider only the $\rho$ contribution, which they model with a modified Breit-Wigner line shape (with a Blatt-Weisskopf factor too) and typical form factors for $D\rightarrow \rho$. %[perhaps it is useful to compare their "normalisation factor" which comes with the helicities to the one that Babar provides]
    \item For the leptonic part $<ll|a(\overline{l}l)_V|0>$ in $D\rightarrow\pi\pi ll$ they model it as a $C_9$ contribution (this, I think, is not conceptually important: it is just a matter of notation), in which they include the line shape of the resonances (Breit-Wigner), a magnitude $a_\rho$ which is the same for $\rho$ and for $\omega$ and a different one for $a_\phi$, and two corresponding strong phases $\delta_\rho$ and $\delta_\phi$. Compared to Cappiello, they end up with more freedom in the strong phases, allowing for a different strong phase between $\rho$ and $\omega$ (on top of the phase coming from the propagators). Later they vary this relative phase $\delta_\rho-\delta_\phi$, stating that in the $SU(3)$ limit it would be equal to $\pi$.
    \item For the hadronic part in $D\rightarrow KK ll$, the $<KK|(\overline{s}s)_{V-A}|0>$ through $\phi$ comes with a Breit-Wigner propagator, but I don't see what is the equivalent of Cappiello's decay constant $<\phi|(\overline{s}s)_V|0>=f_\phi m_\phi \epsilon_\phi^*$ (the polarisation is OK, it gets absorbed later). \textit{Maybe} what happens is that this $f_\phi m_\phi$ is absorbed in the overall $a_\rho^{KK}$, i.e. this free parameter of the $C_9$ appearing in the $0\rightarrow ll$ part. 
    \item For the leptonic part in $D\rightarrow KK ll$, $<ll|(\overline{u}c)_{V-A}|D^0>$, they include the form factors for $D\rightarrow\rho$ normally and then a propagator coupling to $ll$, again replacing the whole (implied) process made explicit in Cappiello, $\rho\rightarrow\gamma\rightarrow ll$, with the effective $C_9$ parameters. 

\end{itemize}
    They also include the contributions from $\eta$ and $\eta'$ through an effective pseudoscalar operator, which however result in small effects [maybe to check: if the phase introduced with $\eta$ affects any observable; LVS: the eta is very narrow, I don't believe it gives an important contribution].

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Expressions derived according to Cappiello et al.}\label{app:brs}
We start from the expression for the squared amplitude:
\begin{equation}
    |\mathcal{M}|^2=\frac{2e^2}{q^4}|\xi|^2\sum_i |F_i|^2 T_{ii}+2Re\sum_{i<j}(F_i^* F_j)T_{ij}
\end{equation}
where \begin{equation}
    \begin{aligned}
        F_1= \frac{b_\rho(p^2) F_{Bl.-Weiss.}(p^2)}{P_\rho(p^2)} i q^2 
    \bigl[\sum_{V'}\frac{f_V'^2 e^{i\delta_{V'}}}{P_{V'}(q^2)} \bigl( \frac{2q\cdot(p_1-p_2)}{m_D+p}A_2(q^2)-(m_D+p)A_1(q^2)\bigr)\\
    +m_\rho f_\rho \sum_{V''}\frac{f_{V''} e^{i\delta_{V''}}}{m_{V''}P_{V''}(q^2)}\bigl( \frac{2q\cdot(p_1-p_2)}{m_D+q}A_2(p^2)-(m_D+q)A_1(p^2)\bigr)\bigr]\\
    +i q^2 \sum_{V'}\frac{f_V'^2 e^{i\delta_{V'}}}{P_{V'}(q^2)} \frac{a_s e^{i\phi_s}}{(1-\frac{q^2}{m_A^2})P_{Bugg}(p^2)}
    \end{aligned}
\end{equation}

\begin{equation}
    \begin{aligned}
        F_2= \frac{b_\rho(p^2) F_{Bl.-Weiss.}(p^2)}{P_\rho(p^2)} i q^2\bigl
    [\sum_{V'}\frac{f_V'^2 e^{i\delta_{V'}}}{P_{V'}(q^2)} \bigl( \frac{2q\cdot(p_1-p_2)}{m_D+p}A_2(q^2)+(m_D+p)A_1(q^2)\bigr)\\
    +m_\rho f_\rho \sum_{V''}\frac{f_{V''} e^{i\delta_{V'}}}{m_{V''}P_{V''}(q^2)}\bigl( \frac{2q\cdot(p_1-p_2)}{m_D+q}A_2(p^2)+(m_D+q)A_1(p^2)\bigr)\bigr] \\
     +i q^2 \sum_{V'}\frac{f_V'^2 e^{i\delta_{V'}}}{P_{V'}(q^2)} \frac{a_s e^{i\phi_s}}{(1-\frac{q^2}{m_A^2})P_{Bugg}(p^2)}
    \end{aligned}
\end{equation}

\begin{equation}
    F_3=\frac{b_\rho(p^2) F_{Bl.-Weiss.}(p^2)}{P_\rho(p^2)}  i q^2 \bigl[ \sum_{V'}\frac{f_V'^2 e^{i\delta_{V'}}}{P_{V'}(q^2)}\frac{-4 i V(q^2)}{m_D+p}+m_\rho f_\rho \sum_{V''}\frac{f_{V''} e^{i\delta_{V'}}}{m_{V''}P_{V''}(q^2)}\frac{-4 i V(p^2)}{m_D+q} \bigr]
\end{equation}

We have made the slight modification of taking the factor $\xi=C_2\lambda_{CKM}  e \frac{G_F}{\sqrt{2}}$ outside the $F$'s. We have also modified the $b_\rho$ to include the contribution of the $\omega$ resonance in the following way
\begin{equation}
    b_\rho(p^2)=b_{\rho,old} (1 + a_\omega\, e^{i \phi_\omega}\frac{p^2}{P_\omega(p^2)})
\end{equation}
according to the paper by BES and their further clarifications. To be consistent with them we have further introduced the Blatt-Weisskopf damping factor. The effect of $\sigma$ appears in the last lines of $F_1$ and $F_2$. The quantities $T_{ij}$, $i,j=1,2,3$ are given in Cappiello; they are kinematical factors which contain the dependencies on the kinematical variables $\theta_l$ and $\phi$.

We are firstly interested in the differential branching ratios with respect to $q^2, p^2$. We can then integrate the quantities $T_{ij}$ over $\theta_l,\phi$. We get that 
\begin{equation}
    \int T_{13} d\text{cos}\theta_l d\phi=\int T_{23} d\text{cos}\theta_l d\phi=0
\end{equation}
For reference we give the expressions for the quantities that affect the $\sigma$ contribution: 
\begin{equation}
\begin{aligned}
    \int T_{11} d\text{cos}\theta_l d\phi=-(1/(12 p^4)) \pi (-p^4 \beta_l^2 \lambda_D - 
   4 p^2 q^2 sin\theta_h^2 \beta_l^2 \lambda_h - 
   2 p^2 cos\theta_h \beta_l^2 \sqrt{\lambda_D}
     \sqrt{\lambda_h} (p^2 + q^2 - m_D^2) \\- 
   cos\theta_h ^2 \beta_l^2 \lambda_h (p^2 + q^2 - m_D^2)^2 + 
   3 (cos\theta_h \sqrt{\lambda_D \lambda_h} + 
      p^2 (p^2 + q^2 - m_D^2))^2 - 48 p^4 q^2 m_\pi^2)
      \end{aligned}
\end{equation}

\begin{equation}
\begin{aligned}
    \int T_{22} d\text{cos}\theta_l d\phi=-(1/(12 p^4)) \pi (-p^4 \beta_l^2 \lambda_D - 
   4 p^2 q^2 sin\theta_h^2 \beta_l^2 \lambda_h +
   2 p^2 cos\theta_h \beta_l^2 \sqrt{\lambda_D}
     \sqrt{\lambda_h} (p^2 + q^2 - m_D^2) \\- 
   cos\theta_h ^2 \beta_l^2 \lambda_h (p^2 + q^2 - m_D^2)^2 + 
   3 (cos\theta_h \sqrt{\lambda_D \lambda_h} - 
      p^2 (p^2 + q^2 - m_D^2))^2 - 48 p^4 q^2 m_\pi^2)
      \end{aligned}
\end{equation}

\begin{equation}\begin{aligned}
    \int T_{12} d\text{cos}\theta_l d\phi=
   1/(12 p^4) \pi (p^4 (-3 (p^4 - 6 p^2 q^2 + 
          q^4) + \beta_l^2 \lambda_D) + (3 p^4 + \beta_l^2\lambda_h cos^2\theta_h) m_D^2 (2 (p^2 + q^2) - m_D^2) \\- 
    48 p^4 q^2 m_\pi^2 + \lambda_h (3 \lambda_D cos^2\theta_h + \beta_l^2 (p^2 + q^2 + p^2 sin\theta_h - 
          q^2 sin\theta_h) (p^2 (-1 + sin\theta_h) - 
          q^2 (1 + sin\theta_h))))
\end{aligned}
\end{equation}
[There are better ways to write the above expressions]
The next step is to integrate over the angle $\theta_h$. This appears also in the dynamical components of the squared amplitude, namely in $F_1$ and $F_2$, through 
\begin{equation}
    q\cdot(p_1-p_2)=-\frac{\sqrt{\lambda_D}\sqrt{\lambda_h}}{2p^2}\cos\theta_h
\end{equation}

\section{Comparison with \cite{DeBoer:2018pdx}: "Experimental" fitting to the peaks}
[Appendix mostly for us]
Reference \cite{DeBoer:2018pdx} writes a $C_9^{eff}$ by making use of arbitrary factors in place of $2f_\rho^2$ and $\frac{\sqrt{2}f_\phi^2}{3}$, which are fixed by the values of the branching ratios close to the peaks of the respective resonances.  In here we make a comparison of the ratio of these so-called 'fudge' factors to the corresponding form factors. Since they fit to data around the resonance peaks, we want to see if our method, of including J and W, makes sense according to the LHCb measurements. We commented that including J and W in a single W-modified type introduces some errors, but should be sufficient near the peaks. Moreover, fig.\ref{withandwithoutJandWmod} shows that the inclusion of J should correct the W contribution by around a factor of two. If then we have only W or W-modified,for the equivalent 'fudge factors' that said reference uses we would get roughly what is shown in \ref{comparisontoG}.
\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    Factorisation used & Only $b_\rho$ & $b_\rho$ with $\omega$ included like in BES \\
    \hline
      only W    & $a_\rho=0.44\text{GeV}^2$, $a_\phi=0.21 \text{GeV}^2$ & $a_\rho=0.52\text{GeV}^2$, $a_\phi=0.24 \text{GeV}^2$ \\
      $W_{mod}$: including W and J & $a_\rho=0.88 \text{GeV}^2$, $a_\phi=0.21 \text{GeV}^2$   &  $a_\rho=1.03 \text{GeV}^2$, $a_\phi=0.24 \text{GeV}^2$\\
      \hline
    Experimental fitting \cite{DeBoer:2018pdx}& \multicolumn{2}{c}{$a_\rho\approx 0.7\text{GeV}^2$, $a_\phi\approx 0.3\text{GeV}^2$}  \\
      \hline
    \end{tabular}
    \caption{Comparison of fudge factors}
    \label{comparisontoG}
\end{table}
It is not clear what this comparison teaches us. Keep in mind that by fitting to the experimental data, by definition they do include the $\sigma$, which as we calculated gives a sizeable effect, especially in the $\phi$ resonance region; this could lead to the effective parameter $a_\phi$ being overestimated compared to the one coming only from $\rho$. 

\section{CP violation}
[appendix for temporary use]
Let's consider for a moment the description with the $C_9^{eff}$ coefficient, only for the P-wave.

$$ C_9 \sim e^{i\phi_\rho}\bigl(\frac{2 f_\rho^2}{P_{\rho}(q^2)}-\frac{2 f_\omega^2}{3 P_{\omega}(q^2)}\bigr)-e^{i\phi_\phi}\frac{\sqrt{2}f_\phi^2}{3P_{\phi}(q^2)}  $$
Here $\phi_\rho$ and $\phi_\phi$ are additional strong phases. Remember that the $\phi$ part comes from the $\overline{u}c\overline{s}s$ operator and thus carries $\lambda_s$. Since the $\lambda_d$ is carried outside, the correct form of $C_9$ is [not keeping CP-even part!]
\begin{align*}
    C_9 \sim e^{i\phi_\rho}\bigl(\frac{2 f_\rho^2}{P_{\rho}(q^2)}-\frac{2 f_\omega^2}{3 P_{\omega}(q^2)}\bigr)-\frac{\lambda_s}{\lambda_d}e^{i\phi_\phi}\frac{\sqrt{2}f_\phi^2}{3P_{\phi}(q^2)}\\
    \sim e^{i\phi_\rho}\bigl(\frac{2 f_\rho^2}{P_{\rho}(q^2)}-\frac{2 f_\omega^2}{3 P_{\omega}(q^2)}\bigr)+i r_{CKM}e^{i\phi_\phi}\frac{\sqrt{2}f_\phi^2}{3P_{\phi}(q^2)} \\
    \sim A_{\rho\omega}+i r_{CKM} A_\phi
\end{align*}
where $A_{\rho\omega}$ and $A_\phi$ carry strong phases. When considering the CP-conjugate process, in place of $C_9$ what appears is 
$$\overline{C_9} \sim A_{\rho\omega}-i r_{CKM} A_\phi$$
Probably what is considered by previous works is that $r_{CKM}<\mathcal{O}(10^{-3})$ hence 
$$ \overline{C_9}\approx C_9 $$
Now for the Wilson coefficients coming from NP, supposedly the CP-conjugate processes carry 
$$\overline{C_{10}}=C_{10}^\ast, \,\overline{C_{10}'}=C_{10}'^\ast,\,\overline{C_{9}'}=C_{9}'^\ast $$
so how do the effective WC parts transform under CP in eq. \ref{WCrhos} and above transform, and why are observables 1,2,3,4,7 called CP-even while 5,6,8,9 are considered CP-odd? Note that in the SM, $I_i$ for i=1,2,3,4,8,9 are CP-even and for i=5,6,7 they are just vanishing. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Towards better amplitude expressions}
\label{amplitude-expressions}




Perhaps it's better to avoid writing the resonances as asymptotic states, so 
\begin{equation}
    <\pi\pi ll|\mathcal{S}|D^0>= <\pi\pi ll|\frac{(-i)^3}{3}T\bigl\{\ \int d^4 x d^4 y d^4z \mathcal{H}_{had}(x)\mathcal{H}_{\gamma,had}(y)\mathcal{H}_{\gamma ll}(z)                \bigr\}|D^0>
\end{equation}

where 

\begin{eqnarray}
    \mathcal{H}_{had}(x)= C_2\frac{G_F}{\sqrt{2}}\bigl(\lambda_d (\overline{u}\gamma^\mu c_L)(\overline{d}\gamma_\mu d_L) (x)+\lambda_s (\overline{u}\gamma^\mu c_L)(\overline{s}\gamma_\mu s_L) (x)\bigr)\\
    \mathcal{H}_{\gamma,had}(y)= e A^\nu (y) \sum_{q=u,d,s}\overline{q}(y)\gamma_\nu q(y)\\
    \mathcal{H}_{\gamma ll}(z) = e A^\kappa (z) \overline{l}(z)\gamma_\kappa l(z)
\end{eqnarray}

\begin{equation}\begin{aligned}
    <\pi\pi ll|\mathcal{S}|D^0>\sim\int d^4 x <\pi\pi |(\overline{u}\gamma^\mu c_L)(x)|D^0>\int d^4 y d^4z <ll|(\lambda_d(\overline{d}\gamma_\mu d_L) (x)+\lambda_s (\overline{s}\gamma_\mu s_L) (x)) \mathcal{H}_{\gamma,had}(y)\mathcal{H}_{\gamma ll}(z)                |0> \\
+  \int d^4 x <\pi\pi |(\overline{d}\gamma^\mu d_L) (x)|0>\int d^4 y d^4z<ll|\lambda_d(\overline{u}\gamma_\mu c_L)(x)\mathcal{H}_{\gamma,had}(y)\mathcal{H}_{\gamma ll}(z) |D^0>\\
\equiv A_W + A_J
    \end{aligned}
    \label{WandJinampl}
\end{equation}

{\color{red} [Jaeger and Camalich \cite{Jager:2012uw} write for the hadronic amplitude

\begin{equation}
    -i \frac{e^2}{q^2} \, \int d^4 x \, e^{-i q \cdot x} \, \langle \ell^- \ell^+ | \left( \overline{l} \gamma^\mu l \right) (x) | 0 \rangle \, \int d^4 y \, e^{i q \cdot y} \, \langle \pi \pi | T \left\{ j^{\rm had}_{\mu, em} (y) \mathcal{H}^{\rm had}_{\rm eff} (0) \right\} | D^0 \rangle
\end{equation}
where $ j^{\rm had}_{\mu, em} = \Sigma_q e_q \overline{q} \gamma_\mu q $, $e_q$ in units of the electric charge $e$. {\color{blue} The $e^{-i q \cdot ( x-y)}$ and the $1/q^2$ are from the photon propagator. [LVS: hence, you are talking about momentum space, while your whole Hamiltonian is given in position space; why are you happy about not including these phase factors in the main text?]}  Also:

\begin{equation}
    \mathcal{H}^{\rm had}_{\rm eff} = \frac{4 G_F}{\sqrt{2}} \Sigma_{p=u, c} \lambda_p \left[ C_1 Q_1^p + C_2 Q_2^p + \Sigma_{i = 3 \ldots 6} C_i P_i + C_{8g} Q_{8g} \right]
\end{equation}
where

\begin{equation}
    Q_{8g} = \frac{g_s}{16 \pi^2} \hat{m}_b \overline{s} \sigma_{\mu \nu} P_R G^{\mu \nu} b
\end{equation}
and $P_i$ are penguin operators.]}

\section{Annihilation topology}
Because of $\sigma$ having $I=0$ (and being scalar) we can write  [\LVS{I disagree}]
\begin{equation}
\braket{\rho\sigma|(\overline{d}d)_{V-A}|0}=\braket{\rho|(\overline{d}d)_{V-A}|0}=-f_\rho m_\rho \epsilon^\ast_{\mu(\rho)}    
\end{equation}
(we define $\braket{\rho|\frac{1}{\sqrt{2}}T(1,0)|0}=f_\rho m_\rho\epsilon^\ast_{\mu(\rho)} $ and we have that $\overline{d}d=\frac{1}{\sqrt{2}}(-\ket{1 0}+\ket{0 0})$).
Then 
\begin{equation}
    Q_A =\braket{\rho\sigma|(\overline{d}d)_{V-A}|0}\braket{0|(\overline{u}c)_{V-A}|D^0}= -f_\rho m_\rho \epsilon^\ast_{\mu(\rho)}  f_D (p+q)^\mu
\end{equation}
The Lorentz index of the polarization is transferred to the lepton pair, so in the end we have 
\begin{equation}
    \braket{\pi\pi \ell\ell |\mathcal{H}|D}_{D\rightarrow 0\rightarrow \rho\sigma} \sim f_D f_\rho m_\rho (\overline{l}\gamma^\mu l)(p_\mu+q_\mu)    
    \end{equation}

Compare this to a generic form factor of a scalar to a vector meson: The only surviving term when contracted with $P^\mu$ from $\braket{0|j^\mu|D}$ is, similarly, 
\begin{equation}
    \frac{\epsilon^\ast \cdot (p+q)}{(p+q)^2} 2 m_\rho A_0 ((p+q)^2)\, (p+q)_\mu f_D\, (p+q)^\mu \approx  \epsilon^\ast \cdot (p+q) 2 m_\rho A_0 (0) f_D
\end{equation}
assuming a soft dependence on the momentum transfer of the $A_0$. Then again transferring the Lorentz index to the lepton pair we end up with 

\begin{equation}
    \braket{\pi\pi \ell\ell |\mathcal{H}|D}_{D\rightarrow 0\rightarrow \rho\sigma} \sim  2 m_\rho A_0 (0) f_D \, (\overline{l}\gamma^\mu l)(p_\mu+q_\mu)   
\end{equation}
A similar argument holds for $\omega\sigma$. Hence we see that the contribution of the annihilation topology with $V'\sigma$ to the form factor of Eq. \eqref{Dpipiff} lies in a modification of $w_+$ and of $r$. Since we anyway ignore the terms that come with $q_\mu$ (given that they yield contributions proportional to the mass of the lepton), the only important modification will be in the $w_+$ term; in any case, we parameterize the effect of the $\sigma$ with the term of Eq.~\eqref{eq:form_factor_S_wave}, which contains a constant $a_s$ that is fitted to the distribution over $p^2$, so the effect of this annihilation topology will be to some extent included in our calculation. A slight difference is found in the leptonic part that comes with it, since $Q_A$ is accompanied by 
\begin{equation}
    A(q^2)=\frac{f_\rho}{m_\rho P_\rho (q^2)}-\frac{f_\omega}{3 m_\omega P_\omega(q^2)}
\end{equation}
instead of the W-type factorization that comes also with $\phi$. [\LVS{Why can't you have a phi?, Zweig}][\LVS{the argument boils down to the decay constant of the charm-meson and the available kinematical structures from the intermediate resonances (the antisymmetric symbol won't contribute)}]

For the annihilation topologies $D\rightarrow 0 \rightarrow VV'$, the matrix element is now the one of the vectorial current: $\braket{VV'|\overline{d}\gamma^\mu d|0}$, and since it is contracted with $P_\mu$ the total topology term is multiplied by  $m_d-m_d=0$.

==> finalTablesFull.tex <==
******************************** Gammas ********************************************************************************
totalgamma= 0.0002835130275803663
gamma only sigma= 5.711026384489282e-05

at bfp:
q-binned gammas from Wmod, unnormalised=  [4.057228093218511e-05, 9.381913005624558e-05, 6.776439041004324e-05]

delta1=0.5Pi:
q-binned gammas from Wmod, unnormalised=  [4.513184574741862e-05, 9.968310609947472e-05, 6.282579285281884e-05]
delta1=0.9Pi:
q-binned gammas from Wmod, unnormalised=  [3.518545820659581e-05, 8.672378253875704e-05, 7.100025715617467e-05]
delta4=0.5Pi:
q-binned gammas from Wmod, unnormalised=  [4.519242997737774e-05, 0, 0]
delta4=0.2Pi:
q-binned gammas from Wmod, unnormalised=  [3.88889266027952e-05, 9.391803814296869e-05, 0]
delta3=-0.4Pi:
q-binned gammas from Wmod, unnormalised=  [4.146407899628424e-05, 9.445907810065883e-05, 6.674913523482495e-05]
delta3=1.2Pi:
q-binned gammas from Wmod, unnormalised=  [4.062719814751893e-05, 9.379159998624103e-05, 6.76739921059027e-05]
asrel=14:
q-binned gammas from Wmod, unnormalised=  [3.4012731870827504e-05, 9.202214290783417e-05, 6.591829085668096e-05]
asrel=22:
q-binned gammas from Wmod, unnormalised=  [4.567658723898041e-05, 9.521744362442377e-05, 6.920092925925069e-05]
bphis lower limit:
q-binned gammas from Wmod, unnormalised=  [4.1053990909901565e-05, 9.015000571148991e-05, 6.419012518156946e-05]


*********************** Gammas only sigma *************************************
at bfp:
q-binned gammas, only sigma unnormalised= [1.4497469214071648e-05, 3.971552415314518e-06, 4.080107623413947e-06]
asrel=14:
q-binned gammas, only sigma unnormalised=  [7.937902905010451e-06, 2.1745717618327933e-06, 2.2340145719927126e-06]
asrel=22:
q-binned gammas, only sigma unnormalised=  [1.9601769884395717e-05, 5.369869135136319e-06, 5.51664040509904e-06]
bphis lower limit:
q-binned gammas, only sigma unnormalised=  [1.4979169432620633e-05, 3.02425542155622e-07, 5.058457934007341e-07]
bphis upper limit:
q-binned gammas, only sigma unnormalised=  [1.4306225672698388e-05, 7.506484816729242e-06, 7.014930093389914e-06]
delta4=0.5Pi:
q-binned gammas, only sigma unnormalised=  [1.911761808289413e-05, 0, 0]
delta4=0.2Pi:
q-binned gammas, only sigma unnormalised=  [1.2814105191425611e-05, 4.07046118800036e-06, 0]
delta3=-0.4Pi:
q-binned gammas, only sigma unnormalised=  [1.5389264315132516e-05, 4.611506313018427e-06, 3.0648544578497925e-06]
delta3=1.2Pi:
q-binned gammas, only sigma unnormalised=  [1.455238687438776e-05, 3.944023053111183e-06, 3.989709889970612e-06]



***************** I2+ (vector+scalar), I3+ (vector), I4-(vector) ***************************)

at bfp:
q-binned i2, unnormalised=  [-6.706297459137457e-06, -4.572619870028666e-06, -3.600202525298e-06]
q-binned i2, only sigma, unnormalised=  [-4.866916350588552e-06, -1.3943002067668554e-06, -1.4344704565599745e-06]
q-binned i3, unnormalised=  [-3.1727938597381073e-06, -1.5071249428004084e-05, -1.0816919192512977e-05]
q-binned i4 vector, unnormalised=  [8.403675625430821e-06, 3.0767797054913124e-05, 2.1865698498075947e-05]

delta1=0.5Pi:
q-binned i2, unnormalised=  [-6.989379962030834e-06, -4.796337441513504e-06, -3.436413692451726e-06]
q-binned i2, only sigma, unnormalised=  [-4.866916350588552e-06, -1.3943002067668554e-06, -1.4344704565599745e-06]
q-binned i3, unnormalised=  [-3.7594014777870238e-06, -1.5988577465245418e-05, -1.0001709077643045e-05]
q-binned i4 vector, unnormalised=  [9.895858274987347e-06, 3.2766229379006875e-05, 2.0166257212884868e-05]
delta1=0.9Pi:
q-binned i2, unnormalised=  [-6.36134368200915e-06, -4.3060568015860905e-06, -3.7066821201083672e-06]
q-binned i2, only sigma, unnormalised=  [-4.866916350588552e-06, -1.3943002067668554e-06, -1.4344704565599745e-06]
q-binned i3, unnormalised=  [-2.4936186076678855e-06, -1.394914464045459e-05, -1.135755727486902e-05]
q-binned i4 vector, unnormalised=  [6.647229790001169e-06, 2.834706337399122e-05, 2.2980086079274815e-05]

asrel=14:
q-binned i2, unnormalised=  [-4.504207489315148e-06, -3.9417504516385e-06, -2.95115811647085e-06]
q-binned i2, only sigma, unnormalised=  [-2.6648186343488585e-06, -7.634311408242572e-07, -7.854246425473067e-07]
asrel=22:
q-binned i2, unnormalised=  [-8.419685129591085e-06, -5.063530238391393e-06, -4.105238700808311e-06]
q-binned i2, only sigma, unnormalised=  [-6.580475211586497e-06, -1.8852071710034979e-06, -1.9395192086262386e-06]
Bphis=0.05:
q-binned i2, unnormalised=  [0, -3.2841437158089833e-06, -2.3437768521223334e-06]
q-binned i2, only sigma, unnormalised=  [0, -1.0589910044237914e-07, -1.7804473344695807e-07]
Bphis=0.27:
q-binned i2, unnormalised=  [0, -5.813609180047512e-06, -4.631730275240701e-06]
q-binned i2, only sigma, unnormalised=  [0, -2.635281543173566e-06, -2.466012347745985e-06]
delta4=0.5Pi:
q-binned i2, unnormalised=  [0, -4.540853441819108e-06, -3.6413998519127966e-06]
q-binned i2, only sigma, unnormalised=  [0, -1.3625334211919977e-06, -1.475667832179959e-06]
delta4=0.2Pi:
q-binned i2, unnormalised=  [0, -4.607349462466324e-06, -3.5890404277304677e-06]
q-binned i2, only sigma, unnormalised=  [0, -1.4290292647802049e-06, -1.423307945751488e-06]
delta3=-0.4Pi:
q-binned i2, unnormalised=  [0, -4.796424654888648e-06, -3.242962990688254e-06]
q-binned i2, only sigma, unnormalised=  [0, -1.6181046131700924e-06, -1.0772324244245792e-06]
delta3=1.2Pi:
q-binned i2, unnormalised=  [0, -4.562922975101808e-06, -3.5684101026827365e-06]
q-binned i2, only sigma, unnormalised=  [0, -1.384603025039869e-06, -1.402677712152775e-06]



\begin{table}
    \centering
    \renewcommand{\arraystretch}{1.4}
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    \multirow{1}{*}{$\sqrt{q^2}$-bin} & \multirow{1}{*}{$\Gamma^r$ (SM)} & $ \frac{\Gamma_\sigma^r}{\Gamma^r} $ (\%) & $\int \langle I_2 \rangle_+^r$ (\%) & $ \frac{\int \langle I_2\rangle _{+,\sigma}^r}{\int \langle I_2\rangle_{+}^r}$ (\%) & $\int \langle I_3 \rangle_+^r$ (\%) & $\int \langle I_4 \rangle_-^r$ (\%) \\
    %\cline{3-7}
    %& & \multicolumn{5}{c|}{ (\%) } \\
    \hline 
   %%$ r^{({\rm low})} $        & 0.08 &   17  & -1.2 & 26 & -0.2 & 0.8\\ 
   %%$ r^{(\eta)} $             & 0.03 &   15  & -0.5 & 28 & -0.1 & 0.5 \\ 
   %%$ r^{(\rho: {\rm inf})} $  & 1.09 &  32  &  -18.8& 61 & -6.4 & 15.0\\
   $ r^{(\rho: {\rm sup})} $  & [3.4,4.6] &  [23,43]    & [-84,-45] & [59,78] & [-38,-25]  & [44, 66]\\ %CV:0.59 %[-12.7, -9.0]
   $ r^{(\phi: {\rm inf})} $  & [8.7,10.0] & [0.3,8]    & [-58,-33]  & [3,45] & [-160,-139] & [189, 219]\\ %CV:1.00 %[0.96,1.03] %[-13.3, -12.2] %[16.5, 18.1]
   $ r^{(\phi: {\rm sup})} $  & [6.3,7.1] &  [0.8,10]   & [-46,-23] &  [8,53] & [-114,-100] & [135, 153]  \\ %CV:0.85 %[-11.9, -9.8] %[13.0, 15.8]
   %%$ r^{({\rm high})} $       & 0.01 &  13 &    -0.1 & 62&  -0.2& 0.3  \\
       \hline 
    \end{tabular}
    \caption{With the wrong fudge factor.}
\end{table}

\begin{table}
    \centering
    \renewcommand{\arraystretch}{1.4}
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    \multirow{1}{*}{$\sqrt{q^2}$-bin} & \multirow{1}{*}{$\Gamma^r$ (SM)} & $ \frac{\Gamma_\sigma^r}{\Gamma^r} $ (\%) & $\int \langle I_2 \rangle_+^r$ (\%) & $ \frac{\int \langle I_2\rangle _{+,\sigma}^r}{\int \langle I_2\rangle_{+}^r}$ (\%) & $\int \langle I_3 \rangle_+^r$ (\%) & $\int \langle I_4 \rangle_-^r$ (\%) \\
    %\cline{3-7}
    %& & \multicolumn{5}{c|}{ (\%) } \\
    \hline 
   %%$ r^{({\rm low})} $        & 0.08 &   17  & -1.2 & 26 & -0.2 & 0.8\\ 
   %%$ r^{(\eta)} $             & 0.03 &   15  & -0.5 & 28 & -0.1 & 0.5 \\ 
   %%$ r^{(\rho: {\rm inf})} $  & 1.09 &  32  &  -18.8& 61 & -6.4 & 15.0\\
   $ r^{(\rho: {\rm sup})} $  & [6.4,8.7] &  [23,43]    & [-159,-85] & [59,78] & [-72,-47]  & [83,125]\\ %CV:0.59 %[-12.7, -9.0]
   $ r^{(\phi: {\rm inf})} $  & [16.4,18.9] & [0.3,8]    & [-110,-62]  & [3,45] & [-302,-263] & [357,414]\\ %CV:1.00 %[0.96,1.03] %[-13.3, -12.2] %[16.5, 18.1]
   $ r^{(\phi: {\rm sup})} $  & [11.9,13.4] &  [0.8,10]   & [-87,-43] &  [8,53] & [-215,-189] & [255,289]  \\ %CV:0.85 %[-11.9, -9.8] %[13.0, 15.8]
   %%$ r^{({\rm high})} $       & 0.01 &  13 &    -0.1 & 62&  -0.2& 0.3  \\
       \hline 
    \end{tabular}
\caption{Corrected fudge factor.}    
\end{table}




********************************** I2, 4, 8 of S-P interference **********************************************
!!! Semi-important: I was using a wrong argC9S, with the Bphi, Bomega instead of BphiS. Basically the BphiS was different, larger than it should be. Hope it doesn't play a role. 
For deltaSP=0 (which is set by phirhol=0, phirhols=Pi)

                                                                                                        at bfp:
                                                                                                        q-binned i2minus, unnormalised=  [1.1595251434146153e-06, -2.393984763242869e-06, 2.833196494738698e-06]
                                                                                                        q-binned i4 scalar, unnormalised=  [-6.699788192491575e-07, 1.6812893026331256e-06, -1.9161241040398626e-06]
                                                                                                        q-binned i8 scalar, unnormalised=  [-3.427353425612539e-07, 1.1147110523508785e-06, 8.651581115800289e-07]

                                                                                                        asrel=14
                                                                                                        q-binned i2minus, unnormalised=  [ 8.57999578e-07 -1.77144750e-06  2.09644561e-06]
                                                                                                        q-binned i4 scalar, unnormalised=  [-4.95755997e-07  1.24408299e-06 -1.41785082e-06]
                                                                                                        q-binned i8 scalar, unnormalised=  [-2.53609662e-07  8.24839045e-07  6.40180421e-07]
                                                                                                        asrel=22
                                                                                                        q-binned i2minus, unnormalised=  [ 1.34828505e-06 -2.78370321e-06  3.29441453e-06]
                                                                                                        q-binned i4 scalar, unnormalised=  [-7.79045139e-07  1.95498756e-06 -2.22805128e-06]
                                                                                                        q-binned i8 scalar, unnormalised=  [-3.98529468e-07  1.29617564e-06  1.00599780e-06]
                                                                                                    delta1=0.5Pi:
                                                                                                    q-binned i2minus, unnormalised=  [1.1741663481504288e-06, -2.4833020141096335e-06, 2.6640108356682237e-06]
                                                                                                    q-binned i4 scalar, unnormalised=  [-6.760465054718888e-07, 1.7419220963457672e-06, -1.7994316387500992e-06]
                                                                                                    q-binned i8 scalar, unnormalised=  [-3.530106774367294e-07, 1.347453402746496e-06, 1.0745638117300424e-06]
                                                                                                    delta1=0.9Pi:
                                                                                                    q-binned i2minus, unnormalised=  [1.1244780487686961e-06, -2.278488072202235e-06, 2.9439078849775253e-06]
                                                                                                    q-binned i4 scalar, unnormalised=  [-6.525806433421043e-07, 1.6024942735391985e-06, -1.9926866510420268e-06]
                                                                                                    q-binned i8 scalar, unnormalised=  [-3.281612283831936e-07, 4.755982984940988e-07, 3.1997256459231437e-07]
                                                                                                    delta3=-0.4Pi:
                                                                                                    q-binned i2minus, unnormalised=  [2.126028651331658e-06, -3.353261157801652e-06, -1.640532268047534e-06]
                                                                                                        q-binned i4 scalar, unnormalised=  [-1.2934548669609292e-06, 2.2449629280118926e-06, 1.158062661314895e-06]
                                                                                                        q-binned i8 scalar, unnormalised=  [-7.404368781202404e-07, 8.478861370557866e-07, 7.266611649146262e-07]

                                                                                                    delta3=1.2Pi:
                                                                                                    q-binned i2minus, unnormalised=    [1.3754859157518184e-06, -2.9273843786524568e-06, 2.3751658431987135e-06]
                                                                                                    q-binned i4 scalar, unnormalised=  [-8.196506704254776e-07, 2.0362921746078936e-06, -1.5967114072223833e-06]
                                                                                                    q-binned i8 scalar, unnormalised=  [-4.6068551679675087e-07, 1.2237621446758566e-06, 9.649324988846956e-07]

                                                                                                        delta4=0.5Pi:
                                                                                                        q-binned i2minus, unnormalised=  [3.065541870820826e-06, -2.3563046469531517e-06, 2.8844586512387715e-06]
                                                                                                        q-binned i4 scalar, unnormalised=  [-1.7391914937127178e-06, 1.6542697549938152e-06, -1.9517487571718385e-06]
                                                                                                        q-binned i8 scalar, unnormalised=  [-9.284166720067115e-07, 1.1023666802010537e-06, 8.693547490031093e-07]

                                                                                                    delta4=0.2Pi:
                                                                                                    q-binned i2minus, unnormalised=    [-5.461870869741066e-07, -2.430678920960329e-06, 2.81229245514679e-06]
                                                                                                    q-binned i4 scalar, unnormalised=  [2.8428038450009536e-07, 1.70731577177725e-06, -1.9012955053986508e-06]
                                                                                                    q-binned i8 scalar, unnormalised=  [1.7267287744575043e-07, 1.1277634235112647e-06, 8.688169605969795e-07]

                                                                                                        BphiS=0.05:
                                                                                                        q-binned i2minus, unnormalised=  [1.140880931642061e-06, -5.829980710807882e-07, 9.81112226478297e-07]
                                                                                                        q-binned i4 scalar, unnormalised=  [-6.52156687417178e-07, 4.045201487484453e-07, -6.671119129324554e-07]
                                                                                                        q-binned i8 scalar, unnormalised=  [-3.277872031132075e-07, 2.7274696962708445e-07, 2.728895482762133e-07]

                                                                                                        Bphis=0.27:
                                                                                                        q-binned i2minus, unnormalised=  [1.1670445964543466e-06, -3.342455702327055e-06, 3.701510263281548e-06]
                                                                                                        q-binned i4 scalar, unnormalised=  [-6.776756213487722e-07, 2.346046289008913e-06, -2.501711123804662e-06]
                                                                                                        q-binned i8 scalar, unnormalised=  [-3.4944675480768533e-07, 1.5378899470353994e-06, 1.1427347578149303e-06]



With phirhol=0, phirhols=Pi with the corrected argC9S:
at bfp with the corrected argument of C9S:
q-binned i2minus, unnormalised=  [1.9543437515818287e-06, -2.219403899613173e-06, 2.9193449155512403e-06]
q-binned i4 scalar, unnormalised=  [-1.1489732435143402e-06, 1.5647665593616364e-06, -1.976793145422716e-06]
q-binned i8 scalar, unnormalised=  [-5.733109498977503e-07, 1.07354624772129e-06, 8.296998822377134e-07]
delta1=0.5Pi:
q-binned i2minus, unnormalised=  [2.0757644947195636e-06, -2.2878344926916398e-06, 2.7483984075279023e-06]
q-binned i4 scalar, unnormalised=  [-1.2207616207934557e-06, 1.6116866132310246e-06, -1.8588194966808905e-06]
q-binned i8 scalar, unnormalised=  [-5.99006737662971e-07, 1.3206268789704302e-06, 1.0681773050452882e-06]
delta1=0.9Pi:
q-binned i2minus, unnormalised=  [1.778005159308109e-06, -2.1327529501903096e-06, 3.0308118712142187e-06]
q-binned i4 scalar, unnormalised=  [-1.0443781537258598e-06, 1.5049107357339787e-06, -2.05391643663453e-06]
q-binned i8 scalar, unnormalised=  [-5.217923311362972e-07, 4.3213368382689994e-07, 2.6721013480547156e-07]
asrel=14:
q-binned i2minus, unnormalised=  [1.4461324100652557e-06, -1.6422728745203887e-06, 2.1601935910890336e-06]
q-binned i4 scalar, unnormalised=  [-8.501900935948539e-07, 1.1578655220082739e-06, -1.4627434034735816e-06]
q-binned i8 scalar, unnormalised=  [-4.242262978109851e-07, 7.943806769215142e-07, 6.139420000079731e-07]
asrel=22:
q-binned i2minus, unnormalised=  [2.2724916914531354e-06, -2.580702040065478e-06, 3.3945853765093277e-06]
q-binned i4 scalar, unnormalised=  [-1.3360153269042218e-06, 1.819494316097837e-06, -2.2985970052404493e-06]
q-binned i8 scalar, unnormalised=  [-6.666410798809199e-07, 1.2483114608576472e-06, 9.647673264182686e-07]
delta3=-0.4Pi, corrected argC9S:
q-binned i2minus, unnormalised=  [2.293823625052209e-06, -2.982311720013263e-06, -1.3602420703469443e-06]
q-binned i4 scalar, unnormalised=  [-1.3608265112565333e-06, 1.99690482243643e-06, 9.64567254897212e-07]
q-binned i8 scalar, unnormalised=  [-6.928593475585266e-07, 7.400789158822773e-07, 7.607657792716198e-07]
delta3=0.7Pi:
q-binned i2minus, unnormalised=  [2.1522511268619514e-06, 3.368665726856851e-06, 3.0396713109193448e-06]
q-binned i4 scalar, unnormalised=  [-1.248174237395593e-06, -2.237281978411208e-06, -2.114122861948863e-06]
q-binned i8 scalar, unnormalised=  [-5.826605614809663e-07, -7.019792978988328e-07, -4.5539907589153224e-07]
delta3=1.2Pi, corrected argC9S:
q-binned i2minus, unnormalised=  [1.970635521575368e-06, -2.749938366994883e-06, 2.4978798276202357e-06]
q-binned i4 scalar, unnormalised=  [-1.1611640791653737e-06, 1.9173726444744963e-06, -1.6826469085559324e-06]
q-binned i8 scalar, unnormalised=  [-5.839069216320976e-07, 1.1867292056828002e-06, 9.28224213393628e-07]
delta3=2.2Pi:
q-binned i2minus, unnormalised=  [2.574475850464653e-06, 4.054726594722981e-06, -1.5737212654951988e-06]
q-binned i4 scalar, unnormalised=  [-1.5050878878342182e-06, -2.7984489591869584e-06, 1.041856554018037e-06]
q-binned i8 scalar, unnormalised=  [-7.151550532190136e-07, -1.545155235661764e-06, -8.784975112687473e-07]
delta4=0.5Pi with the corrected argC9S:
q-binned i2minus, unnormalised=  [3.508692422710007e-06, -2.1180682183270646e-06, 2.986415203484887e-06]
q-binned i4 scalar, unnormalised=  [-1.9875054679813182e-06, 1.4951799532272504e-06, -2.023661174621486e-06]
q-binned i8 scalar, unnormalised=  [-1.0003439262894518e-06, 1.0455414097644993e-06, 8.239843461641413e-07]
delta4=0.5Pi, delta3=2.2Pi:
q-binned i2minus, unnormalised=  [4.128821409531533e-06, 4.1560706728587205e-06, -1.506636260267706e-06] actually this is a value higher than what I gave before. 
delta4=0.2Pi with the corrected argC9S:
q-binned i2minus, unnormalised=  [3.962139657158394e-07, -2.2789927553324484e-06, 2.882174598102631e-06]
q-binned i4 scalar, unnormalised=  [-2.749062858387951e-07, 1.6071168537639457e-06, -1.95035548029473e-06]
q-binned i8 scalar, unnormalised=  [-7.968071520270982e-08, 1.090207672451482e-06, 8.449597551834763e-07]
BphiS=0.05, corrected argC9S:
q-binned i2minus, unnormalised=  [2.193062650265012e-06, -6.556396160064902e-08, 1.0764015917810704e-06]
q-binned i4 scalar, unnormalised=  [-1.2871119202950347e-06, 6.07959016440956e-08, -7.344977977580328e-07]
q-binned i8 scalar, unnormalised=  [-6.304453275594967e-07, 1.3398130354830068e-07, 2.2606839749281716e-07]
Bphis=0.27, corrected argC9S:
q-binned i2minus, unnormalised=  [1.842527981945373e-06, -3.2245414886095596e-06, 3.7793848787013617e-06]
q-binned i4 scalar, unnormalised=  [-1.084493326075927e-06, 2.2666302323608026e-06, -2.5565306380449266e-06]
q-binned i8 scalar, unnormalised=  [-5.465049923268495e-07, 1.5120173540588158e-06, 1.11138989152145e-06]





                                                                                                For phirhol=0, phirhols=Pi/2 (which means DeltaSP=3Pi/2):
                                                                                                
                                                                                                at bfp: 
                                                                                                q-binned i2minus, unnormalised=  [8.438151718382322e-07, -3.1660824917025437e-06, -2.2289493976264722e-06]
                                                                                                q-binned i4 scalar, unnormalised=  [-3.750382399879519e-07, 2.1209953131786942e-06, 1.5634308643807126e-06]
                                                                                                q-binned i8 scalar, unnormalised=  [-1.8056190981133645e-07, 7.103754494133375e-07, 7.21656743278848e-07]
                                                                                                asrel=14
                                                                                                q-binned i2minus, unnormalised=  [ 6.24387548e-07 -2.34276717e-06 -1.64932831e-06]
                                                                                                q-binned i4 scalar, unnormalised=  [-2.77512440e-07  1.56944685e-06  1.15687273e-06]
                                                                                                q-binned i8 scalar, unnormalised=  [-1.33608179e-07  5.25647796e-07  5.33995476e-07]
                                                                                                asrel=22
                                                                                                q-binned i2minus, unnormalised=  [ 9.81180432e-07 -3.68149127e-06 -2.59180163e-06]
                                                                                                q-binned i4 scalar, unnormalised=  [-4.36090977e-07  2.46627362e-06  1.81794287e-06]
                                                                                                q-binned i8 scalar, unnormalised=  [-2.09955709e-07  8.26017964e-07  8.39135748e-07]
                                                                                                Delta1=0.5Pi:
                                                                                                q-binned i2minus, unnormalised=  [8.394983865267595e-07, -3.1862849024305265e-06, -2.180712468116561e-06]
                                                                                                q-binned i4 scalar, unnormalised=  [-3.704296465178349e-07, 2.1330254477491327e-06, 1.5289787885103693e-06]
                                                                                                q-binned i8 scalar, unnormalised=  [-1.701224134255407e-07, -5.657879444201949e-08, 8.23714746201298e-08]
                                                                                                delta1=0.9Pi:
                                                                                                q-binned i2minus, unnormalised=  [8.293329994133127e-07, -3.1168287630464786e-06, -2.2501561705907505e-06]
                                                                                                q-binned i4 scalar, unnormalised=  [-3.711788826181086e-07, 2.0896272359522023e-06, 1.5788165497672084e-06]
                                                                                                q-binned i8 scalar, unnormalised=  [-1.8306708879039546e-07, 1.1940561919904887e-06, 1.1157553838134036e-06]
                                                                                                delta3=-0.4Pi:
                                                                                                q-binned i2minus, unnormalised=  [1.951316486404989e-06, 2.463172226388721e-06, -2.65630216099526e-06]
                                                                                                q-binned i4 scalar, unnormalised=  [-9.775935591340006e-07, -1.7247416165454904e-06, 1.799863966173928e-06]
                                                                                                q-binned i8 scalar, unnormalised=  [-3.557080923796919e-07, -1.1393179211924407e-06, -6.592762789006939e-07]
                                                                                                delta3=1.2Pi:
                                                                                                q-binned i2minus, unnormalised=  [1.2991291759734251e-06, -2.6531702410144506e-06, -2.6494330981928054e-06]
                                                                                                q-binned i4 scalar, unnormalised=  [-6.361734690684073e-07, 1.763060710743692e-06, 1.8461056792406996e-06]
                                                                                                q-binned i8 scalar, unnormalised=  [-2.671911526723194e-07, 4.942062875283637e-07, 5.558638500436675e-07]
                                                                                                delta4=0.5Pi:
                                                                                                q-binned i2minus, unnormalised=  [1.0133977475403957e-06, -3.124876640181653e-06, -2.2191035648410655e-06]
                                                                                                q-binned i4 scalar, unnormalised=  [-3.9740426604397775e-07, 2.0935730801241318e-06, 1.5570097089667354e-06]
                                                                                                q-binned i8 scalar, unnormalised=  [-2.886316041641513e-08, 6.970190943816296e-07, 7.351408265305682e-07]
                                                                                                delta4=0.2Pi:
                                                                                                q-binned i2minus, unnormalised=  [5.982761805302364e-07, -3.211323036526393e-06, -2.255147423311375e-06]
                                                                                                q-binned i4 scalar, unnormalised=  [-3.1677524088342196e-07, 2.151134847686725e-06, 1.5814114604956204e-06]
                                                                                                q-binned i8 scalar, unnormalised=  [-2.6936290444858274e-07, 7.235494588070325e-07, 7.147007403921545e-07]
                                                                                                BphiS=0.05:
                                                                                                q-binned i2minus, unnormalised=  [7.772359167751315e-07, -6.941495242985149e-07, -6.35046743467601e-07]
                                                                                                q-binned i4 scalar, unnormalised=  [-3.375695724589888e-07, 4.628946246805406e-07, 4.466142902051297e-07]
                                                                                                q-binned i8 scalar, unnormalised=  [-1.6385534959143287e-07, 1.4472388301821589e-07, 2.417899412375787e-07]
                                                                                                BphiS=0.27:
                                                                                                q-binned i2minus, unnormalised=  [8.756380685627626e-07, -4.319152827606423e-06, -2.975710442994089e-06]
                                                                                                q-binned i4 scalar, unnormalised=  [-3.929785641341073e-07, 2.891979497911179e-06, 2.0866748305109885e-06]
                                                                                                q-binned i8 scalar, unnormalised=  [-1.8853618357483808e-07, 9.79607919204469e-07, 9.465963821369785e-07]


For phirhol=0, phirhols=Pi/2 (which means DeltaSP=3Pi/2) AND CORRECTED argC9S:

at bfp with corrected argC9S:
q-binned i2minus, unnormalised=  [9.704366043146986e-07, -3.197139334183171e-06, -2.0868129363818463e-06]
q-binned i4 scalar, unnormalised=  [-4.0940865736840646e-07, 2.1465059287524825e-06, 1.4667197314218668e-06]
q-binned i8 scalar, unnormalised=  [-1.207745979602537e-07, 7.365703167941025e-07, 7.596088792611095e-07]
asrel=14:
q-binned i2minus, unnormalised=  [7.180856021732345e-07, -2.36575110873763e-06, -1.5441328486011424e-06]
q-binned i4 scalar, unnormalised=  [-3.0294578627442587e-07, 1.5883238003101621e-06, 1.0852927800674635e-06]
q-binned i8 scalar, unnormalised=  [-8.937520587101153e-08, 5.450319615893013e-07, 5.620788600760091e-07]
asrel=22:
q-binned i2minus, unnormalised=  [1.1283437567224945e-06, -3.7176029242660672e-06, -2.426529175122345e-06]
q-binned i4 scalar, unnormalised=  [-4.760506415893694e-07, 2.495936434342668e-06, 1.7054885052751755e-06]
q-binned i8 scalar, unnormalised=  [-1.4043553891240162e-07, 8.56476880256285e-07, 8.832655162433654e-07]
at bphis=0.05:
q-binned i2minus, unnormalised=  [9.212553883893146e-07, -7.429497850724875e-07, -4.5216614924800517e-07]
q-binned i4 scalar, unnormalised=  [-3.6934236369928726e-07, 5.090168440507644e-07, 3.220018293610608e-07]
q-binned i8 scalar, unnormalised=  [-8.005874157381118e-08, 1.7049364083049946e-07, 2.8591139047816186e-07]
at bphis=0.27:
q-binned i2minus, unnormalised=  [9.93326159357306e-07, -4.3423787976077065e-06, -2.8496142384066863e-06]
q-binned i4 scalar, unnormalised=  [-4.281083860186736e-07, 2.9106580378986758e-06, 2.0008876427814222e-06]
q-binned i8 scalar, unnormalised=  [-1.398000751942374e-07, 1.0007411400260485e-06, 9.806679547847688e-07]
delta1=0.5Pi:
q-binned i2minus, unnormalised=  [9.719783631459916e-07, -3.2142527033293835e-06, -2.049496947291384e-06]
q-binned i4 scalar, unnormalised=  [-4.0332065041389817e-07, 2.1571431212175986e-06, 1.4398354505666888e-06]
q-binned i8 scalar, unnormalised=  [-6.872986487867547e-08, -1.4571590264939023e-08, 1.3081868808185314e-07]
delta1=0.9Pi:
q-binned i2minus, unnormalised=  [9.482414690607299e-07, -3.151515593086042e-06, -2.1006636443911843e-06]
q-binned i4 scalar, unnormalised=  [-4.0784899490702585e-07, 2.1166288877168826e-06, 1.4769895272553307e-06]
q-binned i8 scalar, unnormalised=  [-1.4768175826148445e-07, 1.1990257153744318e-06, 1.1281481915841648e-06]
delta3=-0.4Pi:
q-binned i2minus, unnormalised=  [1.2292036399857367e-06, 2.471420120805744e-06, -2.639965053040712e-06]
q-binned i4 scalar, unnormalised=  [-5.457531120226313e-07, -1.724077777667176e-06, 1.7903035011080288e-06]
q-binned i8 scalar, unnormalised=  [-1.4951083081797978e-07, -1.1557428655850293e-06, -5.826866074694353e-07]
delta3=0.7Pi:
q-binned i2minus, unnormalised=  [6.031788737587465e-07, -3.3270997051489287e-06, 2.1285222291785428e-06]
q-binned i4 scalar, unnormalised=  [-1.8411893053856173e-07, 2.3211152790099786e-06, -1.4218272955471544e-06]
q-binned i8 scalar, unnormalised=  [-8.751980136504949e-10, 1.3477170930739569e-06, 1.0313659562274878e-06]
delta3=1.2Pi:
q-binned i2minus, unnormalised=  [1.0252734821248115e-06, -2.6412885321438816e-06, -2.4845825074744482e-06]
q-binned i4 scalar, unnormalised=  [-4.409592891546032e-07, 1.7599490754681273e-06, 1.7338804556774025e-06]
q-binned i8 scalar, unnormalised=  [-1.3333439327590067e-07, 5.0457538535376e-07, 6.082783562427322e-07]
delta3=2.2Pi:
q-binned i2minus, unnormalised=  [7.84611952141851e-07, 2.7912482811593627e-06, 2.670298849955309e-06]
q-binned i4 scalar, unnormalised=  [-2.710916521386704e-07, -1.8335360149204098e-06, -1.8532908614547227e-06]
q-binned i8 scalar, unnormalised=  [3.611239085162054e-10, -5.409648706938762e-07, -3.5224782166744733e-07]
delta4=0.5Pi:
q-binned i2minus, unnormalised=  [5.889812158091552e-07, -3.1295110687047956e-06, -2.0369826791377726e-06]
q-binned i4 scalar, unnormalised=  [-1.2986348885499826e-07, 2.103186013037645e-06, 1.4329411492780356e-06]
q-binned i8 scalar, unnormalised=  [1.2791397253875207e-07, 7.183195014587718e-07, 7.819746795789592e-07]
delta4=0.2Pi:
q-binned i2minus, unnormalised=  [6.048230589054035e-07, -3.3034018817619544e-06, -2.1616720089145327e-06]
q-binned i4 scalar, unnormalised=  [-2.778543042693713e-07, 2.216701822644733e-06, 1.518098010557106e-06]
q-binned i8 scalar, unnormalised=  [-1.483879756114433e-07, 7.655399557660635e-07, 7.422854460910501e-07]


 \begin{table}  
%%\hspace{-2cm}
\centering
    \renewcommand{\arraystretch}{1.4}
    \begin{tabular}{|c|c|}
        \hline
        $\sqrt{q^2}$-bin & $\int \langle I_{2} \rangle_{-}^r$ (\%) \\
        \hline
        $ r^{(\rho: {\rm sup})} $ & $[-66,-7.5] \, c_{SP}+ [-23,-11] \, s_{SP}$ \\
        \hline
        $ r^{(\phi: {\rm inf})} $ & $[-77,61] \, c_{SP}+[-53,82] \, s_{SP}$ \\ %[-9.1,10.5]
        \hline
        $ r^{(\phi: {\rm sup})} $ & $[-71,30] \, c_{SP}+[-50,54] \, s_{SP}$ \\
        \hline
        %%%%%%
        \hline 
        $\sqrt{q^2}$-bin & $\int \langle I_4 \rangle_{+}^r$ (\%) \\
        \hline
        $ r^{(\rho: {\rm sup})} $ & $[8.2,59] \, c_{SP} + [3.9,16] \, s_{SP}$ \\
        \hline
        $ r^{(\phi: {\rm inf})} $ & $[-67,83] \, c_{SP} + [-86,54] \, s_{SP} $ \\ %[-11.3,9.6]
        \hline
        $ r^{(\phi: {\rm sup})} $ & $[-31,76] \, c_{SP} + [-59,55] \, s_{SP}$ \\
        \hline
        %%%%%%
        \hline  
        $\sqrt{q^2}$-bin & $\int \langle I_8 \rangle_{+}^r$ (\%) \\
        \hline
        $ r^{(\rho: {\rm sup})} $ & $[-30,-2.4] \, c_{SP} + [-4.4,3.8] \, s_{SP}$ \\
        \hline
        $ r^{(\phi: {\rm inf})} $ & $[-46,45] \, c_{SP} + [-34,40] \, s_{SP}$ \\
        \hline
        $ r^{(\phi: {\rm sup})} $ & $[-26,33] \, c_{SP} + [-17,33] \, s_{SP}$ \\
        \hline
    \end{tabular}
    \caption{Corrected for the fudge factor}
 \end{table}



 *************************************************************************** I5, I6 vector *************************8

for phirhol=0 

at bfp:
q-binned i5 vector, unnormalised=  [-4.969114231632318e-06, -3.4556091479203553e-07, -4.582601684372352e-06]
q-binned i6, unnormalised=  [-4.603629876623129e-06, -3.7348470180705367e-07, -4.9323217148448425e-06]
delta1=0.5Pi:
q-binned i5 vector, unnormalised=  [-6.6238362472315135e-06, -3.93681775674495e-06, -2.4411416611653006e-06]
q-binned i6, unnormalised=  [-6.160625434293157e-06, -4.1624470881311816e-06, -2.625196596214577e-06]
delta1=0.9Pi:
q-binned i5 vector, unnormalised=  [-3.927017448615156e-06, 2.8331275306138708e-06, -5.259632139901114e-06]
q-binned i6, unnormalised=  [-3.622772754265262e-06, 2.990378564022298e-06, -5.66547558725723e-06]


for phirhol=Pi/2 (so deltarhoNP=pi/2, but also this means that you have to use a minus):

at bfp:
q-binned i5 vector, unnormalised=  [-1.1585417765184935e-05, -6.572287081497787e-06, 2.033421142321447e-06]
q-binned i6, unnormalised=  [-1.0530264885304452e-05, -6.930828220598064e-06, 2.1920311096395497e-06]
delta1=0.5Pi:
q-binned i5 vector, unnormalised=  [-1.2090031643124703e-05, -6.107326582708013e-06, 3.829048346855339e-06]
q-binned i6, unnormalised=  [-1.1004557948974501e-05, -6.422941399031876e-06, 4.120200169745737e-06]
delta1=0.9Pi:
q-binned i5 vector, unnormalised=  [-1.0204555411282732e-05, -4.837558542893021e-06, -6.780259692280589e-07]
q-binned i6, unnormalised=  [-9.231374635051548e-06, -5.114621132293686e-06, -7.24098990893512e-07]

\begin{comment}
\begin{table}[]
    \centering
    \renewcommand{\arraystretch}{1.4}
   \begin{tabular}{|c|c|}
        \hline
        $\sqrt{q^2}$-bin & $\int \langle I_{5} \rangle_{-}^r$ (\%) \\
        \hline
        $ r^{(\rho: {\rm sup})} $ & $[-4.4, -2.6] \, c_{\rho {\rm NP}}+ [6.8,8.1] \, s_{\rho {\rm NP}}$ \\
        \hline
        $ r^{(\phi: {\rm inf})} $ & $[-2.62667, 1.88667] \, c_{\rho {\rm NP}}+[3.2,4.4] \, s_{\rho {\rm NP}}$ \\
        \hline
        $ r^{(\phi: {\rm sup})} $ & $[-3.5064, -1.62733] \, c_{\rho {\rm NP}}+[-2.6,0.5] \, s_{\rho {\rm NP}}$ \\ %[-1,-0.7]
        \hline
        %%%%%%
        \hline
        $\sqrt{q^2}$-bin & $\int \langle I_6 \rangle_{+}^r$ (\%) \\
        \hline
        $ r^{(\rho: {\rm sup})} $ & $[-6.1606, -3.6228] \, c_{\rho {\rm NP}} + [9.23,11.0] \, s_{\rho {\rm NP}}$ \\
        \hline
        $ r^{(\phi: {\rm inf})} $ & $[-4.16,2.99] \, c_{\rho {\rm NP}} + [5.11,6.93] \, s_{\rho {\rm NP}} $ \\
        \hline
        $ r^{(\phi: {\rm sup})} $ & $[-5.665,-2.625] \, c_{\rho {\rm NP}} + [-4.12,0.724] \, s_{\rho {\rm NP}}$ \\
        \hline
    \end{tabular}
    \caption{This is multiplied with whatever contains the old value of C2, but also the old value of Brho (extracted based on the old C2).}
\end{table}
\end{comment}


\begin{table}[]
    \centering
    \renewcommand{\arraystretch}{1.4}
   \begin{tabular}{|c|c|}
        \hline
        $\sqrt{q^2}$-bin & $\int \langle I_{5} \rangle_{-}^r$ (\%) \\
        \hline
        $ r^{(\rho: {\rm sup})} $ & $[4.9,8.3] \, c_{\rho {\rm NP}}+ [-15,-13] \, s_{\rho {\rm NP}}$ \\
        \hline
        $ r^{(\phi: {\rm inf})} $ & $[-3.6,5.0] \, c_{\rho {\rm NP}}+[-8.3,-6.0] \, s_{\rho {\rm NP}}$ \\
        \hline
        $ r^{(\phi: {\rm sup})} $ & $[3.1,6.6] \, c_{\rho {\rm NP}}+[-0.9,4.9] \, s_{\rho {\rm NP}}$ \\ %[-1,-0.7]
        \hline
        %%%%%%
        \hline
        $\sqrt{q^2}$-bin & $\int \langle I_6 \rangle_{+}^r$ (\%) \\
        \hline
        $ r^{(\rho: {\rm sup})} $ & $[6.8,12] \, c_{\rho {\rm NP}} + [-21,-17] \, s_{\rho {\rm NP}}$ \\
        \hline
        $ r^{(\phi: {\rm inf})} $ & $[-5.7,7.8] \, c_{\rho {\rm NP}} + [-13,-9.7] \, s_{\rho {\rm NP}} $ \\
        \hline
        $ r^{(\phi: {\rm sup})} $ & $[5.0,11] \, c_{\rho {\rm NP}} + [-1.4,7.8] \, s_{\rho {\rm NP}}$ \\
        \hline
    \end{tabular}
    \caption{Corrected fudge factor}
\end{table}

***************************** I5, I7 scalar ************************************

For phirhols=Pi, phirhol=0:
q-binned i5 scalar, unnormalised=  [2.2522386427362684e-07, 5.161287660020507e-07, -1.2219838464216053e-06]
q-binned i7 scalar, unnormalised=  [-6.330578949988806e-06, -4.7592082820816085e-06, -1.995696148233731e-07]

For phirhols=Pi, phirhol=Pi/2:
q-binned i5 scalar, unnormalised=  [-2.5897171902067407e-06, -2.0848364279197584e-06, 4.1253060325240027e-07]
q-binned i7 scalar, unnormalised=  [2.2574246456113135e-06, -1.605509099370539e-06, 3.764626791001874e-06] (new)
And for asrel=22:
q-binned i5 scalar, unnormalised=  [-3.0113002990965764e-06, -2.4242284362083115e-06, 4.796863195490823e-07]


Changes I need to keep track of:
\begin{itemize}
    \item Multiply with 2/3 or Pi/2 for the corresponding observables
    \item Multiply by $(C2old/C2new)^2\approx 1.89$ 
    \item For the null tests, multiply by 0.1 to bring it to a form comparable to the decay rates. 
    \item Multiply with $\Tilde{C_10}$ for the final collective table. 
\end{itemize}

The programme calculates (modulo some signs) 
I2+, I2- \\
I3 \\
2/pi I4+, 3/2 I4- \\
2/pi I5+, 3/2 I5- \\
I6 \\
2/pi I7+, 3/2 I7- \\ 
2/pi I8+, 3/2 I8- \\
Pay attention also to the signs:
I am not adjusting to the corrections below yet. 
On the numerical results side, (the following doesn't include the definitions of Psigma)
(done)the signs of I5, I6 should be flipped for the P-P interference case. I4(P-P) stays the same. 
(done)I4(S-P) should be flipped. (not sure this takes into account the argPsigma; it doesn't)
(done)I2(S-P) should be flipped. I8(S-P) stays the same. I5(S-P) stays the same. 
(doesn't matter) I7(S-P) should be flipped.

Also note that since delta3 is unconstrained ie there is no bfp, it could be that the max of I2,4,8 should be +-, if there is no equal opposite value for the BphiS for example.

==> integrationresults.tex <==
q-binned gammas, unnormalised=            [7.80883085846691e-07, 3.199327684401192e-07, 1.0930909300916493e-05, 5.8622304411911035e-06, 9.958004536084738e-06, 8.459707498282612e-06, 1.4376577749057777e-07]
q-binned gammas from Wmod, unnormalised=  [7.052868982597103e-07, 2.93776841401367e-07, 1.0660286633320164e-05, 5.672243499049174e-06, 9.922741918261606e-06, 8.495146096993606e-06, 1.5913593165038852e-07]
q-binned gammas from Wmod, unnormalised=                                                                       [5.672238782359302e-06, 9.922741730965501e-06, 8.495145814607997e-06]

(newer check 17/8 but not much has changed) 
From best fit point (16/8):
q-binned gammas, only sigma unnormalised=  [2.183261137965943e-06, 2.7333625570486806e-06, 1.8738411271959062e-06]
WITH A NON-OPTIMAL PHASE:
q-binned gammas from Wmod, unnormalised=  [5.445592334392097e-07, 2.391224366497912e-07, 1.0329382965002452e-05, 8.671520088749545e-06, 1.2799408263282645e-05, 6.681402996520821e-06, 2.8276681570985833e-08]
FOR BPHI=1:
q-binned gammas from Wmod, unnormalised=  [8.726704354969627e-07, 3.4491055402564973e-07, 1.0911963001742037e-05, 4.822895584336704e-06, 5.793243755008628e-05, 4.3949819408584024e-05, 4.1052181845862337e-07]


at bfp:
q-binned gammas from Wmod, unnormalised=                                                               5.672238782359302e-06, 9.922741730965501e-06, 8.495145814607997e-06]
for delta1=-0.4pi:
q-binned gammas, unnormalised=  [6.750809135785284e-07, 2.799656657117156e-07, 1.0044785689645962e-05, 6.626709271961168e-06, 1.0621619411372691e-05, 7.5456671126691905e-06, 9.330844830264442e-08]
for delta1=-0.8 *Pi: 
q-binned gammas, unnormalised=  [8.097932226335911e-07, 3.3183487822796943e-07, 1.1293230658329086e-05, 5.72655734671771e-06, 1.0015133734885899e-05, 8.749986433571643e-06, 1.555224587979952e-07]
for Delta1=-0.9Pi:
q-binned gammas from Wmod, unnormalised=                                                               [5.842289999335033e-06, 1.0187165430419727e-05, 8.949043374666311e-06]
for Delta1=-0.5Pi:
q-binned gammas from Wmod, unnormalised=                                                               [5.949967859151627e-06, 1.0255239262953245e-05, 7.895409246091193e-06]
for Delta2=-0.6Pi:
q-binned gammas from Wmod, unnormalised=                                                               [5.682182731241105e-06, 9.925575695106025e-06, 8.50196171126781e-06]
for Delta2=0.3Pi:
q-binned gammas from Wmod, unnormalised=                                                               [6.175041893758193e-06, 9.906208191608362e-06, 8.515801334212614e-06]
for Delta3=1.2Pi:
q-binned gammas from Wmod, unnormalised=                                                               [5.595611508923465e-06, 9.638707990870252e-06, 8.532145164136141e-06]
for Delta3=-0.4Pi:
q-binned gammas from Wmod, unnormalised=                                                               [5.821506765666703e-06, 9.793477950779602e-06, 8.362831953466297e-06]
for Delta4=0.6Pi:
q-binned gammas from Wmod, unnormalised=                                                               [6.4697207854225724e-06, 9.968377247771274e-06, 8.517207846147264e-06]
for Delta4=0.2Pi:
q-binned gammas from Wmod, unnormalised=                                                               [5.373679084683396e-06, 9.925575953268179e-06, 8.45026163480589e-06]


at the best fit point:
q-binned gammas, only sigma unnormalised=  [1.3404577441918685e-07, 4.93276297434481e-08, 3.4537727319956505e-06, 2.1832658546590763e-06, 2.7333627443444505e-06, 1.8738414095813961e-06, 1.920926969509564e-08]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
q-binned gammas, only sigma unnormalised=  [2.183261137965943e-06, 2.7333625570486806e-06, 1.8738411271959062e-06]
for Delta3=-0.4Pi:
q-binned gammas, only sigma unnormalised=  [2.3324393378852928e-06, 2.604099887181693e-06, 1.7415252876380349e-06]
for Delta3=1.2Pi:
q-binned gammas, only sigma unnormalised=  [2.106633338387824e-06, 2.449331418360251e-06, 1.910841754258666e-06]
for Delta4=0.6Pi:
q-binned gammas, only sigma unnormalised=  [2.980734337110988e-06, 2.7789975134420485e-06, 1.8959031330793833e-06]
for Delta4=0.2Pi:
q-binned gammas, only sigma unnormalised=  [1.8847010364898634e-06, 2.7361965067510937e-06, 1.8289569511598256e-06]


***************************************************************************************************I2 plus ***************************************************************************
q-binned i2, unnormalised=  [-1.2383397972990266e-07, -5.229979687730367e-08, -1.882765157316408e-06, -9.97326507650926e-07, -1.213244214154826e-06, -8.82142811866017e-07, -1.0954047826059166e-08]
q-binned i2, unnormalised=                                                                           [-9.97326507650926e-07, -1.213244214154826e-06, -8.82142811866017e-07]
for phirhol =  -0.8 *Pi:
q-binned i2, unnormalised=                                                                           [-9.891840531086483e-07, -1.2148609607914666e-06, -8.919062742610741e-07]
for phirhol =  -0.4 *Pi:
q-binned i2, unnormalised=                                                                           [-1.0443305142245358e-06, -1.239204464195375e-06, -8.516846216479389e-07]
for phirhol =  0.0 *Pi, phioml-phirhol =  0.13852209626946207 *Pi:
q-binned i2, unnormalised=                                                                           [-1.017038325633621e-06, -1.2283631666537211e-06, -8.605840560032448e-07]
the other end of Delta1:
q-binned i2, unnormalised=                                                                           [-1.0081076991559487e-06, -1.2202119444671293e-06, -8.956853358810598e-07]
for phioml-phirhol =  0.6 *Pi:
q-binned i2, unnormalised=                                                                           [-9.573795575069835e-07, -1.213131950856935e-06, -8.823520809609966e-07]
for phioml-phirhol =  -0.3 *Pi:
q-binned i2, unnormalised=                                                                           [-1.0094079490248561e-06, -1.213233386721682e-06, -8.819525428281453e-07]
for Delta3=-0.4Pi:
q-binned i2, unnormalised=                                                                           [-1.0396643715817075e-06, -1.166442904174575e-06, -8.370500969249913e-07]
dor Delta3=1.2Pi:
q-binned i2, unnormalised=                                                                           [-9.630491805516014e-07, -1.1122745525301557e-06, -8.9663748284355e-07]
for phirhols-phiomls= 0.2 *Pi:
q-binned i2, unnormalised=                                                                           [-8.973070528279712e-07, -1.2142224752546097e-06, -8.663506204179649e-07]
for phirhols-phiomls= 0.6 *Pi:
q-binned i2, unnormalised=                                                                           [-1.2659273807768718e-06, -1.2292347071203698e-06, -8.899022606337775e-07]

From sigma only (16/8):
q-binned i2, only sigma, unnormalised=  [-7.332652793509501e-07, -9.593272095450623e-07, -6.585430895020982e-07]
for Delta3=-0.4Pi:
q-binned i2, only sigma, unnormalised=  [-7.833272713915292e-07, -9.139438418897949e-07, -6.120256012706548e-07]
for Delta3=1.2Pi:
q-binned i2, only sigma, unnormalised=  [-7.833272713915292e-07, -9.139438418897949e-07, -6.120256012706548e-07]
for Delta4=0.6Pi:
q-binned i2, only sigma, unnormalised=  [-1.0018790517966229e-06, -9.75317126112562e-07, -6.663027467474423e-07]
for Delta4=0.2Pi:
q-binned i2, only sigma, unnormalised=  [-6.332425420600417e-07, -9.603046517613098e-07, -6.427512494016322e-07]


********************************OBSOLETE******************************
for phis=3.4:
q-binned i2minus, unnormalised=  [4.97901693082265e-08, 2.1519638991988045e-08, -5.740592424059666e-08, -3.627713513306836e-07, 8.619574056900171e-07, -2.473576465938681e-07, -1.2886372230522758e-08]
for phis=3.4-pi/2:
q-binned i2minus, unnormalised=  [-4.1818074217913144e-08, -2.0678617252582356e-08, -1.076360033549839e-06, -2.6631530821061717e-07, -2.743509454800201e-07, -7.413538776226822e-07, -5.216226181729407e-09]
q-binned i2, only sigma, unnormalised=  [-3.1603818214161724e-08, -1.4603858821162519e-08, -1.142179927682304e-06, -7.33266865832893e-07, -9.593272752344916e-07, -6.585431888445676e-07, -6.844747061304706e-09]
for phis=3.4-np.pi:
q-binned i2minus, unnormalised=  [-4.9790169308226365e-08, -2.1519638991988052e-08, 5.740592424059658e-08, 3.627713513306836e-07, -8.619574056900171e-07, 2.473576465938679e-07, 1.2886372230522754e-08]
******************************************************************************

Correct relative phase, phirhol=phirhols=0: $delta_{SP}$
q-binned i2minus, unnormalised=  [5.4425525556453594e-08, 1.0476185031239076e-06, 8.256755111454505e-07]
for Delta1=-0.9Pi:
q-binned i2minus, unnormalised=  [7.113390590782071e-08, 7.072454918107176e-07, 5.647370879000395e-07]
for Delta1=-0.5Pi:
q-binned i2minus, unnormalised=  [3.2670265494251946e-08, 9.283302116245887e-07, 7.672342108722257e-07]
for Delta2=-0.6Pi:
q-binned i2minus, unnormalised=  [3.1326299062097e-08, 1.0466014803934554e-06, 8.261711525499609e-07]
for Delta2=0.3Pi:
q-binned i2minus, unnormalised=  [1.1275054587807543e-07, 1.04772565128933e-06, 8.247068911355504e-07]
for Delta3=-0.4Pi:
q-binned i2minus, unnormalised=  [1.7234093987866098e-07, -9.135251545162793e-07, -7.179955402451723e-07]
for Delta3=1.2Pi:
q-binned i2minus, unnormalised=  [1.883143894681564e-07, -7.198624405506806e-07, -6.294936719721119e-07]
for Delta4=0.6Pi:
q-binned i2minus, unnormalised=  [-1.9779241300939343e-07, 1.0522057966875236e-06, 8.263156294620749e-07]
for Delta4=0.2Pi:
q-binned i2minus, unnormalised=  [1.4617041965796937e-07, 1.0482739917110244e-06, 8.175602522733697e-07]


For phirhol=0, phirhols=Pi/2:
at the best fit point:
q-binned i2minus, unnormalised=  [3.0512203974355263e-07, 9.423403060016981e-08, 1.8644773847712255e-07]
for Delta1=-0.9Pi:
q-binned i2minus, unnormalised=  [3.2821656405594016e-07, 8.155392818144598e-07, 6.696151323633473e-07]
for Delta1=-0.5Pi:
q-binned i2minus, unnormalised=  [2.980288586862756e-07, -5.347491921133821e-07, -2.501950619430295e-07]
for Delta2=-0.6Pi:
q-binned i2minus, unnormalised=  [2.471579350103149e-07, 9.428176315921362e-08, 1.8739224927608554e-07]
for Delta2=0.3Pi:
q-binned i2minus, unnormalised=  [2.919649632535866e-07, 9.326386398800119e-08, 1.8677537140059687e-07]
for Delta3=-0.4Pi:
q-binned i2minus, unnormalised=  [3.9170703657843335e-07, -4.908543419173607e-07, -3.9280360790459035e-07]
for Delta3=1.2Pi:
q-binned i2minus, unnormalised=  [3.05839236531785e-07, 7.162542193152425e-07, 5.881712684329019e-07]
for Delta4=0.6Pi:
q-binned i2minus, unnormalised=  [4.99970398815268e-07, 8.683117631647784e-08, 1.9918186839777397e-07]
for Delta4=0.2Pi:
q-binned i2minus, unnormalised=  [-8.588779851954573e-09, 1.0314293377993209e-07, 1.765285124973161e-07]
################################################
################################################

at best fit:
q-binned i3 unnormalised=  [-1.7965846789851064e-08, -1.3084965088000847e-08, -6.43638008380601e-07, -4.277572720597636e-07, -1.2250750934568575e-06, -1.135615695813615e-06, -2.2992948160884815e-08]
q-binned i3, unnormalised=                                                                           [-4.2775727205976364e-07, -1.2250750934568575e-06, -1.1356156958136152e-06]
at delta1=-0.8Pi: (lower limit of delta1)
q-binned i3 unnormalised=  [-1.878549482555947e-08, -1.3667102221220735e-08, -6.755973947104807e-07, -4.091009136023038e-07, -1.2354770633324126e-06, -1.1861245230444867e-06, -2.51395202220737e-08]
q-binned i3, unnormalised=                                                                          [-4.291152021296758e-07, -1.2354557758901931e-06, -1.1858921400259463e-06]
at delta1=-0.4Pi: (upper limit of delta1) 
q-binned i3 unnormalised=  [-1.5070163981212116e-08, -1.1148494298016927e-08, -5.646803899088796e-07, -5.278303444470818e-07, -1.3335740459442772e-06, -9.757321334149439e-07, -1.3724456409073097e-08]
q-binned i3, unnormalised=                                                                           [-5.039795594986987e-07, -1.333773311017453e-06, -9.76128395066387e-07]
for phioml-phirhol =  0.6 *Pi:
q-binned i3, unnormalised=                                                                           [-3.5700648215257656e-07, -1.2250535841782438e-06, -1.136313889567858e-06]
for phioml-phirhol =  -0.3 *Pi:
q-binned i3, unnormalised=                                                                           [-4.5121817534517793e-07, -1.2248341994163592e-06, -1.1351425268910535e-06]

WRONG because it was still using the simplification argWsigma=0 always 
for phis=3.4:
q-binned i4 scalar, unnormalised=  [-1.3245384463639801e-08, -7.015509838125307e-09, 1.1146508436788792e-07, 2.2187970799061426e-07, -5.841890544942447e-07, 1.81672340449226e-07, 9.321332171371571e-09]
q-binned i4 scalar, unnormalised=  [-1.3245384463639801e-08, -7.015509838125307e-09, 1.1146508436788792e-07, 2.2187970799061426e-07, -5.841890544942447e-07, 1.81672340449226e-07, 9.321332171371571e-09]
for phis=3.4-pi/2:
q-binned i4 scalar, unnormalised=  [1.5573455580335786e-08, 9.201514190017622e-09, 5.427568977530946e-07, 1.2324710687635392e-07, 2.0290885206843343e-07, 5.060676207540863e-07, 3.984708407563956e-09]
for relative phase bt S-P wave set to zero: (phirhol-phirhols=0):
q-binned i4 scalar, unnormalised=                                                                         [7.707221852828734e-08, -5.644486664947486e-07, -2.1458252283660832e-07]

The correct ones are:
for phirhol=phirhols=0:
q-binned i4 scalar, unnormalised=                                                                         [-3.7614647893872875e-09, -7.135341343145777e-07, -5.648279273060901e-07]
for phirhols=pi:
q-binned i4 scalar, unnormalised=                                                                         [3.761464789387262e-09, 7.135341343145775e-07, 5.648279273060898e-07]
for phirhols=np.pi/2:
q-binned i4 scalar, unnormalised=                                                                         [-1.7324831142746582e-07, -8.234956456730127e-08, -1.4008872988692727e-07]
q-binned i4 scalar, unnormalised=                                                                         [1.7324831142746585e-07, 8.234956456730134e-08, 1.4008872988692727e-07] (for 3pi/2)
for phirhols=np/pi/3:
q-binned i4 scalar, unnormalised=                                                                         [-1.5191557854240353e-07, -4.2808768863319296e-07, -4.0382673946403023e-07]
np.cos(np.pi/3)*(i4 @phirhols=0)+np.sin(np.pi/3)*(i4@phirhols=pi/2)=                                      [-1.51918171e-07 -4.28083882e-07 -4.03734363e-07] OK.
for phirhol=2.43524:
q-binned i4 scalar, unnormalised=  [1.1534542034719406e-07, 5.962651198434861e-07, 5.207011755535344e-07] also passes the test. OK



********************I4 plus LOOK FROM HERE ON ******************************************888
For phirhol=phirhols=0 we now vary the phases $Delta_i$:
for everything at b.f.p.:
q-binned i4 scalar, unnormalised=  [-3.7614647893872875e-09, -7.135341343145777e-07, -5.648279273060901e-07]
for Delta1=-0.9Pi:
q-binned i4 scalar, unnormalised=  [-1.1894438374382742e-08, -4.6878724729387535e-07, -3.787140485668034e-07]
for Delta1=-0.8Pi:
q-binned i4 scalar, unnormalised=  [-9.56165329502941e-09, -6.209224367663936e-07, -4.907867045991014e-07]
for Delta1=-0.5Pi:
q-binned i4 scalar, unnormalised=  [8.512499038291045e-09, -6.432739988027581e-07, -5.309448562756069e-07]
################################################################################for Delta1=-0.4Pi: it is outside the range
#################################################################################q-binned i4 scalar, unnormalised=  [1.6261232595064545e-08, -5.035851980128428e-07, -4.412684375273741e-07]
for Delta3=bfp+pi:  
#######################################################3q-binned i4 scalar, unnormalised=  [-7.815633893547772e-08, 6.934171431645654e-07, 5.638844121805407e-07] 
########################################################################for Delta3=bfp-pi/2: 
######################################################################q-binned i4 scalar, unnormalised=  [-1.744896499748529e-08, -1.0612643290511898e-07, -1.1509484767847739e-07]
#######################################################################for Delta3=2.1*np.pi:
######################################################################q-binned i4 scalar, unnormalised=  [-5.918279136763e-09, -3.4694845993541336e-07, -3.0590397845764363e-07]
for Delta3=-0.4*np.pi:
q-binned i4 scalar, unnormalised=  [-6.75275060041124e-08, 6.149298305482746e-07, 4.877378206905049e-07]
for Delta3=1.2*np.pi:
q-binned i4 scalar, unnormalised=  [-8.248086858790198e-08, 5.034533564330599e-07, 4.408509975251903e-07]
for Delta2=-0.6Pi:
q-binned i4 scalar, unnormalised=  [6.092783057146525e-09, -7.129539713629935e-07, -5.651543724509255e-07]
for Delta2=0.3Pi:
q-binned i4 scalar, unnormalised=  [-4.156299238769489e-08, -7.135507318253724e-07, -5.642279164071079e-07]
for Delta4=0.2Pi:
q-binned i4 scalar, unnormalised=  [-7.454899370735052e-08, -7.1377298799029e-07, -5.593181958394511e-07]
for Delta4=0.6Pi:
q-binned i4 scalar, unnormalised=  [1.483092504316566e-07, -7.168443259630052e-07, -5.651176191296122e-07]

For phirhols=pi/2, phirhol=0 we now vary the phases $Delta_i$:
for everything at b.f.:
q-binned i4 scalar, unnormalised=  [-1.7324831142746582e-07, -8.234956456730127e-08, -1.4008872988692727e-07]
for Delta1=-0.9Pi:
q-binned i4 scalar, unnormalised=  [-1.8815962671668586e-07, -5.681399077025897e-07, -4.6820886861393584e-07]
for Delta1=-0.5Pi:
q-binned i4 scalar, unnormalised=  [-1.6744111670218962e-07, 3.4857994796768843e-07, 1.6057490599517887e-07]
for Delta3=-0.4*np.pi:
q-binned i4 scalar, unnormalised=  [-2.3175584540422251e-07, 3.5061432669319203e-07, 2.798318426830277e-07]
for Delta3=1.2Pi:
q-binned i4 scalar, unnormalised=  [-1.822837965084908e-07, -4.7657102377002727e-07, -3.955353882394942e-07]
for Delta2=-0.6Pi:
q-binned i4 scalar, unnormalised=  [-1.3489871519619098e-07, -8.242341250659935e-08, -1.4067073388272606e-07]
for Delta2=0.3Pi:
q-binned i4 scalar, unnormalised=  [-1.6968508896065887e-07, -8.178794404672445e-08, -1.4031052460634344e-07]
for Delta4=0.6Pi:
q-binned i4 scalar, unnormalised=  [-2.6511867120502573e-07, -7.739516965980221e-08, -1.4898020670270177e-07]
for Delta4=0.2Pi:
q-binned i4 scalar, unnormalised=  [-5.3841353875686704e-09, -8.845755092401916e-08, -1.331307270732932e-07]






*******************************I4 minus but OBSOLETE******************************************
(checked that it doesn't change with a change of phis) 
q-binned i4 vector, unnormalised=  [1.205712745535296e-07, 6.827581898142515e-08, 2.2497552714687964e-06, 1.1856947293361024e-06, 2.478898757389924e-06, 2.2662020798716948e-06, 4.3848422783008836e-08]
q-binned i4 vector, unnormalised=                                                                        [1.1856947293361029e-06, 2.4788987573899237e-06, 2.266202079871695e-06]
for phirhol-phiphil = - 0.8 *Pi:
q-binned i4 vector, unnormalised=                                                                        [1.1932221157278848e-06, 2.498833922932907e-06, 2.3655171414231593e-06]
for phirhol-phiphil = -0.4 *Pi:
q-binned i4 vector, unnormalised=                                                                        [1.3757846333512024e-06, 2.7051141043161797e-06, 1.952172698418067e-06]
for phioml-phirhol =  0.6 *Pi:
                                                                                                       [9.987017386883881e-07] 
for phioml-phirhol =  -0.3 *Pi:                                                                         [1.2454595087968933e-06 ]                               
                                                                                                       
for phis=3.4:
q-binned i8 scalar, unnormalised=  [9.714500090840612e-09, 5.505381045121688e-09, 3.078334749235187e-07, 7.521771582058878e-08, 7.089875782805188e-08, 2.1599718562187982e-07, 1.4295233427156983e-09]
for phis=3.4-pi/2:
q-binned i8 scalar, unnormalised=  [9.471923992105768e-09, 4.880170273155028e-09, -3.2523489176819186e-08, -1.0574108155067341e-07, 2.5351383690713654e-07, -6.288337616830921e-08, -3.285497480632236e-09]
for phis=3.4-pi:
q-binned i8 scalar, unnormalised=  [-9.714500090840612e-09, -5.505381045121687e-09, -3.078334749235187e-07, -7.521771582058875e-08, -7.089875782805181e-08, -2.1599718562187982e-07, -1.4295233427156985e-09]

for the new way of writing things:

**********************I8 minus*******************************************
Keeping phirhol=phirhols=0:
at best fit point:
q-binned i8 scalar, unnormalised=  [ 8.752704979534731e-08, 1.740964151182447e-08, 4.4917796272535366e-08]
for Delta1=-0.9Pi:
q-binned i8 scalar, unnormalised=  [9.450674148038081e-08, 2.297678049585216e-07, 1.8653571415235954e-07]
for Delta1=-0.5Pi:
q-binned i8 scalar, unnormalised=  [8.537867035676429e-08, -1.6372369699852114e-07, -8.035564816177443e-08]
for Delta2=-0.6Pi:
q-binned i8 scalar, unnormalised=  [7.196408668083475e-08, 1.7369102034241612e-08, 4.557197165725808e-08]
for Delta2=0.3Pi:
q-binned i8 scalar, unnormalised=  [8.782874369040972e-08, 1.661028556360804e-08, 4.5133381290651624e-08]
for Delta3=-0.4*np.pi:
q-binned i8 scalar, unnormalised=  [1.1265727732238014e-07, -1.3413724773167813e-07, -1.0558666606562837e-07]
for Delta3=1.2Pi:
q-binned i8 scalar, unnormalised=  [8.742811306007755e-08, 2.1479968085255544e-07, 1.7544646897246516e-07]
for Delta4=0.6Pi:
q-binned i8 scalar, unnormalised=  [1.4325955701437185e-07, 1.5174705556101936e-08, 4.848230501600526e-08]
for Delta4=0.2Pi:
q-binned i8 scalar, unnormalised=  [-2.1576701966739474e-09, 2.0049407393777538e-08, 4.2130542601281036e-08]


Keeping phirhol=0, phirhols=np.pi/2:
bfp:
q-binned i8 scalar, unnormalised=  [-1.3161444898152481e-08, -3.0534952864250726e-07, -2.3931207972268477e-07]
for Delta1=-0.9Pi:
q-binned i8 scalar, unnormalised=  [-1.8226333897378902e-08, -2.137499259175501e-07, -1.6872439535951315e-07]
for Delta1=-0.5Pi:
q-binned i8 scalar, unnormalised=  [-6.6786331259454715e-09, -2.646961524697489e-07, -2.1832708462600402e-07]
for Delta2=-0.6Pi:
q-binned i8 scalar, unnormalised=  [-1.1024981710284724e-08, -3.0449782418414745e-07, -2.396433670881498e-07]
for Delta2=0.3Pi:
q-binned i8 scalar, unnormalised=  [-2.8213006113432235e-08, -3.0551596077928715e-07, -2.386429759809326e-07]
for Delta3=-0.4Pi:
q-binned i8 scalar, unnormalised=  [-4.798160975873379e-08, 2.6998076611008677e-07, 2.1039198549644246e-07]
for Delta3=1.2Pi:
q-binned i8 scalar, unnormalised=  [-5.244784075462931e-08, 2.023418874060512e-07, 1.7478721984665037e-07]
for Delta4=0.6Pi:
q-binned i8 scalar, unnormalised=  [5.8910572793878744e-08, -3.066895106753655e-07, -2.396441547808597e-07]
for Delta4=0.2Pi:
q-binned i8 scalar, unnormalised=  [-3.9326650472774477e-08, -3.0567003153899143e-07, -2.3688790870437156e-07]


#############################################################################

q-binned i8 vector, unnormalised=  [-3.211796817741571e-10, -1.1491344246631323e-10, -6.890633594040546e-10, 3.431946417657599e-09, -6.436009228480746e-10, 2.1058138610748654e-09, 2.1076949783207052e-10]

q-binned i9 unnormalised=  [1.6682029837438846e-10, 7.503332311629627e-11, 2.533860875497021e-10, -2.4095986179632614e-09, 6.550954632586156e-10, -2.220866812555714e-09, -2.2537188068419318e-10]


*****************************************************************************************
for phis=3.4
q-binned i5 scalar, unnormalised=  [3.0446686455425774e-07, 1.12156037743008e-07, 1.1435550584315751e-06, -1.476410438173946e-07, 4.776559581500937e-07, 2.238897087212758e-08, -4.244178719225024e-08]
q-binned i5 vector, unnormalised=  [-7.81355187723138e-07, -2.614218021538063e-07, 1.0811135273917857e-06, 4.1953031693778125e-06, -9.979518892754605e-07, 1.5879760521415795e-06, 2.507916972312101e-07]

at the best fit point with phirhol=phirhols=0:
q-binned i5 scalar, unnormalised=  [-6.288386510608947e-07, -1.798341248133265e-07, 3.050979963377353e-08]
q-binned i5 vector, unnormalised=  [-2.4881005447820264e-06, 8.92383785132938e-07, -5.615021988288854e-07]
for Delta1=-0.9Pi:
q-binned i5 scalar, unnormalised=  [-5.549598064013732e-07, -5.647400225901096e-08, -1.453093279452318e-07]
q-binned i5 vector, unnormalised=  [-2.127723412708757e-06, 1.1643968399198916e-06, -1.3832526069857039e-06]
for Delta1=-0.5Pi:
q-binned i5 scalar, unnormalised=  [-7.046993497238547e-07, -3.417725195281372e-07, 1.5186510119405653e-07]
q-binned i5 vector, unnormalised=  [-2.9477790259931576e-06, 1.4686366460092047e-07, 1.9531666035647608e-07]
for Delta2=-0.6Pi:
q-binned i5 scalar, unnormalised=  [-6.14496610721596e-07, -1.8150306812261664e-07, 2.8875653817275348e-08]
q-binned i5 vector, unnormalised=  [-2.377906207879124e-06, 8.881870304064606e-07, -5.680055053602411e-07]
for Delta2=0.3Pi:
q-binned i5 scalar, unnormalised=  [-6.212864532363828e-07, -1.8161127719221125e-07, 2.879320579029825e-08]
q-binned i5 vector, unnormalised=  [-2.3054776686684857e-06, 8.911944052306088e-07, -5.633082628613399e-07]


for Delta3=-0.4Pi:
q-binned i5 scalar, unnormalised=  [-5.926780416571489e-07, 2.1851297656410625e-07, 5.817282577842997e-08]
q-binned i5 vector, unnormalised=  [-2.4881005447820264e-06, 8.92383785132938e-07, -5.615021988288853e-07] should be the same as the best fit point, and it is. 
for Delta3=1.2Pi: 
2 next q-binned i5 scalar, unnormalised=                   [3.573883711165745e-07, -2.1853328472047954e-07, 0]

Now for phirhols=Pi/2: THIS IS USELESS FOR THE VECTOR I5
at bfp:
q-binned i5 scalar, unnormalised=  [-1.9372864796340605e-07, -7.005469509724002e-08, 2.920400625171119e-07]
q-binned i5 vector, unnormalised=  [-2.4881005447820264e-06, 8.92383785132938e-07, -5.615021988288853e-07]
for Delta1=-0.9Pi:
q-binned i5 scalar, unnormalised=  [-1.1983935371721086e-07, 5.329317691931246e-08, 1.1625285638461402e-07]
q-binned i5 vector, unnormalised=  [-2.127723412708757e-06, 1.1643968399198916e-06, -1.383252606985704e-06]
for Delta1=-0.5Pi:
q-binned i5 scalar, unnormalised=  [-2.6960015111106656e-07, -2.319936049822528e-07, 4.134209225835351e-07]
q-binned i5 vector, unnormalised=  [-2.947779025993158e-06, 1.4686366460092047e-07, 1.953166603564761e-07]
for Delta2=-0.6Pi:
q-binned i5 scalar, unnormalised=  [-1.7938271884650082e-07, -7.172358987441864e-08, 2.904059056647127e-07]
q-binned i5 vector, unnormalised=  [-2.377906207879124e-06, 8.881870304064604e-07, -5.680055053602411e-07]
for Delta2=0.3Pi:
q-binned i5 scalar, unnormalised=  [-1.86221693317793e-07, -7.183178772215689e-08, 2.9032349964957915e-07]
q-binned i5 vector, unnormalised=  [-2.3054776686684857e-06, 8.911944052306088e-07, -5.633082628613398e-07]
for Delta3=1.2Pi:
2 next q-binned i5 scalar, unnormalised=                     [4.8932835688361e-08, -9.385375077030103e-08]


for phirhol=Pi/2:
at bfp:
q-binned i5 scalar, unnormalised=  [-9.479491410299864e-07, -1.1919261987786092e-07, -2.991469174303394e-07]
q-binned i5 vector, unnormalised=  [-3.392733511486146e-06, 6.197938309076762e-07, -1.5211406308840957e-06]
for Delta1=-0.9Pi:
q-binned i5 scalar, unnormalised=  [-1.0070831511448223e-06, -2.926206170994022e-07, -2.838278366634143e-07]
q-binned i5 vector, unnormalised=  [-3.871017049356776e-06, -5.860110902459987e-07, -1.0480918679046755e-06]
for Delta1=-0.5Pi:
q-binned i5 scalar, unnormalised=  [-9.443926990802016e-07, -6.474235599788224e-08, -2.261544316942331e-07]
q-binned i5 vector, unnormalised=  [-3.2521660396417576e-06, 1.2744605530743563e-06, -1.440625495788388e-06]
for Delta2=-0.6Pi:
q-binned i5 scalar, unnormalised=  [-9.377521549191286e-07, -1.2133387960268803e-07, -3.0121864056433256e-07]
q-binned i5 vector, unnormalised=  [-3.1822312820876014e-06, 6.178733018994095e-07, -1.5240781055660247e-06]
for Delta2=0.3Pi:
q-binned i5 scalar, unnormalised=  [-9.630215382679042e-07, -1.1729127331146643e-07, -2.9728893999658085e-07]
q-binned i5 vector, unnormalised=  [-3.5286287453914147e-06, 6.24055257673495e-07, -1.5145424785712632e-06]

for phirhol=0, phirhols=Pi:
for Delta1=-0.5Pi:
2 next q-binned i5 scalar, unnormalised=                    [2.2725726736344103e-07, 1.4286289299223386e-07]

for phirhol=0, phirhols=3.4:
at bfp:
2 next q-binned i5 scalar, unnormalised=  [4.243924993300722e-07, -4.63540574657361e-08]
for Delta1=-0.9Pi:
2 next q-binned i5 scalar, unnormalised=  [5.4774730232891e-07, -2.221504207057271e-07]
for Delta1=-0.5Pi:
2 next q-binned i5 scalar, unnormalised=  [2.6242740710466216e-07, 7.502431902107627e-08]

**********************************************************************
New approach for I5 scalar

With C9P=0 (through modW=modJ=0), we isolate the effect of the deltasigmarho phase:

for phirhols=0, everything at bfp:
q-binned i5 scalar, unnormalised=  [-3.627112213054358e-07, -2.8450752789456746e-07, 4.531252221075853e-09]
for phirhols=Pi/2, everything at bfp:
q-binned i5 scalar, unnormalised=  [7.248092764902875e-08, -1.7471068351735928e-07, 2.660436065770023e-07]


With C9S=0 (through modWsigma=0) we isolate the effect of the deltarhorho phase:

for phirhol=0, everything at bfp:
q-binned i5 scalar, unnormalised=  [-2.6611531914225385e-07, 1.0467460313003825e-07, 2.5992144431161388e-08]
for phirhol=Pi/2, everything at bfp:
q-binned i5 scalar, unnormalised=  [-5.852322149943598e-07, 1.652984021501405e-07, -3.036462240224456e-07]





#############################################################################
q-binned i6, unnormalised=  [-3.663116934064214e-07, -1.5436977507655844e-07, 9.965626293864175e-07, 3.7901254730443527e-06, -1.0602344796021856e-06, 1.7137213756818466e-06, 2.707264568170357e-07]

Setting always argC10=0:
When also setting phirhol=0:
at the best fit point:
q-binned i6, unnormalised=  [-2.3080399126037538e-06, 9.560177168618388e-07, -6.097967097311099e-07]
for Delta1=-0.9Pi:
q-binned i6, unnormalised=  [-1.968912658117078e-06, 1.2379038318840947e-06, -1.4942147207066623e-06]
for Delta1=-0.5Pi:
q-binned i6, unnormalised=  [-2.7407387591463833e-06, 1.7122672826647119e-07, 2.0562515851982323e-07]
for Delta2=-0.6Pi:
q-binned i6, unnormalised=  [-2.201481640380858e-06, 9.523758102044084e-07, -6.164807096968036e-07]
for Delta2=0.3Pi:
q-binned i6, unnormalised=  [-2.1411542615845357e-06, 9.54987254111916e-07, -6.116527751005597e-07]

For phirhol=Pi/2:
q-binned i6, unnormalised=  [-3.027552135835387e-06, 6.53458128763773e-07, -1.6392062145385495e-06]
for Delta1=-0.9Pi:
q-binned i6, unnormalised=  [-3.4779114433853342e-06, -6.223673212841558e-07, -1.1282064394526119e-06]
for Delta1=-0.5Pi:
q-binned i6, unnormalised=  [-2.895070735808228e-06, 1.3489977941427934e-06, -1.5537689786569039e-06]
for Delta2=-0.6Pi:
q-binned i6, unnormalised=  [-2.8343677111865147e-06, 6.517925558912387e-07, -1.6422251165404028e-06]
for Delta2=0.3Pi:
q-binned i6, unnormalised=  [-3.1573769299242524e-06, 6.571568474681937e-07, -1.6324247618823745e-06]


q-binned i7 scalar, unnormalised=  [-2.6903338038758634e-07, -1.0713594983565963e-07, -1.4863990665344683e-06, -2.0947704657931116e-09, 5.63499035602507e-07, -1.4304660414100554e-07, -5.256084074989094e-09]

for phirhol=0, phirhols=0:
for Delta1=-0.9Pi:
q-binned i7 scalar, unnormalised=  [-1.275161445244755e-06, 3.846854535871293e-07, -1.3318304934432122e-06]

for phirhol=0,phirhols=3.4:
for Delta1=-0.9Pi:
q-binned i7 scalar, unnormalised=[-9.942775696358575e-07, -3.2043594196213787e-07, -6.428612757183431e-08]
at bfp:
q-binned i7 scalar, unnormalised=  [-8.635682461488451e-07, 1.0092707602852869e-07, -1.2276802786430273e-07]
for Delta1=-0.5Pi:
q-binned i7 scalar, unnormalised=  [-8.433490214725208e-07, 2.536745149679726e-07, 3.920523688005588e-08]

for phirhol=0, phirhols=np.pi/2:
for Delta1=-0.9Pi:
q-binned i7 scalar, unnormalised=  [-1.9294280605237372e-06, -6.866511469095271e-07, -7.049069877964993e-07]
for phirhol=0, phirhols=np.pi/4:
for Delta1=-0.9Pi:
q-binned i7 scalar, unnormalised=  [-1.7590054092850766e-06, -1.9038910329115903e-07, -1.1546710483046402e-06]
for phirhol=0,phirhols=3*np.pi/4:
for Delta1=-0.9Pi:
q-binned i7 scalar, unnormalised=  [-1.6865999432879251e-06, -8.133853845112866e-07, -2.460168530673442e-07]
**********************************************88

New approach for I7 scalar

With C9P=0 (through modW=modJ=0), we isolate the effect of the deltasigmarho phase:

for phirhols=0, everything at bfp:
q-binned i7 scalar, unnormalised=  [-5.1284686110996195e-08, 4.4053311659180796e-07, -6.425143458253759e-07]
for phirhols=Pi/2:
q-binned i7 scalar, unnormalised=  [-7.054503977386191e-07, -6.308335856891953e-07, -1.5596164524707383e-08]
With C9S=0 (through modWsigma=0) we isolate the effect of the deltarhorho phase:

for phirhol=0, all else at bfp:
q-binned i7 scalar, unnormalised=  [-1.0933342942433723e-06, 3.6562050763129535e-07, -7.479344068597128e-07]
for phirhol=Pi/2:
q-binned i7 scalar, unnormalised=  [6.591015269141195e-07, -2.660371782504902e-07, -1.9156574816895906e-08]


###########################################################################################
NP observables, not null tests
###########################################################################################

NP q-binned gammas, unnormalised=  [8.620620198616004e-05, 1.756916352673817e-05, 0.0001127382526817593, 9.783317375287512e-05, 3.514646223720497e-05, 2.903711169364123e-05, 2.6730832227078314e-05]


NP q-binned i2plus, unnormalised=  [-1.526453117056058e-05, -3.6139365225355145e-06, -2.065876708763708e-05, -1.3547597157147221e-05, -3.991230112890651e-06, -3.312101807383887e-06, -4.429871802487086e-06]
NP q-binned i2minus, unnormalised=  [8.674498082666256e-06, 2.158495061295427e-06, 1.3189058947481645e-05, 9.63622525916557e-06, 2.9819889196850736e-06, 2.404645279393384e-06, 2.959555317310299e-06]

NP q-binned i3 unnormalised=  [-1.1017518669030484e-06, -4.980689835158329e-07, -5.680366965260011e-06, -8.986179019946518e-06, -4.300806151120223e-06, -3.8392910209722285e-06, -2.9054505028605437e-06]

NP q-binned i4 scalar, unnormalised=  [-2.686087319437375e-06, -8.619250929323145e-07, -6.456835093174321e-06, -5.918521116211407e-06, -2.03504381480058e-06, -1.6893806390890944e-06, -2.153982038896734e-06]
NP q-binned i4 vector, unnormalised=  [7.622801918267585e-06, 2.5907126989791567e-06, 2.1406452659115365e-05, 2.337656641295929e-05, 9.120904751195027e-06, 7.472722101520944e-06, 5.579942520801178e-06]


NP q-binned i8 scalar, unnormalised=  [-3.883119698719336e-07, -1.4163474195068903e-07, -1.2765106584398622e-06, -1.5408068129590855e-06, -6.401738165708783e-07, -5.928752518117121e-07, -6.569275949236395e-07]
NP q-binned i8 vector, unnormalised=  [0.0, 0.0, 0.0, 0.0, 0.0, 0.0, 0.0]



***************************************************************************************
Definitions 
***************************************************************************************

The programme calculates (modulo some signs) 
I2+, I2- \\
I3 \\
2/pi I4+, 3/2 I4- \\
2/pi I5+, 3/2 I5- \\
I6 \\
2/pi I7+, 3/2 I7- \\ 
2/pi I8+, 3/2 I8- \\

On the numerical results side, the signs of I5, I6 should be flipped for the P-P interference case. I4(P-P) stays the same. I4(S-P) should be flipped. I2(S-P) should be flipped. I8(S-P) stays the same. I5(S-P) stays the same. I7(S-P) should be flipped.

==> isospinargument.tex <==
\section{Isospin phases}

If we assign the phase to the vertices $D\rightarrow \rho\rho$ and $D\rightarrow \rho\omega$ then, following similar steps as in the 2-body decays, we have that
\begin{itemize}
    \item The operator is the same in both cases and is $T_{1/2}+T_{3/2}$
    \item The $D$ is $1/2,-1/2$
    \item Together they make final states with either $I=0,1$ or 2. 
    \item $\rho\rho=-\frac{1}{\sqrt{3}}\ket{0,0}+\frac{\sqrt{2}}{3}\ket{2,0}$ whereas $\rho\omega=\ket{1,0}$ and $\omega\omega=\ket{0,0}$.
\end{itemize}

The $\rho\rho$ part is OK if $\delta_\rho\equiv\delta_{\rho\rho}$ and the omega phase that enters the hadronic part is $\phi_\omega\equiv \delta_{\omega\rho}-\delta_{\rho\rho}$. To bring the whole W-contribution in the form that we have it now, $b_\rho(1+a_\omega e^{i\phi_\omega})(f/P_\rho e^{i\delta_\rho}-1/3 f/P_\omega e^{i\delta_\omega} )$, we need that $\delta_{\omega\omega}-\delta_{\rho\omega}=\delta_{\omega\rho}-\delta_{\rho\rho}$. Notice that this isn't very likely, since $\delta_{\rho\omega}=\delta_{\omega\rho}$.



[discussion on the origin of the relative signs of $\rho$ and $\omega$]If we assign the phase at the current matrix element
\begin{equation}
    <V|\overline{d}d|0>
\end{equation}
then in the case of $\rho$ it is 
\begin{equation}
    <1,0|\frac{1}{\sqrt{2}}(-|1,0>+|0,0>)=-\frac{1}{\sqrt{2}} A_1
\end{equation}
whereas for $\omega$\begin{equation}
    <0,0|\frac{1}{\sqrt{2}}(-|1,0>+|0,0>)=\frac{1}{\sqrt{2}} A_0
\end{equation}



==> old_tables_new_tables_full_digits.tex <==
\begin{table}[h!]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{|lc|c|c|c|c|}
        \hline
        \multicolumn{2}{|c|}{\multirow{2}{*}{$ \int \langle I_i \rangle_{+}^r / \Gamma^r $}} & \multicolumn{2}{c|}{SM: $ C_9^{\rm NP} = C_9' $} & \multicolumn{2}{c|}{NP: $ \tilde{C}_{10} = 0.43 $,} \\
         & & \multicolumn{2}{c|}{$ = C_{10} = C_{10}' = 0 $} & \multicolumn{2}{c|}{$ C_9^{\rm NP} = C_9' = C_{10}' = 0 $} \\
        \cline{3-6}  
        $i$ & $S$-wave & WCs & value (\%) & WCs & value (\%)\\
        \hline
        $ 1^\dagger $ & \gr{$ \circ $} & $ | C_9^{{\rm eff}: S} |^2 $, $ | C_9^{{\rm eff}: P} |^2 $ &  46   & SM $ + \, | C_{10} |^2 $ &  46 \\
        \hline
        $ 2^\dagger $ & \gr{$ \circ $} & $ | C_9^{{\rm eff}: S} |^2 $, $ | C_9^{{\rm eff}: P} |^2 $ &  -13 & SM $ + \, | C_{10} |^2 $ &  -13 \\
        \hline
        $ 3^\dagger $ &  \rd{$ \times $} & $ | C_9^{{\rm eff}: P} |^2 $ &  -11 & SM $ + \, | C_{10} |^2 $ &  -11\\
        \hline
        $4$ & \gr{$ \checkmark $} & $ C_9^{{\rm eff}: S} \, (C_9^{{\rm eff}: P})^\ast $ &  $\pm 8$ & SM $ + \, | C_{10} |^2 $ &  $\pm 8$ \\
        \hline
        $5$ & \gr{$ \checkmark $} & -- & $ 0 $ & $ C^{{\rm eff}: S}_9 \, C_{10}^\ast + C_{10} \, (C^{{\rm eff}: P}_9)^\ast $ &  0.1 \\
        \hline
        $ 6^\dagger $ &  \rd{$ \times $} & -- & $ 0 $ & $ \text{Re} \left[ C^{{\rm eff}: P}_9 \, C_{10}^\ast \right] $ &  0.8 \\
        \hline
        $7$ & \gr{$ \checkmark $} & -- & $ 0 $ & $ C^{{\rm eff}: S}_9 \, C_{10}^\ast + C_{10} \, (C^{{\rm eff}: P}_9)^\ast $ &  0.1 \\
        \hline
        $8$ & \gr{$ \checkmark $} & $ C_9^{{\rm eff}: S} \, (C_9^{{\rm eff}: P})^\ast $ &  $\pm 4$ & SM $ + \, | C_{10} |^2 $ &  $\pm 4$ \\
        \hline
        $ 9^\dagger $ &  \rd{$ \times $} & $ | C_9^{{\rm eff}: P} |^2 $ & $ \sim 0 $ & SM $ + \, | C_{10} |^2 $ & $\sim 0$ \\
        \hline
    \end{tabular}
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \vspace{3mm}
    \begin{tabular}{|lc|c|c|c|c|}
        \hline
        \multicolumn{2}{|c|}{\multirow{2}{*}{$ \int \langle I_i \rangle_{-}^r / \Gamma^r $}} & \multicolumn{2}{c|}{SM: $ C_9^{\rm NP} = C_9' $} & \multicolumn{2}{c|}{NP: $ \tilde{C}_{10} = 0.43 $,} \\
         & & \multicolumn{2}{c|}{$ = C_{10} = C_{10}' = 0 $} & \multicolumn{2}{c|}{$ C_9^{\rm NP} = C_9' = C_{10}' = 0 $} \\
        \cline{3-6}
        $i$ & $S$-wave & WCs & value (\%)& WCs & value (\%)\\
        \hline
        $1$ & \gr{$ \checkmark $} & $ C_9^{{\rm eff}: S} \, (C_9^{{\rm eff}: P})^\ast $ &  $\mp 8$ & SM $ + \, | C_{10} |^2 $ &  $\mp 8$ \\
        \hline
        $2$ & \gr{$ \checkmark $} & $ C_9^{{\rm eff}: S} \, (C_9^{{\rm eff}: P})^\ast $ &  $\pm 8$ & SM $ + \, | C_{10} |^2 $ &  $\pm 8$ \\
        %\hline
        %$I_3$ & $ | C_9^{\rm eff} |^2 $ & 0 & $ | C_9^{\rm eff} |^2 + | C_{10} |^2 $ & 0 \\ %always vanishes
        \hline
        $4^\dagger$ &  \rd{$ \times $} & $ | C_9^{{\rm eff}: P} |^2 $ &  16 & SM $ + \, | C_{10} |^2 $ &  16 \\
        \hline
        $5^\dagger$ &  \rd{$ \times $} & -- & $ 0 $ & $ \text{Re} \left[ C^{{\rm eff}: P}_9 \, C_{10}^\ast \right] $ &  0.6 \\
        %\hline
        %$I_6$ & $ 0 $ & 0 & $ \text{Re} \left[ C^{\rm eff}_9 \, C_{10}^\ast \right] $ & 0 \\ %always vanishes
        \hline
        $7^\dagger$ &  \rd{$ \times $} & -- & $ 0 $ & $ \text{Re} \left[ C^{{\rm eff}: P}_9 \, C_{10}^\ast \right] $ & $ \sim 0 $ \\
        \hline
        $8^\dagger$ &  \rd{$ \times $} & $ | C_9^{{\rm eff}: P} |^2 $ & $ \sim 0 $ & SM $ + \, | C_{10} |^2 $ & $\sim 0$ \\
        %\hline
        %$I_9$ & $ | C_9^{\rm eff} |^2 $ & 0 & $ | C_9^{\rm eff} |^2 + | C_{10} |^2 $ & 0 \\ %always vanishes
        \hline
    \end{tabular}
    \caption{%[Not yet including a discussion about J-type contribution: use effective description]
    Summary of the angular observables: the upper table contains $\langle \cdot \rangle_+$ quantities, while the lower one $\langle \cdot \rangle_-$ quantities. In the first column, a tick \gr{$ \checkmark $} indicates an $S$-wave effect through its interference with the $P$-wave, an empty circle \gr{$ \circ $} means that the $S$-wave manifests through an additive term to the $P$-wave instead of an interference term, and a cross  \rd{$ \times $} indicates the absence of any $S$-wave effect. The SM dependences on the effective Wilson coefficients (WCs) are given in the second column along with a typical value found for the integrated observables in the SM. The integration range considered is $ (0.78 \, \text{GeV})^2 < q^2 (\ell^+ \ell^-) < (1.1 \, \text{GeV})^2 $.
    When two signs are shown, they correspond to different relative phases of the $S$- and $P$-waves.
    The third column indicates the dependence on the effective SM and on the NP WCs in the presence of a non-vanishing $ \tilde{C}_{10} = V_{ub} V_{cb}^\ast C_{10} $, taken at its current upper bound, along with a typical value for the integrated observables.
    The hermitian conjugate is also understood when the displayed combination of WCs is possibly complex.
    Cases carrying a dagger $\dagger$ indicate quantities already measured by LHCb \cite{LHCb:2021yxk,LHCb_supplementary_material_aps,LHCb_supplementary_material_4}.
    %[\LVS{what is the observable for which numerical values are given?, no overall multiplicative factor I guess}]
    [\LVS{compare to other tables}]
    %[I am not sure how to quote ranges (perhaps varying $\Delta_1$? it would underestimate the error for angular observables sensitive to the S-wave)]
    %[I think this table should be kept in the main text with $ q^2_{\ell \ell} \gtrsim m_\rho^2 $ and a favorable $\phi_\phi-\phi_\rho$, while binned cases for different strong phase differences should be given in longer tables in the appendices for reference]
    %[ What is the region in $p^2$, $q^2$ being considered??; how ranges are being determined (variation of complex phases?)??; review unit being shown and put in \%; PREPARE longer table with smaller bins}]
    %[ NOTE THAT LHCb's $ \langle S_{2, 5, 6, 7, 8} \rangle $ are consistent with zero, thus setting constraints on the $P$-wave through $\langle I_2 \rangle_{+}$ and $\langle I_7 \rangle_{-}$; LHCb's $ \langle S_{3, 4, 9} \rangle $ displays some deviation from zero, thus setting constraints on the $P$-wave through $ \langle I_3 \rangle_{+} $ and $ \langle I_4 \rangle_{-} $, while $ \langle S_9 \rangle $ vanishes in the SM; what are our predictions for them???}]
    %[ NOTE THAT the $P$- and the $S$-wave cases for 5 and 7 are both sensitive in the same way to $C_{10}$: however, it is possible that due to interferences the $S$-wave comes with a larger pre-factor, particularly in the case of 7; at least, it is sensitive to a different systematic effect}]
    }
    \label{tab:summary_table}
    %[ NOTE THAT LHCb's $ \langle A_{2, 3, 4, 5, 6, 7, 8, 9} \rangle $ are consistent with zero, thus setting constraints on the $P$-wave through $ \text{Im} \left( \mathcal{F}_P \mathcal{F}^\ast_\perp \right) $ and $ \text{Im} ( \mathcal{F}_\perp \mathcal{F}^\ast_\Vert ) $}; these are CP-violating quantities]
    %[ IS IT better to look at $ C_{10}' $??, first decide on size of interference terms}; we won't dedicate much effort to NP]
\end{table}

\begin{table}
    \centering
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{|lc|c|c|c|c|}
        \hline
        \multicolumn{2}{|c|}{\multirow{2}{*}{$ \int \langle I_i \rangle_{+}^r / \Gamma^r $}} & \multicolumn{2}{c|}{SM: $ C_9^{\rm NP} = C_9' $} & \multicolumn{2}{c|}{NP: $ \tilde{C}_{10} = 0.43 $,} \\
         & & \multicolumn{2}{c|}{$ = C_{10} = C_{10}' = 0 $} & \multicolumn{2}{c|}{$ C_9^{\rm NP} = C_9' = C_{10}' = 0 $} \\
        \cline{3-6}  
        $i$ & $S$-wave & WCs & value (\%) & WCs & value (\%)\\
        \hline
        $ 1^\dagger $ & \gr{$ \circ $} & $ | C_9^{{\rm eff}: S} |^2 $, $ | C_9^{{\rm eff}: P} |^2 $ &  48   & SM $ + \, | C_{10} |^2 $ &  48 \\
        \hline
        $ 2^\dagger $ & \gr{$ \circ $} & $ | C_9^{{\rm eff}: S} |^2 $, $ | C_9^{{\rm eff}: P} |^2 $ & -7  & SM $ + \, | C_{10} |^2 $ &  -7 \\
        \hline
        $ 3^\dagger $ &  \rd{$ \times $} & $ | C_9^{{\rm eff}: P} |^2 $ & -14 & SM $ + \, | C_{10} |^2 $ & -14 \\
        \hline
        $4$ & \gr{$ \checkmark $} & $ C_9^{{\rm eff}: S} \, (C_9^{{\rm eff}: P})^\ast $ & $\pm 2$ & SM $ + \, | C_{10} |^2 $ & $\pm 2$  \\
        \hline
        $5$ & \gr{$ \checkmark $} & -- & $ 0 $ & $ C^{{\rm eff}: S}_9 \, C_{10}^\ast + C_{10} \, (C^{{\rm eff}: P}_9)^\ast $ & $\pm 0.1$ (updated)  \\
        \hline
        $ 6^\dagger $ &  \rd{$ \times $} & -- & $ 0 $ & $ \text{Re} \left[ C^{{\rm eff}: P}_9 \, C_{10}^\ast \right] $ & $\pm 0.3$ (updated) \\
        \hline
        $7$ & \gr{$ \checkmark $} & -- & $ 0 $ & $ C^{{\rm eff}: S}_9 \, C_{10}^\ast + C_{10} \, (C^{{\rm eff}: P}_9)^\ast $ & $\pm 0.4$ (updated)  \\
        \hline
        $8$ & \gr{$ \checkmark $} & $ C_9^{{\rm eff}: S} \, (C_9^{{\rm eff}: P})^\ast $ & $\pm 1$ & SM $ + \, | C_{10} |^2 $ & $\pm 1$  \\
        \hline
        $ 9^\dagger $ &  \rd{$ \times $} & $ | C_9^{{\rm eff}: P} |^2 $ & $ \sim 0 $ & SM $ + \, | C_{10} |^2 $ & $\sim 0$ \\
        \hline
    \end{tabular}
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \vspace{3mm}
    \begin{tabular}{|lc|c|c|c|c|}
        \hline
        \multicolumn{2}{|c|}{\multirow{2}{*}{$ \int \langle I_i \rangle_{-}^r / \Gamma^r $}} & \multicolumn{2}{c|}{SM: $ C_9^{\rm NP} = C_9' $} & \multicolumn{2}{c|}{NP: $ \tilde{C}_{10} = 0.43 $,} \\
         & & \multicolumn{2}{c|}{$ = C_{10} = C_{10}' = 0 $} & \multicolumn{2}{c|}{$ C_9^{\rm NP} = C_9' = C_{10}' = 0 $} \\
        \cline{3-6}
        $i$ & $S$-wave & WCs & value (\%)& WCs & value (\%)\\
        \hline
        $1$ & \gr{$ \checkmark $} & $ C_9^{{\rm eff}: S} \, (C_9^{{\rm eff}: P})^\ast $ & $\mp 2$ & SM $ + \, | C_{10} |^2 $ & $\mp 2$  \\
        \hline
        $2$ & \gr{$ \checkmark $} & $ C_9^{{\rm eff}: S} \, (C_9^{{\rm eff}: P})^\ast $ & $\pm 2$  & SM $ + \, | C_{10} |^2 $ & $\pm 2$  \\
        %\hline
        %$I_3$ & $ | C_9^{\rm eff} |^2 $ & 0 & $ | C_9^{\rm eff} |^2 + | C_{10} |^2 $ & 0 \\ %always vanishes
        \hline
        $4^\dagger$ &  \rd{$ \times $} & $ | C_9^{{\rm eff}: P} |^2 $ & 20  & SM $ + \, | C_{10} |^2 $ &  20 \\
        \hline
        $5^\dagger$ &  \rd{$ \times $} & -- & $ 0 $ & $ \text{Re} \left[ C^{{\rm eff}: P}_9 \, C_{10}^\ast \right] $ & $\pm 0.2$ (updated)  \\
        %\hline
        %$I_6$ & $ 0 $ & 0 & $ \text{Re} \left[ C^{\rm eff}_9 \, C_{10}^\ast \right] $ & 0 \\ %always vanishes
        \hline
        $7^\dagger$ &  \rd{$ \times $} & -- & $ 0 $ & $ \text{Re} \left[ C^{{\rm eff}: P}_9 \, C_{10}^\ast \right] $ & $ \sim 0 $ \\
        \hline
        $8^\dagger$ &  \rd{$ \times $} & $ | C_9^{{\rm eff}: P} |^2 $ & $ \sim 0 $ & SM $ + \, | C_{10} |^2 $ & $\sim 0$ \\
        %\hline
        %$I_9$ & $ | C_9^{\rm eff} |^2 $ & 0 & $ | C_9^{\rm eff} |^2 + | C_{10} |^2 $ & 0 \\ %always vanishes
        \hline
    \end{tabular}
   \caption{Updated table.}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
    \centering
    \renewcommand{\arraystretch}{1.4}
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    \multirow{1}{*}{$\sqrt{q^2}$-bin} & \multirow{1}{*}{$\Gamma^r$ (SM)} & $ \frac{\Gamma_\sigma^r}{\Gamma^r} $ (\%) & $\int \langle I_2 \rangle_+^r$ (\%) & $ \frac{\int \langle I_2\rangle _{+,\sigma}^r}{\int \langle I_2\rangle_{+}^r}$ (\%) & $\int \langle I_3 \rangle_+^r$ (\%) & $\int \langle I_4 \rangle_-^r$ (\%) \\
    %\cline{3-7}
    %& & \multicolumn{5}{c|}{ (\%) } \\
    \hline 
   %%$ r^{({\rm low})} $        & 0.08 &   17  & -1.2 & 26 & -0.2 & 0.8\\ 
   %%$ r^{(\eta)} $             & 0.03 &   15  & -0.5 & 28 & -0.1 & 0.5 \\ 
   %%$ r^{(\rho: {\rm inf})} $  & 1.09 &  32  &  -18.8& 61 & -6.4 & 15.0\\
   $ r^{(\rho: {\rm sup})} $  & [0.54, 0.65] &  [35,46]   &  [-13, -9.0]& [71,81]& [-5.3, -3.6] &[6.7, 9.2]\\ %CV:0.59 %[-12.7, -9.0]
   $ r^{(\phi: {\rm inf})} $  & [0.96, 1.0] &  [25,28] &  [-12.4, -12.1] & [78,82]& [-13, -12]& [17, 18] \\ %CV:1.00 %[0.96,1.03] %[-13.3, -12.2] %[16.5, 18.1]
   $ r^{(\phi: {\rm sup})} $  & [0.79, 0.89]&  [21,25]    & [-9.0, -8.5] & [68,75]& [-12, -9.8]& [13, 16]  \\ %CV:0.85 %[-11.9, -9.8] %[13.0, 15.8]
   %%$ r^{({\rm high})} $       & 0.01 &  13 &    -0.1 & 62&  -0.2& 0.3  \\
       \hline 
    \end{tabular}
    \caption{SM predictions for the non-vanishing observables which only receive $P$-wave contributions ($\int \langle I_3 \rangle_+^r \,, \; \int \langle I_4 \rangle_-^r$), and where the effect of the $S$-wave is additive (i.e., $\Gamma^r = \Gamma^r_{\rho^0/\omega} + \Gamma^r_\sigma$ and $\int \langle I_2 \rangle_+^r = \int \langle I_2 \rangle_{+, \rho^0/\omega}^r + \int \langle I_2 \rangle_{+, \sigma}^r$); a subscript $\sigma$ indicates that only the $S$-wave is kept. The relation $ \Gamma^r = 2 \left( \int \langle I_1 \rangle_+^r - \int \langle I_2 \rangle_+^r / 3 \right) $ holds true. For comparison with LHCb \cite{LHCb:2021yxk,LHCb_supplementary_material_aps,LHCb_supplementary_material_4}, $ \langle S_2 \rangle^r = \int \langle I_2 \rangle_+^r / \Gamma^r $, $ \langle S_3 \rangle^r = \int \langle I_3 \rangle_+^r / \Gamma^r $, and $ \langle S_4 \rangle^r = \int \langle I_4 \rangle_-^r / \Gamma^r $.
    Relevant definitions can be found in Sec.~\ref{sec:observables}, see in particular Eqs.~\eqref{isnormalised} and \eqref{intnotation}.
    The decay rate and the $I_i$'s both need to be multiplied by a common constant factor, $|C_2\lambda_d e G_F/\sqrt{2}|^2\frac{e^2}{m_D} \times 10^{-5}$.
    %[\rd{can you provide for inner use unbinned plots of the angular observables as a function of $q^2$?}]
    }
    \label{gammas,i2}
\end{table}

 \begin{table}
    \centering
    \renewcommand{\arraystretch}{1.4}
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    \multirow{1}{*}{$\sqrt{q^2}$-bin} & \multirow{1}{*}{$\Gamma^r$ (SM)} & $ \frac{\Gamma_\sigma^r}{\Gamma^r} $ (\%) & $\int \langle I_2 \rangle_+^r$ (\%) & $ \frac{\int \langle I_2\rangle _{+,\sigma}^r}{\int \langle I_2\rangle_{+}^r}$ (\%) & $\int \langle I_3 \rangle_+^r$ (\%) & $\int \langle I_4 \rangle_-^r$ (\%) \\
    %\cline{3-7}
    %& & \multicolumn{5}{c|}{ (\%) } \\
    \hline 
   %%$ r^{({\rm low})} $        & 0.08 &   17  & -1.2 & 26 & -0.2 & 0.8\\ 
   %%$ r^{(\eta)} $             & 0.03 &   15  & -0.5 & 28 & -0.1 & 0.5 \\ 
   %%$ r^{(\rho: {\rm inf})} $  & 1.09 &  32  &  -18.8& 61 & -6.4 & 15.0\\
   $ r^{(\rho: {\rm sup})} $  & [6.4,8.7] &  [23,43]    & [-159,-85] & [59,78] & [-72,-47]  & [83,125]\\ %CV:0.59 %[-12.7, -9.0]
   $ r^{(\phi: {\rm inf})} $  & [16.4,18.9] & [0.3,8]    & [-110,-62]  & [3,45] & [-302,-263] & [357,414]\\ %CV:1.00 %[0.96,1.03] %[-13.3, -12.2] %[16.5, 18.1]
   $ r^{(\phi: {\rm sup})} $  & [11.9,13.4] &  [0.8,10]   & [-87,-43] &  [8,53] & [-215,-189] & [255,289]  \\ %CV:0.85 %[-11.9, -9.8] %[13.0, 15.8]
   %%$ r^{({\rm high})} $       & 0.01 &  13 &    -0.1 & 62&  -0.2& 0.3  \\
       \hline %LATEST:
   $ r^{(\rho: {\rm sup})} $  & [6.4,8.7] &  [23,43]    & [-159,-85] & [59,78] & [-72,-47]  & [83,125]\\
   $ r^{(\phi: {\rm inf})} $  & [16.4,18.9] & [0.3,8]    & [-110,-62]  & [3,45] & [-302,-263] & [357,414]\\
   $ r^{(\phi: {\rm sup})} $  & [11.9,13.4] &  [0.8,10]   & [-87,-43] &  [8,53] & [-215,-189] & [255,289]  \\
       \hline 
    \end{tabular}
\caption{Corrected fudge factor.}    
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{table}
%    \centering
%    \renewcommand{\arraystretch}{1.2}
%    \begin{tabular}{|c|c|c|c|}
%    \hline
%    $\sqrt{q^2}$-bin $r$ &  $\int \langle I_{2}\rangle_{-}^r$ (\%) & $\int \langle I_4\rangle_{+}^r$ (\%) & $\int \langle I_8\rangle_{+}^r$ (\%) \\
%    %\cline{2-4}
%    %& \multicolumn{3}{c|}{$[10^{-2}]$} \\
%    \hline 
   %%$ r^{({\rm low})} $        & 0.50 & -0.21  & 0.15  \\ 
   %%$ r^{(\eta)} $             & 0.22  & -0.11 & 0.09\\ 
   %%$ r^{(\rho: {\rm inf})} $  & -0.57 & 1.75 &  4.84\\
%   $ r^{(\rho: {\rm sup})} $ & -3.63  &  3.49 & 1.18\\ 
%   $ r^{(\phi: {\rm inf})} $  & 8.62   & -9.18& 1.11  \\
%   $ r^{(\phi: {\rm sup})} $  & -2.47 & 2.85 & 3.39\\
   %%$ r^{({\rm high})} $  &      -0.13 & 0.15 & 0.02\\
%       \hline
%    \end{tabular}
%    \caption{OLD SM predictions for the non-vanishing angular observables that probe the interference effect between the $S$- and $P$-waves. The relation $ \int \langle I_1 \rangle_-^r = - \int \langle I_2 \rangle_-^r $ holds true. The same overall multiplicative factor shown in the caption of Tab.~\ref{gammas,i2} applies. [\rd{give at most two digits}]}
%\label{i2i4i8OLD}
% \end{table}

\begin{table}
%%\hspace{-2cm}
\centering
    \renewcommand{\arraystretch}{1.4}
    %%\begin{tabular}{|c|c|c|c|}
    %%\hline
    %%$\sqrt{q^2}$-bin $r$ &  $\int \langle I_{2}\rangle_{-}^r$ (\%) & $\int \langle I_4\rangle_{+}^r$ (\%) & $\int \langle I_8\rangle_{+}^r$ (\%) \\
    %\cline{2-4}
    %& \multicolumn{3}{c|}{$[10^{-2}]$} \\
    %%\hline 
   %%$ r^{({\rm low})} $        & 0.50 & -0.21  & 0.15  \\ 
   %%$ r^{(\eta)} $             & 0.22  & -0.11 & 0.09\\ 
   %%$ r^{(\rho: {\rm inf})} $  & -0.57 & 1.75 &  4.84\\
   %%$ r^{(\rho: {\rm sup})} $ & $[-1.9,2.0] c_{SP}+ [-5.0,0.09]s_{SP}$  &  $+[-2.4,1.3]c_{SP}+[-0.08,4.2 ]s_{SP}$ & $[-2.2, 0.03]c_{SP}+[-0.9, 0.8]s_{SP}$\\ 
   %%$ r^{(\phi: {\rm inf})} $  &$[-10.5,9.1]c_{SP}+[-8.2,5.3]s_{SP}$   & $[-11.0,11.3]c_{SP}+[-5.5,9.0]s_{SP} $& $[-3.6, 2.5]c_{SP}+[-4.2, 4.8]s_{SP}$  \\
   %%$ r^{(\phi: {\rm sup})} $  & $[-8.3,7.2]c_{SP}+[-6.7,3.9]s_{SP}$ & $[-7.7,9.0]c_{SP}+[-4.4,7.4]s_{SP}$ & $[-2.7, 1.7]c_{SP}+[-3.3, 3.8]s_{SP}$\\
   %%$ r^{({\rm high})} $  &      -0.13 & 0.15 & 0.02\\
   %%\hline
    %%\end{tabular}
    %%%
    \begin{tabular}{|c|c|}
        \hline
        $\sqrt{q^2}$-bin & $\int \langle I_{2} \rangle_{-}^r$ (\%) \\
        \hline
        $ r^{(\rho: {\rm sup})} $ & $[-2.0,1.9] \, c_{SP}+ [-0.09,5.0] \, s_{SP}$ \\
        \hline
        $ r^{(\phi: {\rm inf})} $ & $[-9.1,11] \, c_{SP}+[-5.3,8.2] \, s_{SP}$ \\ %[-9.1,10.5]
        \hline
        $ r^{(\phi: {\rm sup})} $ & $[-7.2,8.3] \, c_{SP}+[-3.9,6.7] \, s_{SP}$ \\
        \hline
        %%%%%%
        \hline
        $\sqrt{q^2}$-bin & $\int \langle I_4 \rangle_{+}^r$ (\%) \\
        \hline
        $ r^{(\rho: {\rm sup})} $ & $[-1.3,2.4] \, c_{SP} + [-4.2,-0.08 ] \, s_{SP}$ \\
        \hline
        $ r^{(\phi: {\rm inf})} $ & $[-11,9.6] \, c_{SP} + [-9.0,5.5] \, s_{SP} $ \\ %[-11.3,9.6]
        \hline
        $ r^{(\phi: {\rm sup})} $ & $[-9.0,7.7] \, c_{SP} + [-7.4,4.4] \, s_{SP}$ \\
        \hline
        %%%%%%
        \hline
        $\sqrt{q^2}$-bin & $\int \langle I_8 \rangle_{+}^r$ (\%) \\
        \hline
        $ r^{(\rho: {\rm sup})} $ & $[-2.2, 0.03] \, c_{SP} + [-0.9, 0.8] \, s_{SP}$ \\
        \hline
        $ r^{(\phi: {\rm inf})} $ & $[-3.6, 2.5] \, c_{SP} + [-4.2, 4.8] \, s_{SP}$ \\
        \hline
        $ r^{(\phi: {\rm sup})} $ & $[-2.7, 1.7] \, c_{SP} + [-3.3, 3.8] \, s_{SP}$ \\
        \hline %LATEST:
        $\sqrt{q^2}$-bin & $\int \langle I_{2} \rangle_{-}^r$ (\%) \\
        \hline
        $ r^{(\rho: {\rm sup})} $ & $[-66,-7.5] \, c_{SP}+ [-23,-11] \, s_{SP}$ \\
        \hline
        $ r^{(\phi: {\rm inf})} $ & $[-77,61] \, c_{SP}+[-53,82] \, s_{SP}$ \\ %[-9.1,10.5]
        \hline
        $ r^{(\phi: {\rm sup})} $ & $[-71,30] \, c_{SP}+[-50,54] \, s_{SP}$ \\
        \hline
        %%%%%%
        \hline 
        $\sqrt{q^2}$-bin & $\int \langle I_4 \rangle_{+}^r$ (\%) \\
        \hline
        $ r^{(\rho: {\rm sup})} $ & $[8.2,59] \, c_{SP} + [3.9,16] \, s_{SP}$ \\
        \hline
        $ r^{(\phi: {\rm inf})} $ & $[-67,83] \, c_{SP} + [-86,54] \, s_{SP} $ \\ %[-11.3,9.6]
        \hline
        $ r^{(\phi: {\rm sup})} $ & $[-31,76] \, c_{SP} + [-59,55] \, s_{SP}$ \\
        \hline
        %%%%%%
        \hline  
        $\sqrt{q^2}$-bin & $\int \langle I_8 \rangle_{+}^r$ (\%) \\
        \hline
        $ r^{(\rho: {\rm sup})} $ & $[-30,-2.4] \, c_{SP} + [-4.4,3.8] \, s_{SP}$ \\
        \hline
        $ r^{(\phi: {\rm inf})} $ & $[-46,45] \, c_{SP} + [-34,40] \, s_{SP}$ \\
        \hline
        $ r^{(\phi: {\rm sup})} $ & $[-26,33] \, c_{SP} + [-17,33] \, s_{SP}$ \\
        \hline
    \end{tabular}
    \caption{SM predictions for the non-vanishing angular observables that probe the interference between the $S$- and $P$-waves. The parameters appearing stand for $c_{SP} \equiv \cos( \Delta_{SP} )$ and $s_{SP} \equiv \sin( \Delta_{SP} )$. The relation $ \int \langle I_1 \rangle_-^r = - \int \langle I_2 \rangle_-^r $ holds true.
    Relevant definitions can be found in Sec.~\ref{sec:observables}, see in particular Eqs.~\eqref{isnormalised} and \eqref{intnotation}.
    The same overall multiplicative factor shown in the caption of Tab.~\ref{gammas,i2} applies.
    %[\rd{can you provide for inner use unbinned plots of the angular observables as a function of $q^2$?}]
    }
\label{i2i4i8}
 \end{table}
\begin{table}
%%\hspace{-2cm}
\centering
    \renewcommand{\arraystretch}{1.4}
    \begin{tabular}{|c|c|}
        \hline
        $\sqrt{q^2}$-bin & $\int \langle I_{2} \rangle_{-}^r$ (\%) \\
        \hline
        $ r^{(\rho: {\rm sup})} $ & $[7.6, 66] \, c_{SP}+ [11,23] \, s_{SP}$ \\
        \hline
        $ r^{(\phi: {\rm inf})} $ & $[-60,-1.3] \, c_{SP}+[-82,47] \, s_{SP}$ \\ %[-9.1,10.5]
        \hline
        $ r^{(\phi: {\rm sup})} $ & $[-26,71] \, c_{SP}+[-54,-8.5] \, s_{SP}$ \\
        \hline
        %%%%%%
        \hline 
        $\sqrt{q^2}$-bin & $\int \langle I_4 \rangle_{+}^r$ (\%) \\
        \hline
        $ r^{(\rho: {\rm sup})} $ & $[-59,-8] \, c_{SP} + [-16,-3.9] \, s_{SP}$ \\
        \hline
        $ r^{(\phi: {\rm inf})} $ & $[1.8,67] \, c_{SP} + [-51,86] \, s_{SP} $ \\ %[-11.3,9.6]
        \hline
        $ r^{(\phi: {\rm sup})} $ & $[-76,29] \, c_{SP} + [9.5,59] \, s_{SP}$ \\
        \hline
        %%%%%%
        \hline 
        $\sqrt{q^2}$-bin & $\int \langle I_8 \rangle_{+}^r$ (\%) \\
        \hline
        $ r^{(\rho: {\rm sup})} $ & $[-30,-2.4] \, c_{SP} + [-4.5,3.9] \, s_{SP}$ \\
        \hline
        $ r^{(\phi: {\rm inf})} $ & $[3.9,45] \, c_{SP} + [-34,30] \, s_{SP}$ \\
        \hline
        $ r^{(\phi: {\rm sup})} $ & $[6.8,33] \, c_{SP} + [-17,29] \, s_{SP}$ \\
        \hline
    \end{tabular}
    \caption{Corrected for the fudge factor}
 \end{table}

 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{table}[]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline 
    $\sqrt{q^2}$-bin $r$ & $\Gamma^r$ (SM+NP) & $\int \langle I_5 \rangle_{+}^r$ (\%) & $\int \langle I_5 \rangle_{-}^r$ (\%) & $\int \langle I_7 \rangle_{+}^r$ (\%) & $\int \langle I_6 \rangle_{+}^r$ (\%) \\
    %\cline{3-6}
    %& & \multicolumn{4}{c|}{$ [10^{-2}] $} \\
    \hline 
   %%$ r^{({\rm low})} $ & $0.08 + 0.09|\tilde{C}_{10}|^2$       & $0.5$ & $-0.5$  &$-0.5$ &$-0.4$\\ 
   %%$ r^{(\eta)} $ &     $ 0.03+  0.02|\tilde{C}_{10}|^2  $     & $0.2$ &  $-0.2$   &$-0.2$&$-0.2$\\ 
   %%$ r^{(\rho: {\rm inf})} $ & $1.09+  0.11|\tilde{C}_{10}|^2$ & $1.8$ &  $0.7$ &    $-2.4$&$1.0$\\
   $ r^{(\rho: {\rm sup})} $ & $0.59+ 0.10 \, |\tilde{C}_{10}|^2$  & $<1.9$&  $<3.2$ &$ <2$&$<4.4$ \\ 
   $ r^{(\phi: {\rm inf})} $ & $1.00+ 0.04 \, |\tilde{C}_{10}|^2 $ & $<0.8$ &  $<1.2$&$  <1.3$&$<1.8$\\
   $ r^{(\phi: {\rm sup})} $ & $0.85+ 0.03 \, |\tilde{C}_{10}|^2$  & $<0.6$& $<1.4$ &$<2.4 $&$<2.2$\\
   %%$ r^{({\rm high})} $  &     $0.01+ 0.03|\tilde{C}_{10}|^2$  & $-0.07$& $0.17$ &  $-0.008$&$ 0.3$\\
       \hline
    \end{tabular}
    \caption{\rd{To be removed except for the decay rate, which should be moved} The decay rate in the presence of NP and observables that vanish in the SM, here calculated for $C_9'=C_{10}'=C_9^{\rm NP}=0$ and non-zero $C_{10}$. The cases $\braket{I_5}_+$ and $\braket{I_7}_+$ are sensitive to the SM-NP interference in the presence of the $S$-wave. Instead, $\braket{I_5}_-$ and $\braket{I_6}_+$ are sensitive to the SM-NP interference through the $P$-wave, while $\braket{I_7}_-$ approximately vanishes. The same overall multiplicative factor shown in the caption of Tab.~\ref{gammas,i2} applies; additionally, the four last columns are multiplied by $ \tilde{C}_{10} $.}
    \label{NPobsevables}
\end{table}
\end{comment}

\begin{table}[]
    \centering
    \renewcommand{\arraystretch}{1.4}
   \begin{tabular}{|c|c|}
        \hline
        $\sqrt{q^2}$-bin & $\int \langle I_{5} \rangle_{-}^r$ (\%) \\
        \hline
        $ r^{(\rho: {\rm sup})} $ & $[-1.9,-1.4] \, c_{\rho {\rm NP}}+ [-2.6,-2.2] \, s_{\rho {\rm NP}}$ \\
        \hline
        $ r^{(\phi: {\rm inf})} $ & $[0.1,0.8] \, c_{\rho {\rm NP}}+[-0.4,0.9] \, s_{\rho {\rm NP}}$ \\
        \hline
        $ r^{(\phi: {\rm sup})} $ & $[-0.9,0.1] \, c_{\rho {\rm NP}}+[-1.0,-0.7] \, s_{\rho {\rm NP}}$ \\ %[-1,-0.7]
        \hline
        %%%%%%
        \hline
        $\sqrt{q^2}$-bin & $\int \langle I_6 \rangle_{+}^r$ (\%) \\
        \hline
        $ r^{(\rho: {\rm sup})} $ & $[-2.7,-2.0] \, c_{\rho {\rm NP}} + [ -3.5,-2.8] \, s_{\rho {\rm NP}}$ \\
        \hline
        $ r^{(\phi: {\rm inf})} $ & $[0.2,1.2] \, c_{\rho {\rm NP}} + [-0.6,1.3] \, s_{\rho {\rm NP}} $ \\
        \hline
        $ r^{(\phi: {\rm sup})} $ & $[-1.5,0.2] \, c_{\rho {\rm NP}} + [-1.6,-1.1] \, s_{\rho {\rm NP}}$ \\
        \hline
    \end{tabular}
    \caption{Observables that vanish in the SM, arising from the interference of the $P$-wave and NP, here calculated for $C_9'=C_{10}'=C_9^{\rm NP}=0$ and non-zero $C_{10}$. The parameters appearing stand for $c_{\rho {\rm NP}}=\cos( \Delta_{\rho {\rm NP}} )$ and $s_{\rho {\rm NP}}=\sin( \Delta_{\rho {\rm NP}} )$. The other $P$-wave dependent observable $\braket{I_7}_-$ approximately vanishes.
    The NP does not interfere with the SM in the decay rate, and can thus be neglected.
    Relevant definitions can be found in Sec.~\ref{sec:observables}, see in particular Eqs.~\eqref{isnormalised} and \eqref{intnotation}.
    The same overall multiplicative factor shown in the caption of Tab.~\ref{gammas,i2} applies; additionally, the observables are multiplied by $ \tilde{C}_{10}$.
    %[\rd{can you provide for inner use unbinned plots of the angular observables as a function of $q^2$?}]
    }
    %there is a normalization problem, the result must be $ \propto C_2 \times C_{10}^\ast $, while here it is instead $ \propto |C_2|^2 \times C_{10}^\ast $: Ele extracted the numerics things properly
    \label{NPobsevablesPwave}
\end{table}
\begin{table}[]
    \centering
    \renewcommand{\arraystretch}{1.4}
   \begin{tabular}{|c|c|}
        \hline
        $\sqrt{q^2}$-bin & $\int \langle I_{5} \rangle_{-}^r$ (\%) \\
        \hline
        $ r^{(\rho: {\rm sup})} $ & $[-8.3,-4.9] \, c_{\rho {\rm NP}}+ [13,15] \, s_{\rho {\rm NP}}$ \\
        \hline
        $ r^{(\phi: {\rm inf})} $ & $[-5.0,3.6] \, c_{\rho {\rm NP}}+[6.0,8.3] \, s_{\rho {\rm NP}}$ \\
        \hline
        $ r^{(\phi: {\rm sup})} $ & $[-6.6,-3.1] \, c_{\rho {\rm NP}}+[-4.9,0.9] \, s_{\rho {\rm NP}}$ \\ %[-1,-0.7]
        \hline
        %%%%%%
        \hline
        $\sqrt{q^2}$-bin & $\int \langle I_6 \rangle_{+}^r$ (\%) \\
        \hline
        $ r^{(\rho: {\rm sup})} $ & $[-12,-6.8] \, c_{\rho {\rm NP}} + [17,21] \, s_{\rho {\rm NP}}$ \\
        \hline
        $ r^{(\phi: {\rm inf})} $ & $[-7.8,5.7] \, c_{\rho {\rm NP}} + [9.7,13] \, s_{\rho {\rm NP}} $ \\
        \hline
        $ r^{(\phi: {\rm sup})} $ & $[-11,-5.0] \, c_{\rho {\rm NP}} + [-7.8,1.4] \, s_{\rho {\rm NP}}$ \\
        \hline %LATEST:
        $\sqrt{q^2}$-bin & $\int \langle I_{5} \rangle_{-}^r$ (\%) \\
        \hline
        $ r^{(\rho: {\rm sup})} $ & $[4.9,8.3] \, c_{\rho {\rm NP}}+ [-15,-13] \, s_{\rho {\rm NP}}$ \\
        \hline
        $ r^{(\phi: {\rm inf})} $ & $[-3.6,5.0] \, c_{\rho {\rm NP}}+[-8.3,-6.0] \, s_{\rho {\rm NP}}$ \\
        \hline
        $ r^{(\phi: {\rm sup})} $ & $[3.1,6.6] \, c_{\rho {\rm NP}}+[-0.9,4.9] \, s_{\rho {\rm NP}}$ \\ %[-1,-0.7]
        \hline
        %%%%%%
        \hline
        $\sqrt{q^2}$-bin & $\int \langle I_6 \rangle_{+}^r$ (\%) \\
        \hline
        $ r^{(\rho: {\rm sup})} $ & $[6.8,12] \, c_{\rho {\rm NP}} + [-21,-17] \, s_{\rho {\rm NP}}$ \\
        \hline
        $ r^{(\phi: {\rm inf})} $ & $[-5.7,7.8] \, c_{\rho {\rm NP}} + [-13,-9.7] \, s_{\rho {\rm NP}} $ \\
        \hline
        $ r^{(\phi: {\rm sup})} $ & $[5.0,11] \, c_{\rho {\rm NP}} + [-1.4,7.8] \, s_{\rho {\rm NP}}$ \\
        \hline
    \end{tabular}
    \caption{Corrected fudge factor}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> omegarho.tex <==
\section{$\omega$ and $\pi$ signs in J vs W, going to two pions}

For the W type: They come from the $D$ with a $u\overline{u}$ so they have the same sign. We assume the form factors also to be the same (I guess that's OK since they are determined from spin arguments, nothing to do with isospin). Then you have 
\begin{equation}
    b_\rho/P_\rho+b_\omega/P_\omega \approx b_\rho/P_\rho(1+a_\omega s/P_\omega)
\end{equation}
The rest are the same.

For the J type: They come from $\langle V |\overline{d}d|0\rangle$ which gives an opposite sign for the two of them. Then we have  
\begin{equation}
   m_\rho f_\rho( b_\rho/P_\rho-b_\omega/P_\omega) \approx m_\rho f_\rho b_\rho/P_\rho(1-a_\omega s/P_\omega)
\end{equation}



Can we now factor out this $b_{\rho\omega}$ if they come with a different phase? I guess the $\phi_\omega$ is supposed to play this role but still it is not coherent. In reality it is 
\begin{equation}
    \frac{b_\rho(1+a_\omega s/P_\omega)}{P_\rho} W(q^2) + \frac{b_\rho(1-a_\omega s/P_\omega)}{P_\rho} J(q^2)
\end{equation}

The universal $\phi_\omega$ phase makes some sense to be able to explain the data, since in the $p^2$ picture we have from the previous equation, after integrating the $W$ and $J$,  
\begin{equation}
     \frac{b_\rho(1+a_\omega s/P_\omega)}{P_\rho}x(p^2)+ \frac{b_\rho(1-a_\omega s/P_\omega)}{P_\rho} y(p^2)
\end{equation} 
where moreover the $p^2$ dependence of $x,y$ is mild. 

When using the $C_9$ approximation we should end up with 
\begin{equation}
    \frac{b_\rho}{P_\rho(p^2)}\frac{2f_\rho^2}{P_\rho(q^2)}-\frac{b_\rho}{P_\rho(p^2)}a_\omega \frac{s}{P_\omega(p^2)}\frac{2f_\omega^2}{3P_\omega(q^2)} +\frac{b_\rho(1+a_\omega s/P_\omega(p^2))}{P_\rho(p^2)}\frac{\sqrt{2}f_\phi^2}{3P_\phi(q^2)}
\end{equation}
[needs to be checked if this approximation is close to the full approach]
For the discussion of phases, see the other note (isospinargument.tex)

==> tables.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{|cc|c|c|c|c|c|}
        \hline
         & Topology & Decay channel & $ {Re} [a_i] $ & $ {Im} [a_i] $ & FF (\%) & $L$/$S$ \\
        \hline
        \hline
         & cascade & $ D^0 \to \pi^- \, [a_1 (1260)^+ \to \pi^+ \, \rho (770)^0] $ & $ 100 $ (fixed) & $ 0 $ (fixed) & $ 38 \pm 4 $ & 1 \\
        \hline
        $ \ast $ & Q2B & $ D^0 \to [ \rho (770)^0 \, \rho (770)^0 ]_{L=2} $ & $ -34 \pm 6 $ & $ -8 \pm 35 $ & $ 8 \pm 4 $ & 2 \\
        \hline
        $ \ast $ & Q2B & $ D^0 \to [ \rho (770)^0 \, \rho (770)^0 ]_{L=1} $ & $ -3 \pm 2 $ & $ -21 \pm 4 $ & $ 7 \pm 2 $ & 1 \\
        \hline
         & Q2B & $ D^0 \to f_0 (500) \, \rho (770)^0 $ & $ 42 \pm 6 $ & $ -25 \pm 7 $ & $ 7 \pm 3 $ & 1 \\
        \hline
         & cascade & $ D^0 \to \pi^- \, [a_1 (1640)^+ \to [ \pi^+ \, \rho (770)^0 ]_{L=2} ] $ & $ -125 \pm 35 $ & $ -11 \pm 20 $ & $ 4 \pm 2 $ & 1 \\
        \hline
         & cascade & $ D^0 \to \pi^+ \, [a_1 (1260)^- \to \pi^- \, \rho (770)^0] $ & $ - $ & $ - $ & $ 3 \pm 1 $ & 1 \\
        \hline
        $ \ast $ & Q2B & $ D^0 \to [ \rho (770)^0 \, \rho (770)^0 ]_{L=0} $ & $ 2 \pm 2 $ & $ 9 \pm 2 $ & $ 2 \pm 2 $ & 0 \\
        \hline
    \end{tabular}
    \caption{Extract of Tab.~3 from \cite{dArgent:2017gzv} (uncertainties combined in quadrature) discussing $ D^0 \to \pi^+ \pi^- \pi^+ \pi^- $; it shows some of the channels that are expected to contribute to $ D^0 \to \pi^+ \pi^- \ell^+ \ell^- $ at a non-negligible level; the lepton pair is coming from $\rho (770)^0$. Q2B stands for quasi two-body. The Fit Fraction (FF) gives a measure of the relative importance of each channel, not considering possible interference terms. Channels indicated by $ \ast $ are used in the analysis of \cite{DeBoer:2018pdx}. [comment on CPV; rescale $a_i$; $L$ should be the ORBITAL angular momentum (to be added to the spin component); I believe FF is an integrated quantity, and not local; associate FFs to particular vertices for ease of comparison (in particular, COMPLEX factor for $ \rho \to \pi \pi $, call it $g_{\rho \pi \pi}$)] [\rd{$ D^0 \to f_0 (500) \, \rho (770)^0 $ may not be well defined, because $ f_0 (500) $ is broad}] [For a discussion about triangle singularities, see \cite{He:2023plt}][\textbf{indicate spin and isospin Clebsch-Gordan, cost of $L$, symmetry factors, mass suppression/phase space}][You can have a look at \cite{ElHassanElAaoud:1999min}]}
    \label{tab:amplitude_analysis_4pi}
\end{table}
%note that the channel $ D^0 \to \phi (1020) \, \rho (770)^0 $ is expected to contribute to $ D^0 \to \pi^+ \pi^- \ell^+ \ell^- $, but not to $ D^0 \to \pi^+ \pi^- \pi^+ \pi^- $

\begin{table}[t]
    \centering
    \begin{tabular}{|cc|c|c|c|c|c|c|}
        \hline
         & Topology & Decay channel & $ |a_i| $ & $ \arg (a_i) $ (rad) & FF (\%) & & $L$/$S$ \\
        \hline
        \hline
        $ \ast $ & Q2B & $ D^0 \to [\phi (1020) \, (\rho - \omega)^0]_{L=0} $ & $ 1 $ (fixed) & $ 0 $ (fixed) & $ 23.8 \pm 0.6 $ & $ K, \pi $ & 0 \\
        \hline
         & cascade & $ D^0 \to K_1 (1270)^+ \, K^- $ & $ 0.45 \pm 0.02 $ & $ 2.02 \pm 0.06 $ & $ 18 \pm 1 $ & $ K $ & 1 \\
        \hline
         & cascade & $ D^0 \to K_1 (1270)^- \, K^+ $ & $ 0.22 \pm 0.01 $ & $ 2.09 \pm 0.08 $ & $ 4.3 \pm 0.5 $ & $ K $ & 1 \\
        \hline
        $ \ast $ & Q2B & $ D^0 \to [\phi (1020) \, (\rho - \omega)^0]_{L=2} $ & $ 1.31 \pm 0.04 $ & $ 0.54 \pm 0.03 $ & $ 2.3 \pm 0.1 $ & $ K, \pi $ & 2 \\
        \hline
        %$ D^0 \to \phi (1020) [\pi^+ \pi^-]_{L=0} $ &  \\
        %\hline
         & Q2B & $ D^0 \to [\phi (1020) \, \rho (1450)^0]_{L=1} $ & $ 0.76 \pm 0.08 $ & $ 1.17 \pm 0.06 $ & $ 1.0 \pm 0.1 $ & $ K, \pi $ & 1 \\
        \hline
        %$ D^0 \to a_1 (1260)^+ \pi^- $ &  \\
        %\hline
        %$ D^0 \to a_1 (1260)^- \pi^+ $ &  \\
        %\hline
        $ \ast $ & Q2B & $ D^0 \to [\phi (1020) \, (\rho - \omega)^0]_{L=1} $ & $ 0.16 \pm 0.01 $ & $ 0.28 \pm 0.08 $ & $ 0.43 \pm 0.06 $ & $ K, \pi $ & 1 \\
        \hline
         & ``semi-res.'' & $ D^0 \to [K^+ \, K^-]_{L=0} \, (\rho - \omega)^0 $ & $ 0.20 \pm 0.04 $ & $ 3.0 \pm 0.3 $ & $ 0.27 \pm 0.06 $ & $ K $ & 1 \\
        \hline
        \hline
         & ``semi-res.'' & $ D^0 \to \phi (1020) \, [\pi^+ \, \pi^-]_{L=0} $ & $ 0.049 \pm 0.004 $ & $ -1.7 \pm 0.4 $ & $ 1.5 \pm 0.3 $ & $ \pi $ & 1 \\
        \hline
         & cascade & $ D^0 \to a_1 (1260)^+ \, \pi^- $ & $ 0.19 \pm 0.04 $ & $ -2.8 \pm 0.4 $ & $ 0.5 \pm 0.2 $ & $ \pi $ & 1 \\
        \hline
         & cascade & $ D^0 \to a_1 (1260)^- \, \pi^+ $ & $ 0.19 \pm 0.03 $ & $ 0.2 \pm 0.4 $ & $ 0.5 \pm 0.2 $ & $ \pi $ & 1 \\
        \hline
    \end{tabular}
    \caption{Extract of Tab.~2 from \cite{LHCb:2018mzv} (uncertainties combined in quadrature) discussing $ D^0 \to K^+ K^- \pi^+ \pi^- $; it shows some of the channels that are expected to contribute to $ D^0 \to \pi^+ \pi^- \ell^+ \ell^- $ (indicated in the last column by a $\pi$) and $ D^0 \to K^+ K^- \ell^+ \ell^- $ (indicated in the last column by a $K$) at a non-negligible level. Additionally, note that $ K_1 (1270)^+ $ has a large fit fraction into $ [(\rho - \omega)^0 \, K^+]_{L=0} $, of $ (50 \pm 5) \% $; the only decay channel considered for $a_1 (1260)^+$ is $[\phi (1020) \pi^+]_{L=0}$. (See their Tab.~4 for individual $ \rho (770)^0 $ and $ \omega (782) $ contributions, the former being always much larger as given by their respective fit fractions found in \cite{LHCb:2018mzv}.) In the case of $ D^0 \to K^+ K^- \ell^+ \ell^- $, if one neglects the contribution from $\rho(1450)^0$, the lepton pair is always coming from $(\rho - \omega)^0$, while in the case of $ D^0 \to \pi^+ \pi^- \ell^+ \ell^- $ the lepton pair is coming from $\phi (1020)$. See Tab.~\ref{tab:amplitude_analysis_4pi} for more comments. [comment on CPV; rescale $a_i$; $L$ should be the ORBITAL angular momentum (to be added to the spin component); I believe FF is an integrated quantity, and not local; associate FFs to particular vertices for ease of comparison (e.g., COMPLEX factor for $ \phi \to K K $, $ K_1 \to \rho K $, $ a_1 \to \phi \pi $); $f_0 (500)$ not included in the decomposition, but it should reflect into $[\pi^+ \, \pi^-]_{L=0}$/on the other hand \cite{dArgent:2017gzv} considers them separately: not sure of its meaning][\textbf{indicate spin and isospin Clebsch-Gordan, cost of $L$, symmetry factors, mass suppression/phase space; it is however difficult to compare because in one case it is $ \rho $, and in the other $ \pi \pi $}][You can have a look at \cite{ElHassanElAaoud:1999min}]}
    \label{tab:amplitude_analysis_2pi2K}
\end{table}

==> variouscomments.tex <==
\subsection{Implementation-comments}

[About the inclusion of the $ \sigma $: it is more difficult to prove scalar dominance (the idea being that the intermediate dynamics is dominated by resonances, these being vectors, scalars, etc.), ``since the information on the scalar sector is quite poor'' \cite{Pich:2018ltt}]

[Branco et al.: ``Since $ B^0_d $ and $ \pi $ are spinless, $ \rho $ must have helicity zero. Thus, the dependence on the helicity angle $ \theta $ is proportional to $ \cos \theta $.'']

[factor 2 for $\rho \rho$ w.r.t. $ \rho \sigma $]


{\color{red}After factorization, we now write down also the non-leptonic matrix element:} [{\color{red}LVS: should complex phases labelled $V'$ and $V''$ be equal?; (\textbf{that should model a correction to factorization coming from rescattering}, which normally comes with a modulation beyond a phase)?; do they depend on other properties of the daughter particles?}]


\subsection{Approximate $C_9^{eff}$ for the $\rho/\omega$-mediated process}



 

%[also quote private communication with Gudrun]
 {\color{red}LVS: you should rephrase this paragraph; this discussion is yet too abstract: write something like $(A + B) \times (a + b)_{\rm had} \neq A \times a_{\rm had} + B \times b_{\rm had}$ because the two hadronic elements $a_{\rm had}$ and $b_{\rm had}$ are not equivalent}].
{\color{red} The contribution of $\sigma$ compared to the $W$-like ones of the vector resonances is...}

{\color{red}Keeping in mind the degree of precision discussed above when considering the modified $C^W$, the reader may consider useful the expression...}
{\color{red} We stress that we do not use the modified $C^W$ in our following discussion.}



